Reducing information dependency does not cause training data privacy. Adversarially non-robust features do

In this paper, we challenge the prevailing view that information dependency (including rote memorization) drives training data exposure to image reconstruction attacks. We show that extensive exposure can persist without rote memorization and is instead caused by a tunable connection to adversarial robustness. We begin by presenting three surprising results: (1) recent defenses that inhibit reconstruction by Model Inversion Attacks (MIAs), which evaluate leakage under an idealized attacker, do not reduce standard measures of information dependency (HSIC); (2) models that maximally memorize their training datasets remain robust to MIA reconstruction; and (3) models trained without seeing 97% of the training pixels, where recent information-theoretic bounds give arbitrarily strong privacy guarantees under standard assumptions, can still be devastatingly reconstructed by MIA. To explain these findings, we provide causal evidence that privacy under MIA arises from what the adversarial examples literature calls ``non-robust'' features (generalizable but imperceptible and unstable features). We further show that recent MIA defenses obtain their privacy improvements by unintentionally shifting models toward such features. To establish this causal relationship, we introduce Anti Adversarial Training (AT-AT), a training regime that intentionally learns non-robust features to obtain both superior reconstruction defense and higher accuracy than state-of-the-art defenses. Our results revise the prevailing understanding of training data exposure and reveal a new privacy-robustness tradeoff.

==> dareDEVALII/Figure_code/MIA-onerow.tex <==
\begin{figure}[h]
\centering
\vspace{-1em}
\resizebox{\textwidth}{!}{%
\setlength\tabcolsep{2pt}%
{\tiny
\begin{tabular}{ccccccccc}
  \textbf{Orig.} & \textbf{NoDef} & \textbf{MID} & \textbf{BiDO} & 
  \textbf{TL-DMI} & \textbf{RoLSS} & \textbf{{ RoLSS}-SSF}& \textbf{NegLS} & \textbf{AT-AT} \\
    \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_reference.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_NoDef.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_MID.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_BiDO.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_TL.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_RoLSS.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_RoLSS-SSF.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_NegLS.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_AT-AT.png} 
\end{tabular}%
}
}
\caption{PPA reconstructions on a ResNet-152. Class selected via max conf. Full results in Fig. \ref{fig:MIA-grid-R152}.}
\label{fig:MIA-grid-R152-onerow}
\end{figure}


==> dareDEVALII/Figure_code/MIA_grid-protocol-MaxConf.tex <==

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{%
\setlength\tabcolsep{2pt}%
\begin{tabular}{cccccccc}
  \textbf{Reference} & \textbf{No Defense} & \textbf{MID} & \textbf{BiDO} & 
  \textbf{TL-DMI} & \textbf{RoLSS} & \textbf{NegLS} & \textbf{AT-AT} \\
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AaronEckhart_reference.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AaronEckhart_NoDef.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AaronEckhart_mid.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AaronEckhart_bido.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AaronEckhart_TL.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AaronEckhart_rolss.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AaronEckhart_NegLS.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AaronEckhart_AT-AT.png} \\
    \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamBrody_reference.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamBrody_NoDef.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamBrody_mid.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamBrody_bido.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamBrody_TL.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamBrody_rolss.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamBrody_NegLS.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamBrody_AT-AT.png} \\
      \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamMcKay_reference.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamMcKay_NoDef.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamMcKay_mid.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamMcKay_bido.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamMcKay_TL.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamMcKay_rolss.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamMcKay_NegLS.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamMcKay_AT-AT.png} \\
    \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamSandler_reference.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamSandler_NoDef.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamSandler_mid.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamSandler_bido.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamSandler_TL.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamSandler_rolss.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamSandler_NegLS.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdamSandler_AT-AT.png} \\
    \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdrienBrody_reference.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdrienBrody_NoDef.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdrienBrody_mid.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdrienBrody_bido.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdrienBrody_TL.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdrienBrody_rolss.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdrienBrody_NegLS.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/AdrienBrody_AT-AT.png} \\
    \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/WandaDeJesus_reference.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/WandaDeJesus_NoDef.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/WandaDeJesus_mid.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/WandaDeJesus_bido.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/WandaDeJesus_TL.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/WandaDeJesus_rolss.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/WandaDeJesus_NegLS.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid-protocol-MaxConf/WandaDeJesus_AT-AT.png} \\
\end{tabular}%
}
\caption{Image reconstructions generated from PPA attacks for each defense applied on a ResNet-18. \hl{Each selected image is selected by maximum confidence on the evaluation model.}  \textcolor{red}{OLD}
}
\label{fig:pictures-of-reconstructions}
\end{figure}


==> dareDEVALII/Figure_code/MIA_grid.tex <==

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{%
\setlength\tabcolsep{2pt}%
\begin{tabular}{cccccccc}
  \textbf{Reference} & \textbf{No Defense} & \textbf{MID} & \textbf{BiDO} & 
  \textbf{TL-DMI} & \textbf{RoLSS} & \textbf{NegLS} & \textbf{AT-AT} \\
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AaronEckhart_reference.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AaronEckhart_NoDef.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AaronEckhart_mid.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AaronEckhart_bido.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AaronEckhart_TL.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AaronEckhart_rolss.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AaronEckhart_NegLS.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AaronEckhart_AT-AT.png} \\
    \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdamBrody_reference.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdamBrody_NoDef.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdamBrody_mid.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdamBrody_bido.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdamBrody_TL.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdamBrody_rolss.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdamBrody_NegLS.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdamBrody_AT-AT.png} \\
    \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdrienBrody_reference.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdrienBrody_NoDef.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdrienBrody_mid.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdrienBrody_bido.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdrienBrody_TL.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdrienBrody_rolss.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdrienBrody_NegLS.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/AdrienBrody_AT-AT.png} \\
    \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/WandaDeJesus_reference.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/WandaDeJesus_NoDef.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/WandaDeJesus_mid.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/WandaDeJesus_bido.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/WandaDeJesus_TL.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/WandaDeJesus_rolss.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/WandaDeJesus_NegLS.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/ModelInversionGrid/WandaDeJesus_AT-AT.png}
\end{tabular}%
}
\caption{Examples of images generated from plug and play attack for each defense on a ResNet-18.}
\end{figure}


==> dareDEVALII/Figure_code/MIA_onerow_GARBAGE.tex <==
\begin{figure}[h]
\centering
\vspace{-1em}
\resizebox{\textwidth}{!}{%
\setlength\tabcolsep{2pt}%
{\tiny
\begin{tabular}{ccccccccc}
  \textbf{SPACIFIERSPACE} & \textbf{SPACIFIERSPACE} & \textbf{SPACIFIERSPACE} & \textbf{SPACIFIERSPACE} & 
  \textbf{SPACIFIERSPACE} & \textbf{SPACIFIERSPACE} & \textbf{SPACIFIERSPACE}& \textbf{SPACIFIERSPACE} & \textbf{SPACIFIERSPACE} \\
    \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_reference.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_NoDef.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_MID.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_BiDO.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_TL.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_RoLSS.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_RoLSS-SSF.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_NegLS.png} &
  \includegraphics[width=0.5in]{dareDEVALII/Figures/ModelInversionGrid-protocol-R152/WandaDeJesus_R152_AT-AT.png} 
\end{tabular}%
}
}
\caption{PPA reconstructions on a ResNet-152. Class selected via max conf. Full results in Fig. \ref{fig:MIA-grid-R152}.}
\label{fig:MIA-grid-R152-onerow}
\end{figure}

\bigskip \bigskip

==> dareDEVALII/Figure_code/adversarial_examples.tex <==
% \documentclass{article}
% \usepackage{graphicx}
% \usepackage[margin=1in]{geometry}
% \usepackage{amsmath}
% \usepackage{caption}

% \begin{document}

\begin{figure}[h]
\centering
\resizebox{\textwidth}{!}{%
\setlength\tabcolsep{2pt}%
\begin{tabular}{cccccccc}
  \textbf{Original Image} & \boldmath$\epsilon=1$ & \boldmath$\epsilon=0.5$ & \boldmath$\epsilon=0.031$ &
  \boldmath$\epsilon=0.025$ & \boldmath$\epsilon=0.0025$ & \boldmath$\epsilon=0.0005$ & \boldmath$\epsilon=0.00001$ \\

  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/vayqyjba_original_image_0.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_1_0.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.5_0.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.031_0.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.025_0.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.0025_0.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.0005_0.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_1e-05_0.png} \\

  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/vayqyjba_original_image_1.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_1_1.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.5_1.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.031_1.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.025_1.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.0025_1.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.0005_1.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_1e-05_1.png} \\

  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/vayqyjba_original_image_2.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_1_2.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.5_2.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.031_2.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.025_2.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.0025_2.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_0.0005_2.png} &
  \includegraphics[width=1in]{dareDEVALII/Figures/adversarial_examples/rjl90za1_adversarial_image_epsilon_1e-05_2.png} \\
\end{tabular}%
}
\caption{Adversarial examples for different perturbation strengths $\epsilon$ for three individuals. Larger $\epsilon$ values introduce more visible distortion. \textcolor{red}{[Not final product, just made code and gathered images in case we want something like this]}}
\end{figure}

% \end{document}

==> dareDEVALII/Figure_code/lasso_mask.tex <==

\begin{figure}[h]
    \centering
    \includegraphics[width=0.2\linewidth]{dareDEVALII/Figures/lasso/vayqyjba_lasso_mask.png}
    \caption{The mask applied to images to delete pixels. }
    \label{fig:lasso_mask}
\end{figure}

==> dareDEVALII/Sections/DIAGRAM_mockup_ATAT.tex <==
% ===== Preamble (add once) =====
\usepackage{tikz}
\usepackage{amsmath}
\usetikzlibrary{arrows.meta,positioning,fit}

% ===== Figure =====
\begin{figure}[t]
\centering
\begin{tikzpicture}[
  % --- styles ---
  pane/.style={draw, minimum width=46mm, minimum height=24mm, inner sep=2mm},
  smallpane/.style={draw, minimum width=46mm, minimum height=24mm, inner sep=2mm},
  box/.style={draw, minimum width=32mm, minimum height=14mm, align=center},
  small/.style={draw, minimum width=16mm, minimum height=10mm, align=center},
  lab/.style={font=\bfseries},
  eq/.style={font=\scriptsize, align=left},
  >={Latex[length=2mm]}
]

% ----- column titles -----
\node[lab] (ct1) at (0, 4.8) {Vanilla};
\node[lab] (ct2) at (5.4, 4.8) {AT};
\node[lab] (ct3) at (10.8, 4.8) {AT-AT};

% =======================
% Row 1 (top): single centered pane under AT
% =======================
\node (p1) [pane] at (5.4, 3.2) {};               % top pane (same size as others)
\node[lab, anchor=east] at ([xshift=-6mm]p1.west) {Training example (Yoda)};
\node at (p1) {Yoda};                              % label inside top pane

% =======================
% Row 2 (middle): only AT column pane
% =======================
\node (p2) [pane] at (5.4, 0.9) {};
\node[lab, anchor=east] at ([xshift=-6mm]p2.west) {Adversarial perturbation (Yoda $\rightarrow$ Luke)};

% Content inside AT pane: PGD -> adversarial example
\node[small] (xin)  at ([xshift=-7mm,yshift=5mm]p2.center) {Yoda};
\node[small, below=2mm of xin] (pgd) {PGD};
\node at ([xshift=0mm,yshift=5mm]p2.center) {$+$};
\node[small, minimum width=20mm, minimum height=12mm] (xadv) at ([xshift=13mm,yshift=5mm]p2.center) {Luke};

% =======================
% Row 3 (bottom): three panes (Vanilla, AT, AT-AT)
% =======================
\node (p31) [pane] at (0, -1.5) {};
\node (p32) [pane] at (5.4, -1.5) {};
\node (p33) [pane] at (10.8, -1.5) {};
\node[lab, anchor=east] at ([xshift=-6mm]p31.west) {Compute Loss};

% Vanilla loss cell
\node[align=left] at ([yshift=5mm]p31.center) {Yoda $\rightarrow$ Yoda};
\node[eq] at ([yshift=-5mm]p31.center) {$\displaystyle \min_{\theta}\; \mathbb{E}[\,L(\theta,x,y)\,]$};

% AT loss cell
\node[align=left] at ([yshift=5mm]p32.center) {Luke $\rightarrow$ Yoda};
\node[eq] at ([yshift=-5mm]p32.center) {$\displaystyle \min_{\theta}\; \max_{\delta\in S} L(\theta, x+\delta, y)$};

% AT-AT loss cell
\node[align=left] at ([yshift=8mm]p33.center) {Yoda $\rightarrow$ Yoda};
\node[align=left] at ([yshift=1mm]p33.center)  {Luke $\rightarrow$ Luke};
\node[eq]         at ([yshift=-8mm]p33.center) {$\displaystyle
\min_{\theta}\; \mathbb{E}\!\big[\,L(\theta,x,y) + \lambda \cdot \max_{\delta\in S} L(\theta, x+\delta, y^{\prime})\,\big]$};

% =======================
% Arrows (edge-to-edge)
% =======================
% From top pane to bottom-left pane (diagonal)
\draw[->] (p1.south west) -- (p31.north);

% From top pane to bottom-right pane (diagonal)
\draw[->] (p1.south east) -- (p33.north);

% From top pane to middle pane (vertical)
\draw[->] (p1.south) -- (p2.north);

% From middle pane to bottom-middle pane (vertical)
\draw[->] (p2.south) -- (p32.north);

% From middle pane to bottom-right pane (diagonal)
\draw[->] (p2.south east) -- (p33.north west);

\end{tikzpicture}
\caption{Centered training example (top), adversarial perturbation only for AT (middle), and three loss formulations (bottom). Arrows are drawn edge-to-edge between panes.}
\label{fig:atat-centered-edge-arrows}
\end{figure}


==> dareDEVALII/Sections/PLAINTEXT_FOR_OPENREVIEW.tex <==
%
%  PLACEHOLDER ABSTRACT
%In this paper, we show that the prevailing view that memorization drives training data exposure to reconstruction attacks is incomplete. We find that extensive exposure can persist without rote memorization, driven instead by a tunable connection to robustness. 
%We provide  evidence that privacy arises from generalizable but imperceptible features. We further show that recent privacy defenses obtain their privacy improvements by unintentionally shifting models toward such features. We leverage this mechanism to introduce, a training regime that intentionally learns such features to obtain both superior reconstruction defense \emph{and} higher accuracy than state-of-the-art defenses. Our results revise the prevailing understanding of training data exposure and reveal a new tradeoff.
%
%
\begin{abstract}
In this paper, we show that the prevailing view that information dependency (including rote memorization) drives training data exposure to image reconstruction attacks is incomplete.
We find that extensive exposure can persist without rote memorization, driven instead by a tunable connection to adversarial robustness.  We begin by presenting three surprising results: (1) recent defenses that inhibit reconstruction by Model Inversion Attacks (MIAs), which evaluate leakage under an idealized attacker, do *not* reduce standard measures of information dependency (HSIC); (2) models that maximally memorize their training datasets remain robust to MIA reconstruction; and (3) models trained without seeing 97\% of the training pixels, where recent information-theoretic bounds give arbitrarily strong privacy guarantees under standard assumptions, can still be largely reconstructed by MIA. To explain these findings, we provide causal evidence that privacy under MIA arises from what the adversarial examples literature calls ``non-robust'' features (generalizable but imperceptible and unstable features). We further show that recent MIA defenses obtain their privacy improvements by unintentionally shifting models toward such features. We leverage this mechanism to introduce Anti-Adversarial Training (AT-AT), a training regime that intentionally learns non-robust features to obtain both superior reconstruction defense and higher accuracy than state-of-the-art defenses. Our results revise the prevailing understanding of training data exposure and reveal a new privacy-robustness tradeoff.
\end{abstract}

==> dareDEVALII/Sections/SAVE_FORLATER_memorization_definition.tex <==
\section{The meaning of memorization in deep learning}\label{app:memorization-meaning}

While the MIA defenses that attempt to increase privacy generically \citep{ho_model_2024,dibbo_improving_2024,peng_bilateral_2022, wang_improving_2020} do not explicitly state that their methods are connected to memorization, we observe that their focus on dependency of individual examples aligns with much of the collective intuitions for what neural network memorization really is. While many works have proposed specific mathematical definitions of memorization based on concepts such as \emph{exposure}  \cite{carlini_secret_2019} and \emph{influence} \citep{yeom_privacy_2018}, it is nonetheless very common for memorization to be referred to in a more intuitive sense of learning 'too much' or 'irrelevant' info about the training data, such as the following:
\begin{enumerate}
    \item The highly influential Deep Learning textbook \citep{goodfellow_deep_2016} mentions memorization briefly without providing a concrete definition, claiming that ``... [m]odels with high capacity can overfit by memorizing properties of the training set that do not serve them well on the test set."
    \item \citet{zhang_understanding_2017} argue through their permuted-labels experiment that their model has fully memorized the training data, without providing a specific definition of memorization.
    \item \citet{arpit_closer_2017} study memorization in classifiers, remarking the following: ``Like [\cite{zhang_understanding_2017}], we do not formally define memorization; rather, we investigate this intuitive notion of memorization by training DNNs to fit random data... [w]e operationalize the definition of 'memorization' as the behavior exhibited by DNNs trained on noise."
    \item \citet{song_machine_2017} also use memorization to mean the `encoding' of irrelevant information in the training data, without giving a precise definition. Unlike the above works, they show that this type of memorization can exist even when the model has strong generalizability.
\end{enumerate}

\citet{song_machine_2017} provide a particularly interesting note: ``Detecting that a training algorithm is attempting to memorize sensitive data within the model is not straightforward because... there are many techniques and places for encoding this information: directly in the model parameters, by applying a malicious regularizer, or by augmenting the training data with specially crafted inputs." Through this lens, it is clear that each of the strategies of MID, BiDO, TL-DMI, and SCA seek to reduce `memorization', as the word is typically understood by the broader machine learning community.

==> dareDEVALII/Sections/algorithm-AT-AT-wallpaperOVERLAY.tex <==
%
%
%
\begin{AlgWithBGfaint}{dareDEVALII/Figures/ATATiconV4.png}
\begin{algorithm}[H]
\caption*{\textbf{Anti-Adversarial Training (AT-AT)~\ATATicon}} % NOTE caption vs caption* asterisk
%
\addcontentsline{loa}{algorithm}{AT-AT}
%
\begin{algorithmic}
    	\INPUT  Data $\mathcal{D}$,   Model $\mathcal{M}(\theta,  \lambda)$ \\
        %
    	\STATE \textbf{for} $(x,y) \in \mathcal{D}$ \textbf{do} \\
        %
        % \STATE \ \ \ \ $t \overset{uar}{\sim} [C]$
        \STATE \ \ \ \ $y' \sim \text{Uniform}(C\setminus y)$\\ % {y} denotes a set of y's rather than a singleton element y in combinatorics/optimization
        %
        \STATE \ \ \ \ $x_{\text{adv}} \gets \hspace{-0.5em} \min\limits_{||x'\text{-}x||_{\infty}\le\varepsilon} \mathcal{L}_\mathcal{M} (x',y')$  \# \textsc{PGD} \\
        %
        \STATE \ \ \ \ \ $\mathcal{L} \gets %
        \underbrace{\mathcal{L}_\mathcal{M} (x,y)}_{\text{vanilla}} \   +  \ \lambda  \cdot \underbrace{\mathcal{L}_\mathcal{M} (x_{\text{adv}}, y')}_{\text{anti-adv.}}  $ \\
        %
        \STATE \ \ \ \ \ $\theta \gets \theta - \alpha \nabla_\theta \mathcal{L}$
        %
        \STATE \textbf{return} \ \   $\mathcal{M}$
        %
  \end{algorithmic}
  \label{alg:ATAT}
\end{algorithm}
\end{AlgWithBGfaint}

==> dareDEVALII/Sections/algorithm-AT-AT.tex <==
%
\begin{algorithm}[H] % H == "force it to be right here"
\caption*{\textbf{Anti-Adversarial Training (AT-AT)~\ATATicon}} % NOTE caption vs caption* asterisk
%
\addcontentsline{loa}{algorithm}{AT-AT}
%
\begin{algorithmic}
    	\INPUT  Data $\mathcal{D}$,   Model $\mathcal{M}(\theta,  \lambda)$ \\
        %
    	\STATE \textbf{for} $(x,y) \in \mathcal{D}$ \textbf{do} \\
        %
        % \STATE \ \ \ \ $t \overset{uar}{\sim} [C]$
        \STATE \ \ \ \ $y' \sim \text{Uniform}(C\setminus y)$\\ % {y} denotes a set of y's rather than a singleton element y in combinatorics/optimization
        %
        \STATE \ \ \ \ $x_{\text{adv}} \gets \min\limits_{||x'\text{-}x||_{\infty}\le\varepsilon} \mathcal{L}_\mathcal{M} (x',y')$  \# \textsc{PGD} \\
        %
        \STATE \ \ \ \ \ $\mathcal{L} \gets %
        \underbrace{\mathcal{L}_\mathcal{M} (x,y)}_{\text{vanilla}} \  \ + \ \ \lambda  \cdot \underbrace{\mathcal{L}_\mathcal{M} (x_{\text{adv}}, y')}_{\text{anti-adv.}}  $ \\
        %
        \STATE \ \ \ \ \ $\theta \gets \theta - \alpha \nabla_\theta \mathcal{L}$
        %
        \STATE \textbf{return} \ \   $\mathcal{M}$
        %
  \end{algorithmic}
  % \label{alg:ATAT} % Shailen: commenting out so that overlay AT-AT algo label works
\end{algorithm}



==> dareDEVALII/Sections/bckup2.tex <==

\section{Introduction}


A foundational goal of contemporary machine learning is to learn \emph{generalizable} model parameters from the training data without \emph{exposing} training data examples to leakage. However, it is well-known that virtually all modern architectures obtain generalizable performance only at the cost of encoding a substantial amount of sensitive information about their training examples.  



\textbf{Understanding this training data encoding and exposure is expected to be a key to next-generation model performance.} % Venn diagram 
A variety of recent work shows that this tradeoff is deeply connected to the efficiency of current training regimes and the performance of contemporary architectures.

For example, in the context of novel generative paradigms such as diffusion models, influential recent work has conjectured that stronger performance may require \emph{more} training data exposure, up to and including rote memorization of the training set \citep[e.g.,][]{carlini2023extracting, c.f., shah2025memorization}. 
\textcolor{orange}{and LLM's? https://arxiv.org/abs/2205.10770}
\textcolor{blue}{and Apple research generic ML stuff: https://dl.acm.org/doi/pdf/10.1145/3406325.3451131}
\textcolor {green}{and self supervised learning: https://arxiv.org/pdf/2401.12233}
\textcolor{red}{maybe: https://arxiv.org/html/2507.04782v1}
\textcolor{blue}{rasmus's google 2021 paper: https://arxiv.org/abs/1906.05271}
These conjectures stand in contrast to classic ML research on overfitting, where backpropagating to capture idiosyncratic, ungeneralizable training data details is a well-studied as a performance pitfall. Reconciling these perspectives is key to understanding the mechanics that will shape the next generation of high-performance models.


 \textbf{Training data exposure undermines privacy in ML deployments.}
Training data exposure also underlies a rapidly expanding class of practical privacy attacks that reconstruct private training data from real-world machine learning deployments simply by querying models or inspecting their parameters. Recent variants of training data attacks apply not only to CNN's, but also to LLM's, diffusion models, multimodal models, etc. \textcolor{red}{[Cite membership inference, attribute inference, carlini's extraction attacks on text LLM's and on stable diffusion].}




\textbf{Model inversion attacks (MIA's) probe and exploit training data exposure.} 
In particular, model inversion attacks (MIA's) have become a mainstream tool for studying and evaluating training data exposure. Unlike more conservative attacks that merely test for the presence of some exposed training examples, MIAs test the degree to which a powerful attacker armed with white-box model access and significant computational and data resources can reconstruct information from the training examples. While early MIA's applied SGD to directly optimize reconstructions of individual training examples \citep{fredrikson2015model}, contemporary MIA's leverage state-of-the-art pretrained models to attempt to infer the full set of class-level characteristics for each class in the training data. 


\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}



However, while MIA's lower-bound the extent to which training data information is vulnerable to reconstruction, they do not explain what aspect of trained models encodes this vulnerability, or how to prevent it. This raises a fundamental question:


\begingroup
\addtolength\leftmargini{-0.15in} % shrink quote margin
\begin{quote}
%\vspace{-2mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null\\[-2.5mm]
\begin{center}
\vspace{-5mm}
 \textit{What properties of learned representations encode vulnerability to training data leakage and reconstruction, and how can they be controlled?}
 \vspace{-1mm}
\end{center}
\vspace{-2.5mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null
%\vspace{-2mm}
\end{quote}
\endgroup


\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}

\textbf{The prevailing `training data exposure = memorization' theory.} 


\textbf{State-of-the-art defenses theorize that MIA's reveal and exploit memorization in the form of direct data-to-model dependencies.}
An influential recent line of algorithms have obtained practically performant defenses against training data exposure/MIA, and it is widely believed that their practical performance can be attributed to their shared theoretic hypothesis that MIA vulnerability arises from direct and excessive informational/correlative dependency between training inputs and the model’s internal representations or outputs \citep{wang_improving_2020, peng_bilateral_2022, ho_model_nodate}. 

To mitigate this hypothesized dependency, Mutual Information Defense (MID) \citep{wang_improving_2020} introduces a regularizer that reduces mutual information between the training examples and intermediate feature representations, arguing that this ``limit[s] the redundant information about the model input contained in the prediction" so that MIA's cannot ``exploit this correlation.'' Building on this idea, the current state-of-the-art Bilateral Dependency Optimizer (BiDO) algorithm \citep{peng_bilateral_2022} penalizes a kernel-based informational dependency measure (HSIC) between training examples and intermediate embeddings, arguing that this ``limits redundant information propagated from the inputs to the latent representations that can be exploited by the [MIA] adversary.'' 

Similarly, the recent and highly performant TL-DMI approach \citep{ho_model_nodate} advances a ``main hypothesis...that a model with fewer parameters encoding sensitive information from private training dataset'' contains less memorization vulnerable to MIA. This hypothesis is credited with the impressive practical performance of TL-DMI---a transfer-learning based approach that uses the training examples only for fine-tuning later layers of a pre-trained/public model.


The same hypothesis appears again in \textsc{SCA} \citep{dibbo_improving_2024}, which argues that the relevant MIA training data reconstruction vulnerability is reduced by directly “jettison[ing] unnecessary private information in the input image,” e.g. by sparse-coding training images before they are seen by the model, and by also “jettison[ing]…unnecessary private information from downstream layers” to attempt to preclude high-fidelity memorization of the inputs, rather than disincentivizing it via the loss function as in \citep{}\textcolor{red}{MID, BIDO}.

In sum, state-of-the-art defenses advance the theoretic argument that they obtain their practical performance against MIA by reducing memorization defined as informational dependency between training examples and the target model's latent representations/outputs.


\textcolor{red}{[DP-SGD Goodfellow $\rightarrow$ Hayes? Steinke? Guo on encodings? FAIR paper?]}



\textbf{Our contribution I: \  Challenging the theoretic bases of contemporary memorization/MIA defenses.}

In this paper, we challenge this foundational hypothesis. Specifically, we motivate our algorithm by first presenting three surprising experiments that indicate that the memorization view is inadequate to explain MIA reconstruction vulnerability:

\begin{enumerate}
\item \textbf{Reconstruction defenses do not reduce memorization metrics.} First, we show that contemporary defenses that are widely believed to prevent memorization/MIA by reducing training-data-to-model dependency %

 \emph{do  not in fact reduce this dependency}, and may in fact increase it, in some cases even according to their own metrics.
%
\item  \textbf{Low memorization can yield extensive reconstruction.} We construct a novel mask-based model that decimates memorization qua input–output dependency by training without allowing the model to see $98\%$ of input pixels (such that each training example is bounded below 2\% memorization in the worst-case), and we show it remains \emph{highly vulnerable} to extensive MIA reconstruction.
\textcolor{red}{Maybe consider adding FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we crush this hope with our DropLayer mask experiment that is an ineffective defense BECAUSE PPA/IFGMI use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it?}
%

\item \textbf{High memorization can yield low reconstruction.} Conversely, we show that models that perfectly memorize their training dataset are \emph{less vulnerable} to MIA reconstruction than state-of-the-art MIA defenses.
%
\end{enumerate}

In sum, our experiments show that the main theoretic approach in memorization/MIA defense, while well-motivated, is incomplete; state-of-the-art memorization/MIA defenses, we argue, obtain their impressive performance by a different theoretic mechanism.


\textbf{Our contribution II: The privacy-robustness feature tradeoff.}

We uncover a previously unknown mechanism that directly links training data exposure vulnerabilities to the well-studied robust–non-robust feature tradeoff from adversarial robustness. To probe this phenomenon, we conduct the first systematic evaluation of the robustness of memorization/MIA defenses to adversarial examples. Our analysis reveals that state-of-the-art privacy defenses do not primarily protect against reconstruction by reducing direct data–model dependency, as widely assumed. Instead, they operate by reshaping the learned feature basis. Specifically, they protect privacy by unintentionally suppressing reliance on ``robust features'' (i.e., generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics), and in some cases, replacing them with ``non-robust features'' (i.e., features that generalize well but are imperceptible to humans and unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}. This shift yields a tradeoff: suppressing robust features strips semantically meaningful information from the model but degrades accuracy, while replacing robust features with non-robust features recovers accuracy at the cost of brittleness, leaving models vulnerable to adversarial examples. Although robust–non-robust feature reliance is heavily studied in adversarial robustness, our work is the first to show its central role in training data privacy vulnerabilities. 



 \textcolor{red}{[make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with Adversarial Examples]}]




\textbf{Our contribution III: \ \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining \\(\textsc{AT-AT}~\ATATicon) for superior privacy/MIA defense.}

If recent memorization/MIA defenses work by unintentionally `nonrobustifying' the model's feature space, then it stands to reason that we could obtain superior defense performance by deliberately exploiting this mechanism. 
%
To accomplish this, we introduce  \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining (\textsc{AT-AT}~\ATATicon), a novel class of memorization/MIA defenses that balance model accuracy with gradient steps that reverse standard adversarial training.  
Rather than promoting robustness to adversarial perturbations, \textsc{AT-AT} applies targeted gradient updates that suppress reliance on robust features, compelling the model to instead learn non-robust—but still generalizable—features that are semantically meaningless to humans and thereby hinder visual reconstruction under MIA.




We show that our anti-adversarial approach outperforms baselines in terms of \emph{both} model accuracy and standard MIA defense metrics \textcolor{red}{[PLACEHOLDER for specific outperformance factors or something impressive]} across various standard CNN architectures, datasets, and reconstruction metrics. As with other defenses, this performance comes at the cost of increased vulnerability to adversarial examples. However, in our case, this vulnerability cost is a tunable parameter, offering a new design axis for privacy-robust models.



\textbf{Privacy implications}
Our results indicate that learning too many descriptive features is a privacy vulnerability distinct from anything that can reasonably be called “memorization.” In this view, a model does not leak information solely like a camera that stores pixel-perfect images of its training data, but also like a crime eyewitness: even without taking pictures, the witness can recall and describe enough private details for a skilled sketch artist armed with prior information about faces (i.e., the MIA attacker) to reconstruct a convincing likeness. 


==> dareDEVALII/Sections/conclusion.tex <==
\subsection{Conclusion}

\begin{itemize}
    \item We show a strong connection between adversarial non-robustness and model inversion resilience. By exploiting this, we outperform other state-of-the-art defenses.
    \item Therefore, we propose that future research into other defenses should also perform adversarial attacks to verify that they didn’t achieve model inversion defense simply by being non-robust, thus introducing new security vulnerabilities in the network.
    \item Our non-robust model is meant as a proof-of-concept and should not be used in practice, see appendix for more info
    \item While adversarial robustness is often achieved by `good' models, for various definitions of `good', model inversion robustness is instead often caused by `bad' models. This means that model inversion defense research might not end up achieving one of the goals of defense research described in \citet{carlini_evaluating_2019} about `measuring the progress of machine learning algorithms towards human-level abilities'. The study of adversarial robustness might achieve this goal, but model inversion robustness does not.

    \item Some other potentially-related concepts for future work: Relation between model inversion for facial classification vs. uncovering memorization in generative models; connection between representation inversion and model inversion, potential vulnerability of adversarially robust models to MIAs, metrics that measure the 'volatility' in the loss landscape in some way, whether these results apply to black-box attacks, or the low-res scenario, or split learning scenario
\end{itemize}

==> dareDEVALII/Sections/dependency_bido.tex <==
\subsection{A Closer Look at a Common Dependency Metric}

[commented out sections in the draft that are redundant in the main body of the paper now]

% Below, we show that contemporary model inversion defenses fail to reduce, and sometimes increase, the Hilbert-Schmidt Independency Criterion (HSIC) \cite{hutchison_measuring_2005} between inputs and intermediate embeddings.

\subsubsection{BiDO objective function}

% HSIC is utilized in the objective function of the popular Bilateral Dependency Optimization (BiDO) \cite{peng_bilateral_2022} defense in order to measure dependency between inputs, intermediate embeddings, and outputs. As explained in \cite{peng_bilateral_2022}, HSIC measures the scale of nonlinear dependencies in random variables $X$ and $Y$ as follows: First, nonlinear feature transformations $\phi,\psi$ are created such that $\phi(X)$ and $\psi(Y)$ are members of reproducing kernel Hilbert spaces $\mathcal{F}$ and $\mathcal{G}$, respectively; then, HSIC$(X,Y)$ is computed as the Hilbert-Schmidt norm of the cross-covariance between these features: $$\text{HSIC}(X,Y)=\left \lVert\mathbb{E}[\phi(X)\psi(Y)^\top]-\mathbb{E}[\phi(X)]\mathbb{E}[\psi(Y)]^\top\right\rVert_{HS}^2.$$
Let $X$ and $Y$ be random variables representing the inputs and outputs, respectively, and let $Z_1,\ldots,Z_m$ be intermediate embeddings chosen at $m$ different points from passing $X$ as input to the model (e.g. the outputs of the four major blocks of a ResNet). BiDO then uses the following training objective:
$$\tilde{\mathcal{L}}(\theta)=\mathcal{L}(\theta)+\lambda_x\sum_{j=1}^m\text{HSIC}(X,Z_j)-\lambda_y\sum_{j=1}^m\text{HSIC}(Z_j, Y)$$
where $\mathcal{L}$ is a standard cross-entropy loss, and $\lambda_x,\lambda_y>0$ are hyper-parameters. The second term is intended to minimize dependency between inputs and intermediate embeddings. As for the third term, \citet{peng_bilateral_2022} argue that solely minimizing $\text{HSIC}(X,Z_j)$ would ``\ldots lead to the loss of useful information, so it is necessary to keep the [third] term to make sure $Z_j$ is informative enough of $Y$ as well as to maintain the discriminative nature of the classifier."

% \subsubsection{HSIC is Orthogonal to Model Inversion Robustness}
% In this section, we show that 1) all recent model inversion defenses, including BiDO, fail to decrease HSIC$(X,Z_i)$ for all typically used intermediate embeddings $Z_i$; 2) using sufficiently small values of $\lambda_x$ in the BiDO defense does succeed at decreasing HSIC without compromising model utility, rendering the third term in the BiDO equation unnecessary; 3) Such models with reduced values of HSIC$(X, Z_j)$ are ineffective as defenses against model inversion. \\\\
% To show this, we train ResNet-18 and ResNet-152 models on FaceScrub in [the same setup as above?]. We measure HSIC as an average across the train set; we use the exact implementation of the HSIC calculation used in \cite{peng_bilateral_2022}. We measure model inversion robustness by the top-1 attack accuracy of PPA \cite{struppek_plug_2022} on 75 randomly chosen target classes.

% As Table \ref{tab:hsic-fs-bido-hyp} shows, the models trained with BiDO$(0.1, 0)$, BiDO$(0.01, 0)$, and BiDO$(0.001, 0)$, respectively, succeed in lowering HSIC$(X, Z_j)$ for most values of $j$, but provide no significant advantage over the undefended model against a Plug-and-Play attack.
% shows, while the BiDO models trained with $(\lambda_x, \lambda_y)=(0.05, 0.5)$ obtain moderate success as defenses, they fail to decrease HSIC$(X, Z_j)$ for some values of $j$, actually raising it in some cases, compared to an undefended model. In a similar vein, recent SOTA defenses NegLS and TL-DMI are robust against model inversion while failing to decrease HSIC.


% [transition into droplayer section]


==> dareDEVALII/Sections/intro_mi_defenses.tex <==
\subsection{Introduction: Re-Thinking Model Inversion Defenses}

In the field of adversarial robustness, \citet{carlini_evaluating_2019} describes how while some adversarial defenses seek to be robust against a specific type of adversarial attack, others instead seek to ``generally \textit{be robust}". We believe that this concept is useful to apply to model inversion defenses as well; below, we categorize each of the recent popular model inversion defenses as either \textit{general}, i.e. seeking general model inversion robustness, or \textit{specific}, i.e. disrupting a specific aspect of certain model inversion attacks. In this paper, we study the following question:
\begin{center}
    \textit{What properties of target models create general model inversion robustness?}
\end{center}

[commented out some stuff that's redundant with our current intro]
% In the following sections, we show through a variety of experiments that all of the given explanations for general model inversion defense are fundamentally misguided. In pursuit of a better explanation, we offer the hypothesis that the presence of \textit{adversarially non-robust features} \cite{ilyas_adversarial_2019} has a direct positive impact on model inversion robustness, using the adversarial vulnerability of TL-DMI \cite{ho_model_nodate} as a motivating example. Based on this hypothesis, we then create a novel general model inversion defense, Anti Adversarial Training (Anti-AT); we show through extensive experiments that Anti-AT significantly outperforms all previous general model inversion defenses, as well as many specific model inversion defenses. Our result shines light on a previously-unknown tradeoff between \textit{model inversion} robustness and \textit{adversarial} robustness.

% Our contributions are as follows... 



==> dareDEVALII/Sections/junk.tex <==

% training privacy vulnerability is ascribed to memorization across various SOTA models like LLM, diffusion, classification, etc.

% Memorization can refer to a variety of related concepts but in the context of MI, defenses are trying to minimize the explicit dependency of training data that are “rote encoded” into the model such inputs and embeddings have high joint HSIC, MI, etc.

% In the appendix, we can hide a paragraph of quotes about memorization since some reviewer will certainly attack some aspect of the fact that the concept of memorization is vague, and it’s not clear that a fully memorized model relates to a high HSIC model or something.


\textcolor{purple}{Among the most celebrated results in ML is the finding that adversarial examples are not bugs, but non-robust features \citep{ilyas_adversarial_2019}. In other words, adversarial examples reveal features that are generalizable and discriminatory of the classes we want to learn, but visually imperceptible to humans. Our argument in this paper is that these properties make them ideal instruments for privacy-preserving learning, where our goal is to classify accurately without encoding visually meaningful information that is vulnerable to visual reconstructions.}

\section{Introduction}

\textbf{\textcolor{red}{Rewriting this as it mentions memorization a lot incorrectly}}

A foundational goal of contemporary machine learning is to learn \emph{generalizable} model parameters from the training data. However, it is well-known that virtually all modern architectures obtain generalizable performance only at the cost of encoding and exposing a substantial amount of sensitive information about their training examples.


\textbf{Understanding training data encoding and exposure is a key to next-generation model performance.} % Venn diagram 
A variety of recent research shows that this tradeoff is deeply connected to the performance of contemporary architectures.
For example, influential recent work has conjectured that obtaining stronger performance may require rote memorization of the training set, not only for vanilla CNNs, but also for novel paradigms such as LLM's and diffusion models \citep[e.g.,][]{carlini2023extracting, c.f., shah2025memorization}. 
\textcolor{orange}{and LLM's? https://arxiv.org/abs/2205.10770}
\textcolor{blue}{and Apple research generic ML stuff: https://dl.acm.org/doi/pdf/10.1145/3406325.3451131}
\textcolor {green}{and self supervised learning: https://arxiv.org/pdf/2401.12233}
\textcolor{red}{maybe: https://arxiv.org/html/2507.04782v1}
\textcolor{blue}{rasmus's google 2021 paper: https://arxiv.org/abs/1906.05271}
These conjectures stand in contrast to classic ML research on overfitting, where training to encode idiosyncratic, ungeneralizable training data details is well-studied as a performance pitfall. Reconciling these perspectives is key to understanding the mechanics that will shape the next generation of high-performance models.


 \textbf{Training data exposure undermines privacy in ML deployments.}
Training data encoding and exposure also underlies a rapidly expanding class of practical privacy attacks that reconstruct private training data from real-world machine learning deployments simply by querying models or inspecting their parameters. Recent variants of training data attacks apply not only to CNN's, but also to LLM's, diffusion models, multimodal models, etc. \textcolor{red}{[Cite membership inference, attribute inference, carlini's extraction attacks on text LLM's and on stable diffusion].}




\textbf{Model inversion attacks (MIA's) probe and exploit training data exposure.} 
In particular, model inversion attacks (MIA's) have become a mainstream tool for studying and evaluating training data exposure. Unlike more conservative attacks that merely test for the presence of some exposed training examples, MIAs test the degree to which a powerful attacker armed with white-box model access and significant computational and data resources can reconstruct information from the training examples. While early MIA's applied SGD to directly optimize reconstructions of individual training examples \citep{fredrikson2015model}, contemporary MIA's leverage state-of-the-art pretrained models to attempt to infer the full set of class-level characteristics for each class in the training data. 


\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }


However, while MIA's lower-bound the extent to which training data information is vulnerable to reconstruction, they do not explain what aspect of a model encodes this vulnerability, or how to prevent it. This raises a fundamental question:


\begingroup
\addtolength\leftmargini{-0.15in} % shrink quote margin
\begin{quote}
%\vspace{-2mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null\\[-2.5mm]
\begin{center}
\vspace{-5mm}
 \textit{What properties of learned representations encode vulnerability to training data leakage and reconstruction,\\and how can they be controlled?}
 \vspace{-1mm}
\end{center}
\vspace{-2.5mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null
%\vspace{-2mm}
\end{quote}
\endgroup


% \textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }

\textbf{The prevailing `memorization $\rightarrow$ training data exposure' theory.} 
\textbf{\textcolor{red}{PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER}}


\textbf{Defenses theorize that MIA's reveal and exploit memorization in the form of direct data-to-model dependencies.}
An influential recent line of algorithms have obtained practically performant defenses against training data exposure/MIA, and it is widely believed that their practical performance can be attributed to their shared theoretic hypothesis that MIA vulnerability arises from direct and excessive informational/correlative dependency between training inputs and the model’s internal representations or outputs \citep{wang_improving_2020, peng_bilateral_2022, ho_model_nodate}. 

To mitigate this hypothesized dependency, Mutual Information Defense (MID) \citep{wang_improving_2020} introduces a regularizer that reduces mutual information between the training examples and intermediate feature representations, arguing that this ``limit[s] the redundant information about the model input contained in the prediction" so that MIA's cannot ``exploit this correlation.'' Building on this idea, the current state-of-the-art Bilateral Dependency Optimizer (BiDO) algorithm \citep{peng_bilateral_2022} penalizes a kernel-based informational dependency measure (HSIC) between training examples and intermediate embeddings, arguing that this ``limits redundant information propagated from the inputs to the latent representations that can be exploited by the [MIA] adversary.'' 

Similarly, the recent and highly performant TL-DMI approach \citep{ho_model_nodate} advances a ``main hypothesis...that a model with fewer parameters encoding sensitive information from private training dataset'' contains less memorization vulnerable to MIA. This hypothesis is credited with the impressive practical performance of TL-DMI---a transfer-learning based approach that uses the training examples only for fine-tuning later layers of a pre-trained/public model.


The same hypothesis appears again in \textsc{SCA} \citep{dibbo_improving_2024}, which argues that the relevant MIA training data reconstruction vulnerability is reduced by directly “jettison[ing] unnecessary private information in the input image,” e.g. by sparse-coding training images before they are seen by the model, and by also “jettison[ing]…unnecessary private information from downstream layers” to attempt to preclude high-fidelity memorization of the inputs, rather than disincentivizing it via the loss function as in \citep{}\textcolor{red}{MID, BIDO}.

In sum, state-of-the-art defenses advance the theoretic argument that they obtain their practical performance against MIA by reducing memorization defined as informational dependency between training examples and the target model's latent representations/outputs.


\textcolor{red}{[DP-SGD Goodfellow $\rightarrow$ Hayes? Steinke? Guo on encodings? FAIR paper?]}

\textcolor{orange}{adam should remember to say that these defenses are well-motivated and well-grounded in recent theoretical intuitions...to soften the blow :)}


\textbf{Our contribution I: \  Challenging the theoretic bases of contemporary memorization/MIA defenses.}

In this paper, we challenge this foundational hypothesis. Specifically, we motivate our algorithm by first presenting three surprising experiments that indicate that the memorization dependency view is inadequate to explain MIA reconstruction vulnerability:

\begin{enumerate}
\item \textbf{Reconstruction defenses do not reduce memorization metrics.} First, we show that contemporary defenses that are widely believed to prevent memorization/MIA by reducing training-data-to-model dependency % do not in fact reduce this dependency, and may in fact increase it, even according to their own metrics. 
 \emph{do  not in fact reduce this dependency}, and may in fact increase it, in some cases even according to their own metrics.
%


\item \textbf{High memorization can yield low reconstruction.} We show that models that perfectly memorize their training dataset are \emph{less vulnerable} to MIA reconstruction than state-of-the-art MIA defenses.

\item \textbf{Low memorization can yield extensive reconstruction, contra recent information-theoretic privacy bounds.}
We construct a novel mask-based model that decimates memorization qua input–output dependency by training without allowing the model to see $98\%$ of input pixels (so each training example contains at most $2\%$ of its pixels in the worst case).
Very recent privacy theory allows us to show that these pixels are provably unreconstructable under standard unbiased reconstuction estimator assumptions (via Hammersley-Chapman-Robbins bounds).
Yet in practice, the model remains \emph{highly vulnerable} to extensive MIA reconstruction, revealing that recent bounds do not protect against a salient leakage mode exploited by modern attacks.

\textcolor{red}{Maybe consider adding FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we crush this hope with our DropLayer mask experiment that is an ineffective defense BECAUSE PPA/IFGMI use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it?}
%


%
\end{enumerate}

In sum, our motivating experiments show that the main theoretic approach in memorization/MIA defense is incomplete; state-of-the-art memorization/MIA defenses obtain their impressive performance by a different theoretic mechanism.



\textbf{Our contribution II: The privacy-robustness feature tradeoff.}


To probe these phenomena, we conduct the first systematic evaluation of the robustness of memorization/MIA defenses to adversarial examples. Our analysis reveals that state-of-the-art privacy defenses do not primarily protect against reconstruction by reducing direct data–model dependency, as widely assumed. Instead, they operate by reshaping the learned feature basis. Specifically, they protect privacy by unintentionally suppressing reliance on ``robust features'' (i.e., generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics), and in some cases, replacing them with ``non-robust features'' (i.e., features that generalize well but are imperceptible to humans and unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}. This shift yields a tradeoff: suppressing robust features strips semantically meaningful information from the model but degrades accuracy, while replacing robust features with non-robust features recovers accuracy at the cost of brittleness, leaving models vulnerable to adversarial examples. Although robust–non-robust feature reliance is heavily studied in adversarial robustness, our work is the first to show its central role in training data privacy vulnerabilities. 




%


 \textcolor{red}{[make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with Adversarial Examples]}




\textbf{Our contribution III: \ \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining \\(\textsc{AT-AT}~\ATATicon) for superior privacy/MIA defense.}

If recent privacy/MIA defenses work by unintentionally `nonrobustifying' the model's feature space, then it stands to reason that we could obtain superior defense performance by deliberately exploiting this mechanism. 
%
To accomplish this, we introduce  introduce \textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI), a novel class of memorization/MIA defense training regimes that balance model accuracy with gradient steps that reverse standard adversarial training.  
Rather than promoting robustness to adversarial perturbations, \textsc{AT-AT} applies targeted gradient updates that suppress reliance on robust features, compelling the model to instead learn non-robust—but still generalizable—features that are semantically meaningless to humans and thereby hinder visual reconstruction under MIA.
% "reverse"? maybe something more explicit/clear.


% \textcolor{red}{non-robust features}

We show that our anti-adversarial approach outperforms baselines in terms of \emph{both} model accuracy and standard MIA defense metrics \textcolor{red}{[PLACEHOLDER for specific outperformance factors or something impressive]} across various standard CNN architectures, datasets, and reconstruction metrics. As with other defenses, this performance comes at the cost of increased vulnerability to adversarial examples. However, in our case, this vulnerability cost is a tunable parameter, offering a new design axis for privacy-robust models.




\textbf{Privacy implications}
Our results indicate that learning too many descriptive features is a privacy vulnerability distinct from anything that can reasonably be called “memorization.” In this view, a model does not leak information solely like a camera that stores pixel-perfect images of its training data, but also like a crime eyewitness: even without taking pictures, the witness can recall and describe enough private details for a skilled sketch artist armed with prior information about faces (i.e., the MIA attacker) to reconstruct a convincing likeness. 

\textbf{Implications for private learning.}
This perspective has four implications. First, eliminating rote memorization does not guarantee privacy, as descriptive-feature leakage can persist in its absence. Second, if recent work is correct in suggesting that rote memorization can confer performance benefits, then such benefits may be attainable without incurring all of the privacy risks that memorization is widely assumed to entail. On the other hand, our results suggest that there may be an inherent privacy vulnerability associated with powerful and robust learned representations. As such, `good' models may be inherently privacy compromising, beyond any specific aspects of how they encode data. This intuition is consistent with recent notions that more interpretable/explainable models are less private. 

\textbf{Implications for privacy theory.}
Finally, our results provide intuition regarding why classic DP guarantees are widely regarded as unsuccessful at preventing MIA, since DP degrades by correlated data, and robust features are correlations rather than idiosyncracies of specific training examples. Similarly, they also show that reconstruction attacks violate the assumptions and protections promised by recent privacy bounds.




%Reconstruction vulnerability is present even absent seeing pixels.

\textcolor{red}{THIS MOVES TO EXPERIMENT BASELINES SECTION}
For completeness, we note that another stream of recent defenses in the literature do not seek to address the underlying privacy vulnerability at all, but instead interfere with specific MIA attack implementations (e.g., by making the loss landscape unamenable to gradients taken in the most popular MIA attacks).\textcolor{green}{negLS;RoLSS;}\textcolor{red}{ label smoothing; trapdoor}.





\textcolor{red}{\textbf{FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein} 


\subsection{notes from slack}
\textcolor{purple}{
I think we will need to be explicit as to what we mean by 'memorization'. We need to back up the claims that 1) there is a prevailing view that memorization drives training data exposure; 2) one can reasonably call the approaches of MID, BiDO, and TL-DMI some form of memorization reduction; 3) our DropLayer and Permutation models decrease and increase memorization, respectively.\\\\
%
We argue that memorization is not the whole story for understanding privacy leakage through models, using model inversion attacks as a case study\\\\
%
"By only focusing on memorization, privacy researchers risk failing to defend properly against certain classes of privacy attacks..."\\\\
%
Previous MIA defenses have focused on a data-to-model dependency that intuitively is related to memorization, but we show that this approach is wrong for model inversion, this is not what makes defenses successful\\\\
%
Instead, we propose that MIA defenses focus on adversarially non-robust features... (describe contributions more)\\\\
%
MIA works well on ideal models with powerful learned representations, in some sense these models are easy to 'traverse'\\\\
%
This is similar to the recent papers [cite, cite] that shows that explainable/interpretable models are more privacy leaking\\\\
%
'Ideal models' likely have similar vulnerabilities in other fields, this should continue to be investigated as an orthogonal (or opposing) axis to 'level of memorization'\\\\
%


We can say that defending against model inversion is the antithesis of powerful learned representations and good deep learning practices. 
}

\textbf{Codebase and Replication Materials.} \textcolor{red}{[Maybe include in intro since it's great marketing/we have a great codebase, it will look strong/confident since we are calling ppl out.}



\textbf{Questions for July 28 mtng.} \textcolor{purple}{Do we want to continue with the "available defenses claim to work via dependency reduction but all actually work via shifting models to rely on non-robust features, so we can exploit this deliberately with AT-AT" framing? Or do we want to more conservatively say "[Just] The best defense TL-DMI seems to work via shifting models to rely on non-robust features, and we notice that vanilla adversarial training does the opposite, so let's exploit this to do AT-AT" framing?}


\textbf{Some framing notes from July 28 mtng.} \textcolor{orange}{
Consider the Venn diagram of features that describe Adams (like an Adam class centroid in a perfect GAN) and the features that describe Adam's centroid in a good classifier. The former are descriptive; the latter are descriminative. You can have descriminative features that are a very small subset of the descriptive ones (small Venn overlap). Or maybe descriminative features are just a strict subset. Plug and play paper talks about features that matter to faces.\\
%
By doing non-robust features, we search for features in a small $\epsilon$ ball ergo humans cannot perceive and don't care. In practice, ATTACKS DONT CONVERGE but even if they do, we leak an imperceptible noise.\\\\
%
- HSIC is unrelated. Could be that HSIC doesn't capture the appropriate dependency measure, OR that dependency is just the wrong story. Suppose HSIC is just a bad measure, so then DropLayer should reduce dependency. BUT that doesn't work! So we need a new story. Should leave DropLayer and Permutation OUT of the HSIC table. \\\\
%
ALL Defenses are dropping robust features. Some (TL-DMI) are replacing them with non-robust to make up the accuracy. In the AutoAttack table, the accuracy under adv examples captures this...it either gets the example wrong because it sucks at classifying or because it was vulnerable to a small noise.\\\\
%
Adam: in intro talk less about screwing up gradients. Talk more about non-robust features.\\\\
%
Need to introduce and out-of-scope-ify the Neg-LS and Trap-MID or skip-connection defenses are like gradient masking. Trap-MID appendix is the only place they tried against PPA and it sucked and they had to cherry pick aka fine tune)\\\\
The new story is that dependency-based defenses delete robust features, and either take the concomitant accuracy penalty (BiDO) or replace them with non-robust features (TL-DMI).
}



\textbf{Paper organization.} \textcolor{red}{PLACEHOLDER.}

\section{\textcolor{red}{Preliminaries}} \textcolor{red}{PLACEHOLDER.}
\textbf{Threat model.}  \textcolor{red}{- white box because (1) we care about evaluating memorization in target models, and (2) we want strong defenses that are practically effective under strong adversaries with minimal assumptions.\\-Our experiments focus on vision because it's the central MIA research stream, though we intend to expand this in future work, and we include a codebase designed to facilitate this expansion }


\section{Model inversion attacks}
The objective of model inversion attacks is to generate images representing a class of the dataset that ideally is closely resembling images of the dataset. The success of the attack is determined by the confidence of the target model (AvgConf), the accuracy of an independently trained evaluation model (AttAcc@1 \& AttAcc@5) and the $L^2$ distance between the VGGFace2 embeddings of the generated images and the images of the class. Importantly, the image need not be a perfect reconstruction of any individual image in the training data, but aims to create a class representative images or class centroids. \textcolor{red}{Maybe we can start with a natural language explanation before the math like this, and the metrics can be explained here.}   

Formally, MIA's consider a private training dataset $\mathcal{D}_{priv}=\{x_i,y_i\}_{i=1}^{N}$, where $x_i\in\mathbb{R}^{d_X}$, $y_i\in\{0,1\}^C$, and each $(x_i,y_i)$ are sampled i.i.d. from a joint distribution $\mathbb{P}_{XY}$. Let $T:\mathbb{R}^{d_X}\to\{0,1\}^C$ be a target model trained on $\mathcal{D}_{priv}$ that the adversary wishes to attack. To conduct a model inversion attack, an adversary seeks a new `inverted' model \textcolor{red}{$\hat{\mathcal{I}}_T$ [do we elsewhere denote it by something else? What do the best other ppl use? I like $\hat{\mathcal{I}}_T$ or maybe $\hat{T}'$]} that maps outputs of $T$, such as $T$'s softmax layer or intermediate outputs, back to the corresponding training examples in $\mathcal{D}_{priv}$. The adversary then queries $\hat{\mathcal{I}}_T$ to `predict' $T$'s private training examples. 

\textcolor{red}{note:    The goal in model inversion is to infer the class \emph{centroids} on the data manifold defined on all pixels/features. privacy leakage exists to the extent that these centroids permit reconstruction of features we `care about' (rather than features that are class-descriminative-but not-otherwise-interesting stuff... \ \ The goal of Model Inversion Defense is to build models that infer decision boundaries without leaking information about the training examples via their class centroids, or that are impervious to having their class centroids re-inferred by an attacker.}

Early MIA's trained the inverted model $\hat{\mathcal{I}}_T$ from scratch by using SGD to directly optimize reconstructions of individual training examples \citep{fredrikson2015model}. However, this approach suffers from various optimization complexities when applied to contemporary vision architectures like deep CNN's. Therefore, recent state-of-the-art attacks simplify optimization by adopting an `image prior'---that is, by restricting the search space of training example reconstructions to the image outputs of a domain-relevant GAN, and conducting SGD-based optimization on the GAN's input noise vectors instead of directly on the high-dimensional images' feature space \cite{zhang_secret_2020}. More specifically, GAN-based MIA's optimize a latent noise vector $\hat{z} \in Z$ such that the resultant GAN-generated image is classified as class $c$ maximized confidence by the target model $T$:
%
$$\min_{\hat{z}} \mathcal{L}(T, G, D, \hat{z}, c)$$ 
%
where $\mathcal{L}$ is a standard loss function (e.g. cross-entropy) to maximize the confidence of the GAN-generated image on class $c$,  given pretrained GAN generator $G:Z \to X_{prior}$ and GAN discriminator $D$. Recent attacks on facial recognition classifiers take advantage of pretrained GANs like StyleGAN to perform far more efficient and accurate training data reconstructions \citep{struppek_plug_2022, qiu_closer_2024}. \textcolor{red}{[Mention in the body of the paper that App. \ref{mia-related-work-supp} gives details of SOTA MIA attacks.]}

==> dareDEVALII/Sections/notes.tex <==
\sisetup{table-number-alignment = center, detect-weight, detect-inline-weight = math}
%
\begin{table}[t]
\begin{compacttable}
\centering
\caption{HSIC$(X,Z_j)$ for defenses on FaceScrub (ResNet-152).  PPA \textbf{AttAcc@1} measures reconstruction.}
\setlength{\tabcolsep}{3pt}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}m{0.6cm}l
                S[table-format=1.0]
                S[table-format=1.3]@{}
                S[table-format=2.5]
                S[table-format=2.2]
                S[table-format=2.2]
                S[table-format=2.2]}
\toprule
\textbf{Arch.} & \textbf{Defense} &
\textbf{TestAcc} &
\textbf{AttAcc@1} &
\textbf{HSIC$(X,Z_0)$} &
\textbf{HSIC$(X,Z_1)$} &
\textbf{HSIC$(X,Z_2)$} &
\textbf{HSIC$(X,Z_3)$} \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{ResNet-152}}}
  & NoDef         & 0.958 & 0.882 & 71.66 & 72.32 & 72.72 & 72.72  \\
  & MID      & 0.950 & 0.391 & 71.52 & 72.57 & 72.84 & 61.98  \\
  & BiDO  & 0.928 & 0.780 & 73.68 & 73.68 & 73.68 & 73.63  \\
  & TL-DMI            & 0.911 & 0.190 & 71.73 & 72.52 & 72.93 & 72.58 \\
\cmidrule(lr){2-8}
  & NegLS         & 0.906 & 0.160 & 71.64 & 72.33 & 72.29 & 73.63  \\
  & RoLSS         & 0.886 & 0.474 & 72.09 & 72.30 & 29.69 & 61.92  \\
  & RoLSS\mbox{-}SSF & 0.869 & 0.343 & 71.88 & 72.02 & 32.75 & 64.94  \\
\cmidrule(lr){2-8}
\cmidrule(lr){2-8}
    &  BiDO**     & 0.940 & 0.815 & 2.159 & 1.256 & 9.310 & 71.81 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:hsic-fs-body}
\end{compacttable}
\end{table}

==> dareDEVALII/Sections/old-SEC_Anti-AT_alternative.tex <==
% %
% %
% %
% %
% \section{\underline{A}n\underline{t}i \underline{A}dversarial \underline{T}raining (\textsc{AT-AT)}\huge~\ATATicon}
% To formalize this idea, we introduce Anti-Adversarial Training (AT-AT), a defense that explicitly encourages non-robust feature reliance. Whereas standard adversarial training (AT) rewards models for resisting adversarial perturbations (thus promoting robust features), AT-AT does the opposite: it rewards models for following adversarial perturbations, thereby promoting non-robust—but still predictive—features that are visually imperceptible and unamenable to MIA reconstruction.
% For example, suppose we draw an image $x_{\text{Yoda}}$ of class $y=\text{Yoda}$, and construct a perturbation $\delta_{\text{Luke}}$ that makes $(x_{\text{Yoda}}+\delta_{\text{Luke}})$ map to class Luke. 
% AT rewards the mapping $(x_{\text{Yoda}}+\delta_{\text{Luke}})\mapsto \text{Yoda}$, while AT-AT rewards the opposite mapping $(x_{\text{Yoda}}+\delta_{\text{Luke}})\mapsto \text{Luke}$. 

% \paragraph{Objective.} 
% Because training only on non-robust features degrades accuracy, we combine the standard classification loss with an anti-adversarial loss that rewards non-robust features:

% \begin{align}
% \text{\textbf{AT-AT Objective:}} \quad
% \min_{\theta} \ \mathbb{E}_{(x,y)\sim\mathcal{D}} 
% \Big[ \mathcal{L}(\theta,x,y) \;+\; 
% \lambda \cdot \max_{\delta\in\mathcal{S}} \mathcal{L}(\theta, x+\delta, y') \Big],
% \quad y'\neq y.
% \end{align}

% Here $\mathcal{L}$ is the standard cross-entropy loss, $\delta$ is an $L_1$-bounded perturbation, and $y'$ is a randomly chosen incorrect label. 
% The coefficient $\lambda$ balances standard accuracy against privacy defense. 

% \paragraph{Algorithm.} 
% AT-AT can be optimized similarly to AT. In each SGD step, we sample $(x,y)$ and a random $y'\neq y$, construct an adversarial perturbation $x_{\text{adv}}$ targeted at $y'$, and update parameters with the combined loss:

% \input{dareDEVALII/Sections/algorithm-AT-AT-wallpapered}

% \paragraph{Privacy link.} 
% By explicitly discouraging robust, semantically meaningful features and rewarding non-robust ones, AT-AT limits the semantic information available to MIAs, yielding stronger reconstruction defense while maintaining competitive accuracy.

==> dareDEVALII/Sections/old-abstr.tex <==

%




In this paper, we show that the prevailing view that memorization drives training data exposure to reconstruction attacks is incomplete: extensive exposure can persist without rote memorization, driven instead by a previously unknown but tunable connection to adversarial example vulnerability. % 
We present a surprising set of experiments showing that: (1) recent defenses that reduce reconstruction by Model Inversion Attacks (MIAs) designed to evaluate leakage under an idealized attacker do \emph{not} reduce well-known measures of memorization (the hypothesized driver of their protection); (2) models that perfectly memorize their training dataset are robust to MIA reconstruction; and (3) 
models trained without seeing 98\% of the training data pixels, for which we show that recent information-theoretic privacy results give arbitrarily high bounds against reconstruction under standard assumptions, can be highly vulnerable in practice to (total) MIA training data reconstruction.

To explain these results, we conduct the first systematic evaluation of the robustness of model inversion defenses to adversarial examples.

We find that recent defenses hinder reconstruction in part by unintentionally shifting models away from what are known in the adversarial examples literature as “robust features" and, in some cases, toward ``non-robust features" (i.e., generalizable but imperceptible and unstable features). 

We leverage this property to introduce \textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI), a training regime that tunes this mechanism to obtain both superior reconstruction defense \emph{and} higher accuracy than state-of-the-art defenses. Our results reframe the theory of training data exposure and reveal a new, practically relevant privacy–robustness trade-off. 

==> dareDEVALII/Sections/old2_SEC_INTRO_firstcut.tex <==
\section{ORIGINAL Introduction}
A foundational goal of contemporary machine learning is to learn \emph{generalizable} model parameters from the training data without \emph{memorizing} idiosyncratic or sensitive details that may later be leaked. However, it is well known that virtually all contemporary architectures obtain generalizable performance only at the cost of some training data memorization \textcolor{red}{[Cite a bunch of papers]}. This tradeoff is a key research frontier because it compromises both learning efficiency and practical model privacy.


\textbf{Memorization is a key impediment to more optimal models.}  First, in the era of billion dollar training expenditures, backpropagating to learn idiosyncratic, ungeneralizable training example information reflects a fundamental learning inefficiency that continues to accrue costs when ungeneralizable parameters are called at inference time \textcolor{red}{[Cite a bunch of papers]}.


\textbf{Memorization undermines privacy in ML deployments.}
Second, memorization underlies a rapidly expanding class of practical privacy attacks that reconstruct private training data from real-world machine learning deployments simply by querying models or inspecting their parameters. \textcolor{red}{[Cite membership inference, attribute inference, carlini's extraction attacks on text and on stable diffusion].}


\textbf{Model inversion attacks (MIA's) probe and exploit memorization.} 
In particular, model inversion attacks (MIA's) are a mainstream approach both for studying memorization and for conducting memorization-based privacy attacks on deployed models. Consider a private training dataset $\mathcal{D}_{priv}=\{x_i,y_i\}_{i=1}^{N}$, where $x_i\in\mathbb{R}^{d_X}$, $y_i\in\{0,1\}^C$, and each $(x_i,y_i)$ are sampled i.i.d. from a joint distribution $\mathbb{P}_{XY}$. Let $T:\mathbb{R}^{d_X}\to\{0,1\}^C$ be a target model trained on $\mathcal{D}_{priv}$ that the adversary wishes to attack. To conduct a model inversion attack, an adversary trains a new `inverted' model \textcolor{red}{$\hat{\mathcal{I}}_T$ [do we elsewhere denote it by something else? What do the best other ppl use? I like $\hat{\mathcal{I}}_T$ or maybe $\hat{T}'$]} that maps outputs of $T$, such as $T$'s softmax layer or intermediate outputs, back to the corresponding training examples in $\mathcal{D}_{priv}$. The adversary then queries $\hat{\mathcal{I}}_T$ to `predict' $T$'s private training examples. 

\textcolor{red}{note:    The goal in model inversion is to infer the class \emph{centroids} on the data manifold defined on all pixels/features. privacy leakage exists to the extent that these centroids permit reconstruction of features we `care about' (rather than features that are class-descriminative-but not-otherwise-interesting stuff... \ \ The goal of Model Inversion Defense is to build models that infer decision boundaries without leaking information about the training examples via their class centroids, or that are impervious to having their class centroids re-inferred by an attacker.}

Early MIA's trained the inverted model $\hat{\mathcal{I}}_T$ by using SGD to directly optimize reconstructions of individual training examples \citep{fredrikson2015model}. However, this approach suffers from various optimization complexities when applied to contemporary vision architectures like deep CNN's. Therefore, recent state-of-the-art attacks simplify optimization by adopting an `image prior'---that is, by restricting the search space of training example reconstructions to the image outputs of a domain-relevant GAN, and conducting SGD-based optimization on the GAN's input noise vectors instead of directly on the high-dimensional images' feature space \citep{zhang_secret_2020}. More specifically, GAN-based MIA's optimize a latent noise vector $\hat{z} \in Z$ such that the resultant GAN-generated image is classified as class $c$ maximized confidence by the target model $T$:
%
$$\min_{\hat{z}} \mathcal{L}(T, G, D, \hat{z}, c)$$ 
%
where $\mathcal{L}$ is a standard loss function (e.g. cross-entropy) to maximize the confidence of the GAN-generated image on class $c$,  given pretrained GAN generator $G:Z \to X_{prior}$ and GAN discriminator $D$. Recent attacks on facial recognition classifiers take advantage of pretrained GANs like StyleGAN to perform far more efficient and accurate training data reconstructions \citep{struppek_plug_2022, qiu_closer_2024}. \textcolor{red}{[Mention in the body of the paper that App. \ref{mia-related-work-supp} gives details of SOTA MIA attacks.]}

\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }



%While the success of MIA's demonstrates the existence of memorized training examples in contemporary models, 
While the success of MIA's demonstrates the existence of training data memorization in contemporary models, it does not explain what aspect of trained models encodes the aspects of memorization relevant to generalization or privacy, or how to prevent it. This raises a fundamental question:

\begingroup
\addtolength\leftmargini{-0.15in} % shrink quote margin
\begin{quote}
%\vspace{-2mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null\\[-2.5mm]
\begin{center}
\vspace{-5mm}
 \textit{What exactly \ *is* \ the memorization that impedes generalization and undermines data privacy?}
 \vspace{-1mm}
\end{center}
\vspace{-2.5mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null
%\vspace{-2mm}
\end{quote}
\endgroup


\textbf{Classical privacy frameworks like DP do not explain the `memorization' that MIA's exploit.}
While classical privacy frameworks such as Differential Privacy (DP) \citep{dwork2006differential, dwork2014algorithmic} offer provable guarantees against training example memorization \citep{hayes_bounding_2023}, they do not explain why it arises in contemporary learning settings. DP was designed to protect the privacy of individual training examples while releasing parameters that characterize in-sample group-level statistics, not parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning). As a result, the very high computational and accuracy costs of adding DP-based protections may be unnecessary to address the training data memorization problem, and these techniques are generally not used to address memorization in large-scale learning applications.

\textcolor{red}{\textbf{FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein} have recent bounds that also use noise and try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we crush this hope with our DropLayer mask and PPA/IFGMI use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it? Or below?}



\textbf{State-of-the-art defenses theorize that the `memorization' MIA's exploit is a data-to-model dependency.}
An influential recent line of algorithms have obtained practically performant defenses against memorization/MIA, and argued that their practical performance can be attributed to their shared theoretic hypothesis that MIA vulnerability arises from excessive informational/correlative dependency between training inputs and the model’s internal representations or outputs \citep{wang_improving_2020, peng_bilateral_2022, ho_model_nodate}. 

To mitigate this hypothesized dependency, Mutual Information Defense (MID) \citep{wang_improving_2020} introduces a regularizer that reduces mutual information between the training examples and intermediate feature representations, arguing that this ``limit[s] the redundant information about the model input contained in the prediction" so that MIA's cannot ``exploit this correlation.'' Building on this idea, the current state-of-the-art Bilateral Dependency Optimizer (BiDO) algorithm \citep{peng_bilateral_2022} penalizes a kernel-based informational dependency measure (HSIC) between training examples and intermediate embeddings, arguing that this ``limits redundant information propagated from the inputs to the latent representations that can be exploited by the [MIA] adversary.'' 

Similarly, the recent and highly performant TL-DMI approach \citep{ho_model_nodate} advances a ``main hypothesis...that a model with fewer parameters encoding sensitive information from private training dataset'' contains less memorization vulnerable to MIA. This hypothesis is credited with the impressive practical performance of TL-DMI---a transfer-learning based approach that uses the training examples only for fine-tuning later layers of a pre-trained/public model.

The same hypothesis appears again in \textsc{SCA} \citep{dibbo_improving_2024}, which argues that the relevant memorization is reduced by ``control[ling] the amount of irrelevant private information encoded in a model's intermediate representations'', e.g., via sparse coding.

In sum, state-of-the-art defenses advance the theoretical argument that they obtain their practical performance against MIA by reducing memorization defined as informational dependency between training examples and the target model's latent representations/outputs.


\textcolor{red}{[DP-SGD Goodfellow $\rightarrow$ Hayes? Steinke? Guo on encodings? FAIR paper?]}



\textbf{Our contribution I: \  Challenging the theoretic bases of contemporary memorization/MIA defenses.}

In this paper, we challenge this foundational theoretic hypothesis.

\begin{enumerate}
\item First, we show that contemporary defenses that claim to prevent memorization/ MIA by reducing training-data-to-model dependency % do not in fact reduce this dependency, and may in fact increase it, even according to their own metrics. 
 \emph{do  not in fact reduce this dependency}, and may in fact increase it, in some cases even according to their own metrics.
%
\item  We construct a novel mask-based model that decimates input–output dependency by deleting $98\%$ of input pixels, and show it remains \emph{highly vulnerable} to MIA.
\textcolor{red}{Maybe consider adding FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we crush this hope with our DropLayer mask experiment that is an ineffective defense BECAUSE PPA/IFGMI use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it?}
%
\item Conversely, we show that a model that is said to perfectly memorize its training dataset is \emph{less} vulnerable to MIA than these state-of-the-art defenses.




\end{enumerate}

In sum, our experiments show that the main theoretic approach in memorization/MIA defense, while well-motivated, is incomplete; state-of-the-art memorization/MIA defenses, we argue, obtain their impressive performance by a different theoretic mechanism.

\textbf{Our contribution II:\\ The Invertability--Adversarial-Example tradeoff.}
 
 We probe these counterintuitive findings and discover a surprising result: 
 %recent defenses against inversion attacks actually work in part by unintentionally encouraging models to rely on what are elsewhere canonically known as “non-robust” features in the context of research on adversarial examples---that is, 
 recent defenses against inversion attacks actually work in part by unintentionally encouraging models to rely on what are elsewhere canonically known as “non-robust” features in the context of research on adversarial examples---that is, features that are generalizable, but imperceptible to humans and unstable under perturbation \citep{ilyas_adversarial_2019}\textcolor{red}{[Cite Ilya 2019, 2016, szegedy intriguing 2013, and the most influential follow-up papers from after Ilya 2019]}. “Non-robust” features are extremely well-studied in the context of adversarial examples and model robustness, but they are not known to be fundamentally connected to memorization/MIA.


% This shift disrupts gradient-based MIA attacks (which now face a fractured loss landscape), but it comes at a cost: the resulting `defended' models are substantially more vulnerable to adversarial examples. We provide the first systematic evaluation of adversarial robustness across MIA defenses, revealing this overlooked tradeoff.

To demonstrate this phenomenon, we conduct the first systematic evaluation of the robustness of memorization/MIA defenses to adversarial examples. 
 By unintentionally promoting this shift, MIA defenses disrupt gradient-based MIA attacks (which now face a fractured loss landscape), \textcolor{red}{[will be revised per July 24 mtng] and also reduce models' reliance on "robust features" that humans find visually/semantically meaningful, and that are captured in MIA reconstruction similarity metrics. This means that dependency-based MIA defenses obtain their performance at a previously overlooked cost: MIA defenses cause models to become far more vulnerable to adversarial examples.}


 \textcolor{red}{[make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with Adversarial Examples]}]


% To probe these counterintuitive results, we analyze the resulting models’ feature space geometry. Our findings suggest that instead of working by reducing training data dependency, recent defenses unintentionally work by “unsmoothing” the target model's feature space, forcing MIA attack gradients to traverse a volatile and brittle loss landscape reminiscent of overfitting.


\textbf{Our contribution III: \ \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining \\(\textsc{AT-AT}~\ATATicon) for superior memorization/MIA defense.}

If recent memorization/MIA defenses work by unintentionally `nonrobustifying' the model's feature space, then it stands to reason that we could obtain superior defense performance by deliberately exploiting this mechanism. To accomplish this, we design a novel class of memorization/MIA defenses that balance model accuracy with gradient steps that reverse standard adversarial training designed to promote robustness to adversarial examples. 
% "reverse"? maybe something more explicit/clear.
This simple technique allows us to deliberately compel models to learn non-robust-but-generalizable features that are semantically meaningless to humans (and thus limit visual reconstruction similarity under MIA), but that generalize as well as vanilla CNNs' features.

\textcolor{red}{non-robust features}

\textcolor{orange}{We call our approach \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining (\textsc{AT-AT}~\ATATicon)}

We show that our anti-adversarial approach outperforms baselines in terms of both model accuracy and standard MIA defense metrics \textcolor{red}{[PLACEHOLDER for specific outperformance factors or something impressive]} across various standard CNN architectures, datasets, and reconstruction metrics. As with other defenses, this performance comes at the cost of increased vulnerability to adversarial examples. However, in our case, this vulnerability cost is a tunable parameter, offering a new design axis for privacy-robust models.




\textbf{Codebase and Replication Materials.} \textcolor{red}{[Maybe include in intro since it's great marketing/we have a great codebase, it will look strong/confident since we are calling ppl out.}



\textbf{Questions for July 28 mtng.} \textcolor{purple}{Do we want to continue with the "available defenses claim to work via dependency reduction but all actually work via shifting models to rely on non-robust features, so we can exploit this deliberately with AT-AT" framing? Or do we want to more conservatively say "[Just] The best defense TL-DMI seems to work via shifting models to rely on non-robust features, and we notice that vanilla adversarial training does the opposite, so let's exploit this to do AT-AT" framing?}


\textbf{Some framing notes from July 28 mtng.} \textcolor{orange}{
Consider the Venn diagram of features that describe Adams (like an Adam class centroid in a perfect GAN) and the features that describe Adam's centroid in a good classifier. The former are descriptive; the latter are descriminative. You can have descriminative features that are a very small subset of the descriptive ones (small Venn overlap). Or maybe descriminative features are just a strict subset. Plug and play paper talks about features that matter to faces.\\
%
By doing non-robust features, we search for features in a small $\epsilon$ ball ergo humans cannot perceive and don't care. In practice, ATTACKS DONT CONVERGE but even if they do, we leak an imperceptible noise.\\\\
%
- HSIC is unrelated. Could be that HSIC doesn't capture the appropriate dependency measure, OR that dependency is just the wrong story. Suppose HSIC is just a bad measure, so then DropLayer should reduce dependency. BUT that doesn't work! So we need a new story. Should leave DropLayer and Permutation OUT of the HSIC table. \\\\
%
ALL Defenses are dropping robust features. Some (TL-DMI) are replacing them with non-robust to make up the accuracy. In the AutoAttack table, the accuracy under adv examples captures this...it either gets the example wrong because it sucks at classifying or because it was vulnerable to a small noise.\\\\
%
Adam: in intro talk less about screwing up gradients. Talk more about non-robust features.\\\\
%
Need to introduce and out-of-scope-ify the Neg-LS and Trap-MID or skip-connection defenses are like gradient masking. Trap-MID appendix is the only place they tried against PPA and it sucked and they had to cherry pick aka fine tune)\\\\
The new story is that dependency-based defenses delete robust features, and either take the concomitant accuracy penalty (BiDO) or replace them with non-robust features (TL-DMI).
}



\textbf{Paper organization.} \textcolor{red}{PLACEHOLDER.}

\section{\textcolor{red}{Preliminaries}} \textcolor{red}{PLACEHOLDER.}
\textbf{Threat model.}  \textcolor{red}{- white box because (1) we care about evaluating memorization in target models, and (2) we want strong defenses that are practically effective under strong adversaries with minimal assumptions.\\-Our experiments focus on vision because it's the central MIA research stream, though we intend to expand this in future work, and we include a codebase designed to facilitate this expansion }


% \textcolor{purple}{
% \subsection{Related Work: Model Inversion Defenses}
% \subsubsection{General Model Inversion Defenses}
% All previous model inversion defenses that argue for general robustness have focused on limiting the information leakage from the training data into the model. MID \cite{wang_improving_2020} minimizes an approximation to mutual information between inputs and embeddings calculated using variational methods, arguing that since ``[model inversion] adversaries exploit the correlation between the model input and output for successful attacks, our idea for the defense is to limit the redundant information about the model input contained in the prediction". In place of mutual information, BiDO \cite{peng_bilateral_2022} instead seeks to minimize a kernel-based dependency measure between input and embedding while adding a second regularizer term that maximizes the dependency between embedding and output; the BiDO authors claim that this approach `` limits redundant information propagated from the inputs to the latent representations which can be exploited by the adversary" \cite{peng_bilateral_2022}. More recently, TL-DMI \cite{ho_model_nodate} freezes the first few layers of the pre-trained target model when fine-tuning on $\mathcal{D}_{priv}$, seeking to ``limit the number of layers encoding sensitive information" from $\mathcal{D}_{priv}$. SCA \cite{dibbo_improving_2024} intersperses sparse coding layers into the target model in order to ``control the amount of irrelevant private information encoded in a model's intermediate representations".
% %
% %
% %
\subsubsection{Specific Model Inversion Defenses}
We have Neg-LS and Skip Connections but we are missing TRAP-MID. Probably beats us. Can be combined. \textbf{}
\textcolor{blue}{Other model inversion defenses have instead more directly `disrupted' the MIA optimization process in a specific way. RoLSS and its variants \citep{koh_vulnerability_2024} remove or weaken the target model's skip connections to impede gradient flow during attack optimization. NegLS \citep{struppek_be_2024} employs negative label smoothing to make the target model consistently overconfident in its predictions, taking advantage of the reliance of most MIAs on target model confidence scores. Trap-MID \citep{liu_trap-mid_2024} uses strategies from backdoor attacks to build `trapdoors' during training to mislead the MIA optimization process.}
% %
% %
% %
% \subsubsection{Connections between Adversarial Examples and Model Inversion}
% Cite membership inference/adv. vulnerability paper, MIAs that use adversarial examples, ... this is how what we're doing is different...
% }





% \textcolor{orange}{
% \subsection{Dependency is Unrelated to Model Inversion Robustness}
% %
% %
% \subsubsection{Bilateral Dependency Optimization}
% Based on the two above experiments in apparent contradiction with the intuitions used to support BiDO and TL, we investigate both BiDO and TL further.
% Bilateral Dependency Optimization (BiDO) \cite{peng_bilateral_2022} is a popular recent model inversion defense that seeks to minimize the dependency between the inputs and intermediate embeddings during training. To quantify this dependency, BiDO uses an approximation to the Hilbert-Schmidt Independency Criterion (HSIC) . As explained in \cite{peng_bilateral_2022}, [explain how HSIC works]. The BiDO training objective is then
% $$\tilde{\mathcal{L}}(\theta)=\mathcal{L}(\theta)+\lambda_x\sum_{j=1}^M\text{HSIC}(X,Z_j)-\lambda_y\sum_{j=1}^M\text{HSIC}(Z_j, Y)$$
% where [define the normal loss, define the symbols].
% %
% %
% \subsubsection{BiDO is flawed and ineffective}
% In this section, we show that 1) BiDO, in its most used form, fails to decrease HSIC$(X,Z_i)$ for all typically used intermediate embeddings $Z_i$; 2) sufficiently small values of $\lambda_x$ do succeed at decreasing HSIC without compromising model utility, rendering the HSIC$(Z_j,Y)$ term in the above equation unnecessary; 3) Such models with reduced values of HSIC$(X, Z_j)$ are ineffective as defenses against model inversion. \\\\
% To show this, we train ResNet-18 and ResNet-152 models on FaceScrub in [the same setup as above?]. As Table \ref{table:hsic-r18} shows, while the BiDO models trained with $(\lambda_x, \lambda_y)=(0.05, 0.5)$ obtain moderate success as defenses, they fail to decrease HSIC$(X, Z_j)$ for some values of $j$, actually raising it in some cases, compared to an undefended model. Conversely, the models trained with BiDO$(0.1, 0)$, BiDO$(0.01, 0)$, and BiDO$(0.001, 0)$, respectively, succeed in lowering HSIC$(X, Z_j)$ for most values of $j$, but provide no significant advantage over the undefended model against a Plug-and-Play attack. \\\\
% In pursuit of a better explanation for the causes of general model inversion robustness, we present our hypothesis that \textit{adversarially non-robust features} \cite{ilyas_adversarial_2019} play an essential role in ensuring model inversion robustness. Section \ref{related_work_non_robust} briefly details some history and preliminaries for our following discussion; section \ref{related_work_adversarial} describes our experimental setup for calculating adversarial robustness and shows that TL-DMI \cite{ho_model_nodate} is adversarially vulnerable. The following section then introduces our own defense, Anti-AT...
% }










% @inproceedings{guo2022bounding,
%   title={Bounding training data reconstruction in private (deep) learning},
%   author={Guo, Chuan and Karrer, Brian and Chaudhuri, Kamalika and Van der Maaten, Laurens},
%   booktitle={International Conference on Machine Learning},
%   pages={8056--8071},
%   year={2022},
%   organization={PMLR}
% }

% @inproceedings{dwork2006differential,
%   title={Differential privacy},
%   author={Dwork, Cynthia},
%   booktitle={International colloquium on automata, languages, and programming},
%   pages={1--12},
%   year={2006},
%   organization={Springer}
% }

% @article{dwork2014algorithmic,
%   title={The algorithmic foundations of differential privacy},
%   author={Dwork, Cynthia and Roth, Aaron and others},
%   journal={Foundations and trends{\textregistered} in theoretical computer science},
%   volume={9},
%   number={3--4},
%   pages={211--407},
%   year={2014},
%   publisher={Now Publishers, Inc.}

% @inproceedings{xia2025theoretical,
%   title={Theoretical Insights in Model Inversion Robustness and Conditional Entropy Maximization for Collaborative Inference Systems},
%   author={Xia, Song and Yu, Yi and Yang, Wenhan and Ding, Meiwen and Chen, Zhuo and Duan, Ling-Yu and Kot, Alex C and Jiang, Xudong},
%   booktitle={Proceedings of the Computer Vision and Pattern Recognition Conference},
%   pages={8753--8763},
%   year={2025}
% }




==> dareDEVALII/Sections/oldSEC_ABSTRACTv3.tex <==
%
%  PLACEHOLDER ABSTRACT
%In this paper, we show that the prevailing view that memorization drives training data exposure to reconstruction attacks is incomplete. We find that extensive exposure can persist without rote memorization, driven instead by a tunable connection to robustness. 
%We provide  evidence that privacy arises from generalizable but imperceptible features. We further show that recent privacy defenses obtain their privacy improvements by unintentionally shifting models toward such features. We leverage this mechanism to introduce, a training regime that intentionally learns such features to obtain both superior reconstruction defense \emph{and} higher accuracy than state-of-the-art defenses. Our results revise the prevailing understanding of training data exposure and reveal a new tradeoff.
%
%
\begin{abstract}
% \textbf{A: Submission?:\\}  
% In this paper, we show that the prevailing view that memorization (\textcolor{orange}{formalized as information dependency}) drives training data exposure to image reconstruction attacks is incomplete.
In this paper, we show that the prevailing view that information dependency (including rote memorization) drives training data exposure to image reconstruction attacks is incomplete.
We find that extensive exposure can persist without rote memorization, driven instead by a tunable connection to adversarial robustness. 
%
%
% \textbf{B: Camera-Ready:\\} In this paper, we challenge the prevailing view that memorization (formalized as information dependency) drives training data exposure to image reconstruction attacks. We show that extensive exposure can persist without rote memorization, driven instead by a tunable connection to adversarial robustness. 
%
%
We begin by presenting three surprising results: (1) recent defenses that inhibit reconstruction by Model Inversion Attacks (MIAs), which evaluate leakage under an idealized attacker, do \emph{not} reduce standard measures of information dependency (HSIC); (2) models that maximally memorize their training datasets remain robust to MIA reconstruction; and (3) models trained without seeing 97\% of the training pixels, where recent information-theoretic bounds give arbitrarily strong privacy guarantees under standard assumptions, can still be devastatingly reconstructed by MIA. 
%
%
To explain these findings, we provide causal evidence that privacy under MIA arises from what the adversarial examples literature calls ``non-robust'' features (generalizable but imperceptible and unstable features). We further show that recent MIA defenses obtain their privacy improvements by unintentionally shifting models toward such features. We leverage this mechanism to introduce \mbox{\textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining} (\textbf{AT-AT}~\ATATiconMINI), a training regime that intentionally learns non-robust features to obtain both superior reconstruction defense and higher accuracy than state-of-the-art defenses. Our results revise the prevailing understanding of training data exposure and reveal a new privacy-robustness tradeoff.
\end{abstract}

==> dareDEVALII/Sections/old_APP_adversarial_experimental_setup.tex <==
% \section{Adversarial Robustness Evaluation: More Experimental Details}
% \label{app:adversarial_exp_setup}

% As explained by \citep{carlini_evaluating_2019}, adversarial robustness (and, therefore, adversarial vulnerability) is often improperly quantified. To mitigate this issue, \citep{carlini_evaluating_2019} provide a checklist of actions to take to ensure proper evaluation of adversarial robustness, including performing adaptive attacks, applying a diverse set of attacks, and verifying that attacks have converged. In response to this advice, the AutoAttack ensemble \citep{croce_reliable_2020} has emerged as a popular benchmark to measure adversarial robustness due to its fixed hyperparameters, automatic convergence checks, and diversity of attacks. The four primary adversarial attacks in the ensemble are 1) untargeted Auto-PGD with cross-entropy loss; 2) targeted Auto-PGD with Difference of Logits Ratio (DLR) loss; 3) Fast Adaptive Boundary (FAB) \citep{croce_minimally_2020}; and 4) Square Attack \citep{andriushchenko_square_2020}. The two Auto-PGD variants are original to the AutoAttack paper \citep{croce_reliable_2020}. We run AutoAttack with varying $L_\infty$ ball constraints on 1024 examples of the validation set for each of the reported target models. \\\\

==> dareDEVALII/Sections/old_SEC_ABSTRACTorig.tex <==
%
%
%
%
\begin{abstract}
%
\textcolor{lightgray}{
In this paper, we show that the prevailing view that memorization drives training data exposure to reconstruction attacks is incomplete: extensive exposure can persist without rote memorization, driven instead by a previously unknown but tunable connection to adversarial example robustness. % shaped by
%
We present a surprising set of experiments showing that: (1) recent defenses that inhibit reconstruction by Model Inversion Attacks (MIAs), which evaluate leakage under an idealized attacker, do \emph{not} reduce well-known measures of memorization (the hypothesized driver of their defenses); (2) models that perfectly memorize their training dataset are robust to MIA reconstruction; and (3) 
%
models trained without seeing 98\% of the training data pixels, for which recent information-theoretic privacy results give arbitrarily large bounds against reconstruction, can still be largely reconstructed by MIA.
%
To explain these results, we conduct the first systematic evaluation of the robustness of model inversion defenses to adversarial examples.
%
We find that recent defenses hinder reconstruction in part by unintentionally shifting models away from what are known in the adversarial examples literature as “robust features" and, in some cases, toward ``non-robust'' (i.e., generalizable but imperceptible and unstable) features. 
%
We leverage this property to introduce \textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI), a training regime that tunes this mechanism to obtain both superior reconstruction defense \emph{and} higher accuracy than state-of-the-art defenses. Our results reframe the theory of training data exposure and reveal a new privacy–robustness tradeoff. \textcolor{red}{(225 words==OK).}
%
}
%\vspace{2em}
\end{abstract}






% \section{tl;dr}
% We show that the prevailing view that memorization drives training data exposure to reconstruction attacks is incomplete: extensive exposure can persist without rote memorization, driven instead by a previously unknown but tunable connection to adversarial example vulnerability. This property reveals a new privacy–robustness trade-off and enables stronger privacy defenses.% shaped by



==> dareDEVALII/Sections/old_SEC_ABSTRACTv2.tex <==
%
%
%
%
\begin{abstract}
\textcolor{lightgray}{
%
In this paper, we show that the prevailing view that memorization drives training image exposure to reconstruction attacks is incomplete: extensive exposure can persist without rote memorization, driven instead by a previously unknown but tunable connection to adversarial example robustness. % shaped by
%
We present a surprising set of experiments showing that: 
%
(1) recent defenses that inhibit reconstruction by Model Inversion Attacks (MIAs), which evaluate leakage under an idealized attacker, do \emph{not} reduce well-known measures of memorization (the hypothesized driver of their defenses); 
%
(2) models that perfectly memorize their training dataset are robust to MIA reconstruction; 
%
and (3) models trained without seeing 98\% of the training data pixels, for which recent information-theoretic privacy results give arbitrarily large bounds against reconstruction, can still be largely reconstructed by MIA. 
%
To explain these results, we present converging evidence that recent defenses hinder reconstruction in part by unintentionally shifting models towards what are known in the adversarial examples literature as ``non-robust'' (i.e., generalizable but imperceptible and unstable) features.
%
% To explain these results, we present converging evidence that privacy under MIA is caused what are known in the adversarial examples literature as ``non-robust'' (i.e., generalizable but imperceptible and unstable) features. Recent defenses hinder reconstruction in part by unintentionally shifting models towards such features
%
We leverage this property to introduce \textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI), a training regime that intentionally tunes this mechanism to obtain both superior reconstruction defense \emph{and} higher accuracy than state-of-the-art defenses. Our results reframe the theory of training data exposure and reveal a novel privacy–robustness tradeoff. \textcolor{red}{(207 words==OK).}
%
}
\end{abstract}



\begin{abstract}
\textcolor{lightgray}{
In this paper, we present converging evidence that reducing memorization dependency does not cause training data privacy leakage under modern model inversion attacks (MIA) designed to evaluate leakage under an idealized attacker. This evidence contradicts a dominant assumption in the MIA literature. Building on this insight, we show  that recent defenses hinder reconstruction in part by unintentionally shifting models towards what are known in the adversarial examples literature as ``non-robust'' (i.e., generalizable but imperceptible and unstable) features.
%
We leverage this property to introduce \textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI), a training regime that intentionally tunes this mechanism to obtain both superior reconstruction defense \emph{and} higher accuracy than state-of-the-art defenses. Our results reframe the theory of training data exposure and reveal a new privacy–robustness tradeoff.
}
\end{abstract}



% \section{tl;dr}
% We show that the prevailing view that memorization drives training data exposure to reconstruction attacks is incomplete: extensive exposure can persist without rote memorization, driven instead by a previously unknown but tunable connection to adversarial example vulnerability. This property reveals a new privacy–robustness trade-off and enables stronger privacy defenses.% shaped by





% \section{Reversed abstract}
% %
% In this paper, we show that the prevailing view that memorization drives training data exposure to reconstruction attacks is incomplete, and exposure is instead governed by a previously unknown but tunable link to adversarial example vulnerability.
% %
% We leverage this property to introduce \textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI), a training regime that tunes this mechanism to obtain both superior reconstruction defense \emph{and} higher accuracy than state-of-the-art defenses.
% %
% We motivate our contribution with a surprising set of experiments: (1) recent defenses that reduce reconstruction by Model Inversion Attacks (MIAs) designed to evaluate leakage under an idealized attacker do \emph{not} reduce well-known measures of memorization (the hypothesized driver of their protection); (2) models that perfectly memorize their training dataset are robust to MIA reconstruction; and (3) models trained without seeing 98\% of the training data pixels can be highly vulnerable to (total) training data reconstruction.
% %
% To explain these results, we conduct the first systematic evaluation of the robustness of model inversion defenses to adversarial examples.
% %
% We find that recent defenses already succeed in part by unintentionally shifting models away from what are known in the adversarial examples literature as “robust features" and, in some cases, toward ``non-robust features" (i.e., generalizable but imperceptible and unstable features). 
% %
%  Our results reframe the theory of training data exposure and reveal a new, practically relevant privacy–robustness trade-off.
%

% \section{Mini abstract}
% In this paper, we show that the prevailing view that memorization drives training data exposure to reconstruction attacks is incomplete: extensive exposure can persist without rote memorization, driven instead by a previously unknown but tunable connection to adversarial example vulnerability. 
% We present a surprising set of experiments showing that: (1) recent defenses that reduce reconstruction by model inversion attacks (MIAs) designed to evaluate leakage under an idealized attacker do \emph{not} reduce standard measures of memorization (as widely hypothesized); (2) models that perfectly memorize their training set can be robust to MIA reconstruction; and (3) models trained without 98\% of training pixels can still be almost fully reconstructed.
% The first systematic evaluation of the robustness of model inversion defenses to adversarial examples reveals that leading defenses work by unintentionally shifting models away from “robust” features and, in some cases, toward “non-robust” (i.e. generalizable but imperceptible and unstable) features.
% Exploiting this property, we introduce \textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI), which deliberately tunes this mechanism to achieve state-of-the-art reconstruction defense while improving accuracy.
% Our results reframe the theory of training data exposure and expose a new privacy–robustness trade-off.  %\textcolor{red}{(170ish words).}


% \bigskip 

% {
% \centering
% \medskip
%     \includegraphics[height=27ex]{dareDEVALII/Figures/starwars.jpeg}
%     \smallskip
%     \vspace{1.5em}
%     \includegraphics[height=27.38ex]{dareDEVALII/Figures/at-ats.jpg}
% }

    

%
% Recently, multiple algorithms have obtained strong performance in terms of protecting training data from reconstruction by model inversion attacks designed to evaluate leakage under an idealized attacker, and this performance has been attributed to the hypothesis that rote memorization drives the vulnerability. 
%
% However, we present a surprising set of experiments showing that (1) models that perfectly memorize their training dataset are robust to reconstruction; (2) models trained without seeing 98\% of the training data pixels can be highly vulnerable to reconstruction; (3) defenses reduce reconstruction often without reducing well-known measures of direct memorization. 
% %
% %
% %
% Recently, multiple algorithms have obtained strong performance in terms of protecting training data from reconstruction by model inversion attacks designed to evaluate leakage under an idealized attacker, and this performance has been attributed to the hypothesis that rote memorization drives the vulnerability. 
%

==> dareDEVALII/Sections/old_SEC_Anti-AT.tex <==



\section{\underline{A}n\underline{t}i \underline{A}dversarial \underline{T}raining (\textsc{AT-AT)}\huge~\ATATicon}

We now show how to exploit this mechanism \textcolor{red}{[hopefully `this mechanism' makes sense per wtv is directly above]} to obtain both superior and higher accuracy. We describe \textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI), a novel class of privacy/MIA defense training regimes that balance model accuracy with gradient steps that reverse standard adversarial training. These steps reshape the learned feature basis by shifting towards non-robust (but still generalizable) features that are visually imperceptible to humans and thus unamenable to visual reconstruction under MIA.  For intuition, suppose that on a given iteration of SGD, we draw an image $x_{\text{Yoda}}$ of class $y=\text{Yoda}$.


\textbf{Vanilla Training.} A vanilla loss function $\mathcal{L}(\theta, x, y)$  just rewards the accurate mapping $x_{\text{Yoda}}\rightarrow \text{Yoda}$. 

\textbf{Classic Adversarial Training (AT).}
Classic Adversarial Training \citep{madry_towards_2019} separately computes for $x_{\text{Yoda}}$ a small feasible adversarial perturbation $\delta \in \mathcal{S}, \text{s.t.} \ |\delta|_\infty \leq \epsilon$, which attempts to `fool' the training model into mapping $(x_{\text{Yoda}} + \delta)\rightarrow y', \ y'$$\ne$Yoda, where $y'$ is a randomly drawn target class. For example, suppose $\delta$ is a ``Luke perturbation,'' i.e., $(x_{\text{Yoda}} + \delta_{\text{Luke}})\rightarrow y'$=Luke$\ne$Yoda. The classic AT loss function $\max_{\delta \in \mathcal{S}} \mathcal{L_{\text{AT}}}(\theta, x + \delta, y$=\text{Yoda}$)$ rewards features that are \emph{robust} to this perturbation, i.e., ``($x_{\text{Yoda}}$ $+$ $\delta_{\text{Luke}}$) $\rightarrow$ Yoda,'' and penalizes features that are \emph{non-robust}. 
%
\textcolor{red}{If we define the $\delta$ stuff above im the adv example vulnerability part then this can be more concise.}
%

\textbf{\underline{A}n\underline{t}i \underline{A}dversarial \underline{T}raining (\textbf{AT-AT}~\ATATiconMINI).} Our goal is the opposite: we seek to learn to \emph{ignore} visually robust features and \emph{reward} features that are visually imperceptible but generalizable (`non-robust features'). Thus, compared to AT, we optimize for the opposite mapping: ``($x_{\text{Yoda}}$ $+$ $\delta_{\text{Luke}}$) $\rightarrow$ Luke.'' More formally, we seek     \mbox{$\max_{\delta \in \mathcal{S}} \mathcal{L}(\theta, x + \delta, \mathbf{y'})
    %}_{\text{anti adv.}} 
    $$,
    \ \text{where } \mathbf{y'} \neq y$}. However, as a practical matter, it is infeasible to obtain competitive accuracy for challenging learning tasks like hi-def facial recognition using exclusively non-robust features. Thus, we adopt a dual loss function that balances vanilla accuracy with non-robust features:
%
 \begin{align}
 %
 % % Vanilla
 %    \min_{\theta} \ \mathbb{E}_{(x, y) \sim \mathcal{D}} &\left[ 
 %    \mathcal{L}(\theta, x, y)\right]; \text{i.e., ``$x_{Luke}$ $\rightarrow$ $Luke$''}\\
 % %
 % % AT (Madry)
 %    \min_{\theta} \ \mathbb{E}_{(x, y) \sim \mathcal{D}} &\left[ 
 %     \cdot \max_{\delta \in \mathcal{S}} \mathcal{L}(\theta, x + \delta, y) 
 %    \right]; \text{i.e., ``$x_{Luke} + \delta_{Yoda} \rightarrow Luke$''} \\
 % %
 %
 %
 % % ANTI-AT
    % \text{\textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI) \ \ \ \  }
    %
    \text{\textbf{AT-AT Objective: \ \ }}\min_{\theta} \ \mathbb{E}_{(x, y) \sim \mathcal{D}} 
    %
    [ 
    %\underbrace{
 \mathcal{L}(\theta, x, y) %}_{\text{vanilla}} 
    %
    \ + \ \lambda \cdot 
    %\underbrace{
    \max_{\delta \in \mathcal{S}} \mathcal{L}(\theta, x + \delta, \mathbf{y'})
    %}_{\text{anti adv.}} 
    ],
    \ \text{where } \mathbf{y'} \neq y \ \ \ \
    %\text{\ i.e.,  \ \ ``$x_{Luke} \rightarrow Luke \ \& \ x_{Luke} + \delta_{Yoda} \rightarrow Yoda$''} 
\end{align}
%
%
This \textbf{AT-AT} loss can be optimized similarly to vanilla AT. In each SGD iteration $i$ where the training model is denoted by $\mathcal{M}_i$, we draw a training image $x$ and a target class $y'$ each uniformly at random. We then compute a non-robust perturbation $\delta$ that causes $\mathcal{M}_i$ to classify $x$ not as $y$, but as $y'$, e.g., ``($x_{\text{Yoda}}$ $+$ $\delta_{\text{Luke}}$) $\rightarrow$ Luke.'' We then just sum vanilla loss on $y$ and anti-adversarial loss on $y'$. The latter penalizes robust features and rewards non-robust ones. Then, we backpropagate:
%
%\input{dareDEVALII/Sections/algorithm-AT-AT}
%
\input{dareDEVALII/Sections/algorithm-AT-AT-wallpapered}
%
\input{dareDEVALII/Sections/algorithm-AT-AT-wallpaperOVERLAY}

==> dareDEVALII/Sections/old_SEC_Anti-AT_v2.tex <==



\section{\underline{A}n\underline{t}i \underline{A}dversarial \underline{T}raining (\textsc{AT-AT)}\huge~\ATATicon}

We now show how to exploit this mechanism \textcolor{red}{[hopefully `this mechanism' makes sense per wtv is directly above]} to obtain both superior and higher accuracy. We describe \textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI), a novel class of privacy/MIA defense training regimes that balance model accuracy with gradient steps that reverse standard adversarial training. These steps reshape the learned feature basis by shifting towards non-robust (but still generalizable) features that are visually imperceptible to humans and thus unamenable to visual reconstruction under MIA.  For intuition, suppose that on a given iteration of SGD, we draw an image $x_{\text{Yoda}}$ of class $y=\text{Yoda}$.


\textbf{Vanilla Training.} A vanilla loss function $\mathcal{L}(\theta, x, y)$  just rewards the accurate mapping of the clean image $x_{\text{Yoda}}\rightarrow \text{Yoda}$. 

\textbf{Classic Adversarial Training (AT).}
Classic Adversarial Training replaces each clean training example $x$ with a pertur

\textbf{Classic Adversarial Training (AT).}
Classic Adversarial Training \citep{madry_towards_2019} separately computes for $x_{\text{Yoda}}$ a small feasible adversarial perturbation $\delta \in \mathcal{S}, \text{s.t.} \ |\delta|_\infty \leq \epsilon$, which attempts to maximally `fool' the training model into mapping the perturbed example to a different class (chosen $\mathcal{UAR}$). 
%$(x_{\text{Yoda}} + \delta)\rightarrow y', \ y'$$\ne$Yoda, where $y'$ is a randomly drawn target class. 
For example, suppose $\delta$ is a ``Luke perturbation,'' i.e., $(x_{\text{Yoda}} + \delta_{\text{Luke}})\rightarrow y'$=Luke$\ne$Yoda. The classic AT loss function $\max_{\delta \in \mathcal{S}} \mathcal{L_{\text{AT}}}(\theta, x + \delta, y$=\text{Yoda}$)$ rewards features that are \emph{robust} to this perturbation, i.e., ``($x_{\text{Yoda}}$ $+$ $\delta_{\text{Luke}}$) $\rightarrow$ Yoda,'' and penalizes features that are \emph{non-robust}. 
%
\textcolor{red}{If we define the $\delta$ stuff above im the adv example vulnerability part then this can be more concise.}
%

\textbf{\underline{A}n\underline{t}i \underline{A}dversarial \underline{T}raining (\textbf{AT-AT}~\ATATiconMINI).} Our goal is the opposite: we seek to learn to \emph{ignore} visually robust features in $x$ and \emph{reward} features exposed by the perturbation $\delta$ that are visually imperceptible but generalizable (`non-robust features'). Thus, compared to AT, we optimize for the opposite mapping: ``($x_{\text{Yoda}}$ $+$ $\delta_{\text{Luke}}$) $\rightarrow$ Luke.'' More formally, we seek     \mbox{$\max_{\delta \in \mathcal{S}} \mathcal{L}(\theta, x + \delta, \mathbf{y'})
    %}_{\text{anti adv.}} 
    $$,
    \ \text{where } \mathbf{y'} \neq y$}. However, as a practical matter, it is infeasible to obtain competitive accuracy for challenging learning tasks like hi-def facial recognition using exclusively non-robust features. Thus, we adopt a dual loss function that balances vanilla accuracy with non-robust features:
%
 \begin{align}
 %
 % % Vanilla
 %    \min_{\theta} \ \mathbb{E}_{(x, y) \sim \mathcal{D}} &\left[ 
 %    \mathcal{L}(\theta, x, y)\right]; \text{i.e., ``$x_{Luke}$ $\rightarrow$ $Luke$''}\\
 % %
 % % AT (Madry)
 %    \min_{\theta} \ \mathbb{E}_{(x, y) \sim \mathcal{D}} &\left[ 
 %     \cdot \max_{\delta \in \mathcal{S}} \mathcal{L}(\theta, x + \delta, y) 
 %    \right]; \text{i.e., ``$x_{Luke} + \delta_{Yoda} \rightarrow Luke$''} \\
 % %
 %
 %
 % % ANTI-AT
    % \text{\textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI) \ \ \ \  }
    %
    \text{\textbf{AT-AT Objective: \ \ }}\min_{\theta} \ \mathbb{E}_{(x, y) \sim \mathcal{D}} 
    %
    [ 
    %\underbrace{
 \mathcal{L}(\theta, x, y) %}_{\text{vanilla}} 
    %
    \ + \ \lambda \cdot 
    %\underbrace{
    \max_{\delta \in \mathcal{S}} \mathcal{L}(\theta, x + \delta, \mathbf{y'})
    %}_{\text{anti adv.}} 
    ],
    \ \text{where } \mathbf{y'} \neq y \ \ \ \
    %\text{\ i.e.,  \ \ ``$x_{Luke} \rightarrow Luke \ \& \ x_{Luke} + \delta_{Yoda} \rightarrow Yoda$''} 
\end{align}
%
%
This \textbf{AT-AT} loss can be optimized similarly to vanilla AT. In each SGD iteration $i$ where the training model is denoted by $\mathcal{M}_i$, we draw a training image $x$ and a target class $y'$ each uniformly at random. We then compute a non-robust perturbation $\delta$ that causes $\mathcal{M}_i$ to classify $x$ not as $y$, but as $y'$, e.g., ``($x_{\text{Yoda}}$ $+$ $\delta_{\text{Luke}}$) $\rightarrow$ Luke.'' We then just sum vanilla loss on $y$ and anti-adversarial loss on $y'$. The latter penalizes robust features in $x$ and rewards non-robust ones exposed by perturbation $d$.% Then, we backpropagate:

%The total loss sums the vanilla term on $(x,y)$ with an anti-adversarial term on $(x+\delta,\mathbf{y'})$. Unlike standard AT, which enforces robustness to perturbations and therefore learns robust features, AT-AT explicitly rewards the model for ignoring those robust features and learning to classify using the non-robust features exposed by $\delta$.

% This \textbf{AT-AT} loss can be optimized similarly to vanilla AT. On each SGD iteration with model $\mathcal{M}i$, we draw an image $x$ and a random target class $y'\neq y$. We then compute a perturbation $\delta$ such that $\mathcal{M}i(x+\delta)=y'$, e.g. “$x\text{Yoda}+\delta\text{Luke}\to$ Luke.” The total loss sums the vanilla term on $(x,y)$ with an anti-adversarial term on $(x+\delta,y')$. Unlike standard AT, which enforces invariance to perturbations and therefore emphasizes robust features, AT-AT explicitly rewards the model for ignoring those robust features and learning to classify primarily from the subtle, non-robust features exposed by $\delta$.

%
%\input{dareDEVALII/Sections/algorithm-AT-AT}
%
\input{dareDEVALII/Sections/algorithm-AT-AT-wallpapered}
%
\input{dareDEVALII/Sections/algorithm-AT-AT-wallpaperOVERLAY}

==> dareDEVALII/Sections/old_SEC_AutoAttack.tex <==
% Training data privacy is not caused by reducing memorization dependency, but by adversarially non-robust features.

% Adversarially non-robust features cause training data privacy. Reducing memorization dependency does not. 

% Reducing memorization dependency does not cause training data privacy. Adversarially non-robust features do.

% Reductions in memorization dependency do not cause training data privacy. Adversarially non-robust features do.

% Training data privacy is not caused by reductions in memorization dependency. It is caused by adversarially non-robust features.

% Training data privacy is not caused by reducing memorization dependency. Privacy is caused by adversarially non-robust features.




\section{The privacy leakage - adversarial robustness tradeoff}
\label{sec-autoattack}

\textcolor{orange}{different epses measure different types of non-robust features. Accuracy observation story.\\}

%
\textcolor{blue}{Reminder: Drop the nodefs (once we have many more) and re-run so we don't dominate regression. Report both.\\}
%
Our goal in this section is to describe a previously unobserved three-way \{privacy leakage, accuracy, adversarial robustness\} tradeoff that characterizes the performance of memorization dependency-based MIA defenses on the main architectures and datasets used to benchmark privacy attacks and defenses in recent work. We accomplish this by presenting the first systematic tests of the robustness of MIA defenses to a very different attack vector: adversarial examples. These tests allow us to consider the privacy and accuracy of MIA defenses against the robustness of their feature bases, which has not yet been measured comparatively. It equally allows us to evaluate the degree to which defenses unintentionally rely on imperceptible `non-robust features' of various magnitudes.

% Adversarial examples are small noise perturbations that when added to an image in the dataset, changes the prediction of the model. The noise is restricted to be in a small range $\lvert \lvert \delta \rvert\rvert_{p}<\epsilon$, where $\delta$ is the perturbation, $p$ is the norm and $\epsilon$ is the limit of the size of perturbations. Since the perturbations are limited to very small changes, they are mostly imperceptible for humans and don't carry semantic meaning.     

% The existence of adversarial examples was first discovered in \cite{szegedy_intriguing_2014} and it has since been widely studied how to generate them \cite{croce_reliable_2020} and defend against them \cite{madry_towards_2019, shafahi_adversarial_2019, wong_fast_2020}. 


%
%
% Top of page pics banner of woman with various autoattack noises epsilon vals
\input{dareDEVALII/Figure_code/adversarial_examples_mini_banner}
%
%
\textbf{Tradeoff experimental setup.} Following seminal work by \citep{carlini_evaluating_2019, croce_reliable_2020}, and others, a scholarly consensus has emerged regarding the design elements necessary to ensure the rigor of experiments that measure robustness to adversarial examples. This includes testing models under a diverse variety of attacks and a broad range of constraints $\epsilon$ on the magnitude of feasible adversarial perturbations. We carefully follow these design elements here. Specifically, we report worst-case accuracy on adversarial examples across all attacks in the AutoAttack ensemble, and also separately report accuracy for each of its four constituent attacks: untargeted Auto-PGD with cross-entropy loss; targeted Auto-PGD with Difference of Logits Ratio (DLR) loss; Fast Adaptive Boundary (FAB) \cite{fab}; and Square Attack \cite{square}. \textcolor{red}{!Fix attack citations.}   We find that all models under consideration have identical $0\%$ accuracy under AutoAttack with default $\epsilon=8/255$ (i.e. $0.031$), which renders model comparisons uninformative. Thus we also recompute attacks with a wide range of smaller perturbations: $\epsilon\in \{0.031, 0.0025, 0.0005, 0.00001\}$.  Fig. \ref{fig:adv-images-banner} shows an example of each. %Importantly, this range of $\epsilon$'s permit richly informative comparisons of (1) the robustness of defenses to various attack magnitudes, and (2) the degree to which each defense \emph{unintentionally relies on imperceptible `non-robust features' of various magnitudes.} 

\textbf{\textcolor{red}{Currently assuming that all defenses, architectures, datasets, and also PPA and AttackAcc@1 have already been introduced in the motivating experiments. Also assuming that adversarial examples and non-robust features have been described above. Maybe not and maybe not, respectively? Revisit.}}

\textbf{Tradeoff raw results tables.} Table \ref{tab:leakage-accuracy-robustness} presents privacy leakage (PPA Attack@1), test accuracy on clean images, and the worst-case robust accuracy under under AutoAttack adversarial examples (across all constituent attacks) with various perturbation magnitudes $\epsilon$. We also report disaggregated robust accuracy results in Appendices \textcolor{red}{REF, REF, REF, REF}.

Across Table \ref{tab:leakage-accuracy-robustness}, the \{privacy leakage, accuracy, adversarial robustness\} tradeoff is qualitatively noticeable for the undefended model (NoDef) and all defenses that attempt to reduce memorization (MID, BiDO, TL-DMI). Specifically, less privacy leakage (lower Attack@1) corresponds to \emph{worse} clean test accuracy and \emph{worse} robust accuracy under all AutoAttacks. 


\textbf{Estimating the \{privacy leakage, accuracy, adversarial robustness\} tradeoff.} To obtain a principled test of the explanatory strength of the  tradeoff, we estimate simple linear regression models of the following form. This allows us to explicitly test the degree to which a model's privacy leakage (PPA Attack@1) is a simple linear combination of its clean test accuracy and its robust accuracy:
%
% \begin{align}
%     \text{Leakage}_{\text{Attack@1}} = 
%     \beta_0 + 
%     \beta_1 \text{TestAcc} + 
%     \beta_2 \text{Acc}_{\epsilon\text{=}0.0025} + \beta_3 \text{Acc}_{\epsilon\text{=}0.0005} + \beta_4 \text{Acc}_{\epsilon\text{=}0.00001}
%     \label{OLS}
% \end{align}
%
% \begin{align}
% \text{Leakage}_{\text{Attack@1}} &= 
%     \beta_0 + 
%     \beta_1 \text{TestAcc} &\text{ \emph{(Clean accuracy only)};}\\
%     %
%     \text{Leakage}_{\text{Attack@1}} &= 
%     \beta_0 + 
%     \beta_1 \text{TestAcc} + 
%     \beta_2 \text{Acc}_{\epsilon\text{=}0.0025} &\text{\emph{(Clean \& robust at $\epsilon\text{=}0.0025$ only)};}\\
%     %
%     \text{Leakage}_{\text{Attack@1}} &= 
%     \beta_0 + 
%     \beta_1 \text{TestAcc} + 
%     \beta_2 \text{Acc}_{\epsilon\text{=}0.0025} + \beta_3 \text{Acc}_{\epsilon\text{=}0.0005} + \beta_4 \text{Acc}_{\epsilon\text{=}0.00001} &\text{\emph{(All predictors).}}
%     \label{OLS}
% \end{align}
%
%
%
%
%
% \begin{align}
% \text{Leakage}_{\text{Attack@1}} &=
%   \beta_0 + \beta_1 \,\text{TestAcc}
%   \tag*{\emph{(Clean accuracy only)}}\\
% %
% \text{Leakage}_{\text{Attack@1}} &=
%   \beta_0 + \beta_1 \,\text{TestAcc} + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
%   \tag*{\emph{(Clean \& robust at $\epsilon$=$0.0025$ only)}}\\
% %
% \text{Leakage}_{\text{Attack@1}} &=
%   \beta_0 + \beta_1 \,\text{TestAcc} + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
%   + \beta_3 \,\text{Acc}_{\epsilon=0.0005} + \beta_4 \,\text{Acc}_{\epsilon=0.00001}
%   \tag*{\emph{(All predictors)}}
% \end{align}
%
%
%
%
\vspace{-1em}
%
\begin{align}
\text{Leakage}_{\text{Attack@1}} &=
  \beta_0 + \beta_1 \,\text{TestAcc}
   \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad 
   \text{\emph{(Clean accuracy only)}} \label{eq:OLSclean}\\
%
\text{Leakage}_{\text{Attack@1}} &=
  \beta_0 + \beta_1 \,\text{TestAcc} + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
   \quad \quad \quad \quad \quad \quad \quad \quad \ \
   \text{\emph{(Clean \& robust at $\epsilon\text{=}0.0025$ only)}} \label{eq:OLSrobust}\\
%
\text{Leakage}_{\text{Attack@1}} &=
  \beta_0 + \beta_1 \,\text{TestAcc} + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
  + \beta_3 \,\text{Acc}_{\epsilon=0.0005} + \beta_4 \,\text{Acc}_{\epsilon=0.00001}
   \quad \ \ \text{\emph{(All predictors)}} \label{eq:OLSall}
\end{align}
%
%
\vspace{-1em}
%
%
%
% \[
% \begin{alignedat}{2}
% \text{Leakage}_{\text{Attack@1}} &= \beta_0 + \beta_1 \,\text{TestAcc}
%   &\quad& \text{\emph{(Clean accuracy only)}};\\
% \text{Leakage}_{\text{Attack@1}} &= \beta_0 + \beta_1 \,\text{TestAcc}
%   + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
%   &\quad& \text{\emph{(Clean \& robust at $\epsilon$=$0.0025$ only)}};\\
% \text{Leakage}_{\text{Attack@1}} &= \beta_0 + \beta_1 \,\text{TestAcc}
%   + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
%   + \beta_3 \,\text{Acc}_{\epsilon=0.0005}
%   + \beta_4 \,\text{Acc}_{\epsilon=0.00001}
%   &\quad& \text{\emph{(All predictors).}}
% \end{alignedat}
% \]
%

We are careful to also estimate alternative Beta regression variants of each of the above models with appropriate distributional assumptions to capture the fact that the response variable (PPA Attack@1) is bounded in $[0,1]$:

%
% Technically, the response variable (PPA Attack@1) is bounded in $[0,1]$, this we also consider a Beta regression variation of the above model that conveys the appropriately bounded distributional assumption:
%
\begin{align}
    \text{Leakage}_{\text{Attack@1}} &\sim \text{Beta}(\mu_j \phi, \ (1 - \mu_j) \phi)   \nonumber\\
    g(\mu_j) &=     
    \beta_0 + 
    \beta_1 \text{TestAcc} 
       \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad 
   \text{\emph{(Clean accuracy only)}} \label{eq:betaclean}\\
    %
    g(\mu_j) &= 
    \beta_0 + 
    \beta_1 \text{TestAcc} + 
    \beta_2 \text{Acc}_{\epsilon\text{=}0.0025}    \quad \quad \quad \quad \quad \quad \quad \quad \quad
   \text{\emph{(Clean \& robust at $\epsilon\text{=}0.0025$ only)}} \label{eq:betarobust}\\
    % 
    g(\mu_j) &= 
    \beta_0 + 
    \beta_1 \text{TestAcc} + 
    \beta_2 \text{Acc}_{\epsilon\text{=}0.0025} + \beta_3 \text{Acc}_{\epsilon\text{=}0.0005} + \beta_4 \text{Acc}_{\epsilon\text{=}0.00001}
    \quad \quad \ \ \text{\emph{(All predictors)}} 
     \label{eq:betaall}
\end{align}
%
Where response PPA Attack@1 is modeled as a beta distribution with mean $\mu_j$ and precision $\phi$, where the mean is linked to predictors via the standard logit link function $g(x)$.


\begin{wrapfigure}{r}{0.35\textwidth} % r=right, l=left
    \centering
%
        \caption{Top: Leakage vs. clean accuracy. Bottom: leakage predicted by clean \& robust accuracy (pseudo $R^2$=$0.947$).}
%
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{dareDEVALII/Figures/leak_vs_TestAcc_4.85.pdf}
        \caption{Top: Observed leakage vs. clean accuracy.}
        \label{fig:leakage_vs_accuracyonly}
    \end{subfigure}
%
    % \vspace{0.5em} % small gap between the two
    % \begin{subfigure}[t]{\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{dareDEVALII/Figures/leak_vs_pred_4.85.pdf}
    %     \caption{Leakage vs. leakage predicted by simple linear model of clean \& robust accuracy (adj. $R^2$=$0.924$).}
    %     \label{fig:leakage_vs_pred_leakage}
    % \end{subfigure}
%
    \vspace{0.5em} % small gap between the two
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{dareDEVALII/Figures/leak_vs_pred_RobOnlyBeta_4.85.pdf}
        \caption{Bottom: Observed leakage vs. leakage predicted by robust accuracy only (pseudo $R^2$=$0.947$).}
        \label{fig:leakage_vs_pred_leakage}
    \end{subfigure}
%
    \label{fig:leakage_comparison}
\end{wrapfigure}



\input{dareDEVALII/Tables/AutoAttack_RegTable_MemDef}
\input{dareDEVALII/Tables/AutoAttack_RegTable_TrickDef}
\input{dareDEVALII/Tables/AutoAttack_RegTable_Sanity_MemDef}
\input{dareDEVALII/Tables/AutoAttack_RegTable_Sanity_TrickDef}

                  
\textbf{Results.}
Across various specifications, linear models show that linear combinations of clean test accuracy and robust accuracy at various AutoAttack $\epsilon$ explain $R^2=94.2\%$ of the variance of privacy leakage, measured by PPA Attack@1. These results are robust to various alternate specifications, robust clustered standard errors (clustered by architecture and/or dataset), etc. See Appendix \textcolor{red}{REFERENCE}.

\textbf{Computing \emph{accuracy-adjusted privacy gain}: a new comparison metric for privacy benchmarking}

\textbf{Computing \emph{accuracy-adjusted robustness cost}: a new comparison metric for privacy benchmarking}

We can use these linear models to compute the concrete costs of privacy. For example, 
holding test accuracy constant, reducing leakage (PPA Attack@1) by $1$ percentage point corresponds to a:
\begin{itemize}
    \item  $0.43$ percentage-point decrease (95\% CI: 0.31–0.71 pp) in AutoAttack robust accuracy at $\epsilon=0.0025$;
    \item $1.93$ percentage-point decrease (95\% CI: 1.44–2.94 pp) in AutoAttack robust accuracy at $\epsilon=0.0005$.
\end{itemize}
In other words, each increase in privacy that hurts MIA attacker accuracy by $1\%$ costs the model approximately $2\%$ accuracy under imperceptible adversarial examples ($\epsilon=0.0005$). \textcolor{orange}{correlation not causation lang here.}


\begingroup
\addtolength\leftmargini{-0.15in} % shrink quote margin
\begin{quote}
%\vspace{-2mm}
\begin{center}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null\\
\vspace{-2mm}
 \textit{These results provide evidence that non-robust features were unknowingly \emph{correlated} with greater privacy. Can non-robust features \emph{cause} privacy through deliberate algorithmic design?}
 \vspace{-1mm}
\end{center}
\vspace{-2mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null
%\vspace{-2mm}
\end{quote}
\endgroup




%
%
% Main Body AutoAttack Table
\input{dareDEVALII/Tables/AA-bodyofpaper}
%
%
\newpage
\clearpage
%
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{dareDEVALII/Figures/leak_vs_TestAcc_4.85.pdf}
%     \caption{Leakage (PPA Attack@1) vs. clean test accuracy (see Table \ref{tab:leakage-accuracy-robustness}).}
%     \label{fig:leakage_vs_accuracyonly}
% \end{figure}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{dareDEVALII/Figures/leak_vs_pred_4.85.pdf}
%     \caption{Leakage (PPA Attack@1) vs. leakage predicted from a simple linear combination of clean accuracy and robust accuracy (see Table \ref{tab:leakage-accuracy-robustness}). Goodness of fit $R^2$=$0.94$.}
%     \label{fig:leakage_vs_pred_leakage}
% \end{figure}

% \begin{figure}[t] % [t] = top of page
%     \centering
%     %
%     \begin{subfigure}[t]{0.44\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{dareDEVALII/Figures/leak_vs_TestAcc_4.85.pdf}
%         \caption{Leakage (PPA Attack@1) vs. clean test accuracy.}
%         \label{fig:leakage_vs_accuracyonly}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}[t]{0.44\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{dareDEVALII/Figures/leak_vs_pred_4.85.pdf}
%         \caption{Leakage (PPA Attack@1) vs. leakage predicted from a linear combination of clean and robust accuracy. $R^2$=$0.94$.}
%         \label{fig:leakage_vs_pred_leakage}
%     \end{subfigure}
%     %
%     \caption{see (see Table \ref{tab:leakage-accuracy-robustness})}
%     \label{fig:leakage_comparison}
% \end{figure}


% OLS LINEAR REGRESSION TABLE
\input{dareDEVALII/Tables/RegressionTableOLS}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.\linewidth]{dareDEVALII/Figures/leak_vs_robustacc.pdf}
%     \caption{Leakage (PPA Attack@1) vs. robust accuracy at various AutoAttack$\epsilon$.}
%     \label{fig:leakage_vs_each_AdvExEpsilon}
% \end{figure}



% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.3\linewidth]{dareDEVALII/Figures/tradeoffsMarioKart.jpg}
%     \caption{Accurate illustration of the tradeoffs between accuracy, robustness, and privacy.}
%     \label{fig:tradeoffs-mariokart}
% \end{figure}



% As explained by \cite{carlini_evaluating_2019}, adversarial robustness (and, therefore, adversarial vulnerability) is often improperly quantified. To mitigate this issue, \cite{carlini_evaluating_2019} provide a checklist of actions to take to ensure proper evaluation of adversarial robustness, including performing adaptive attacks, applying a diverse set of attacks, and verifying that attacks have converged. In response to this advice, the AutoAttack ensemble \cite{croce_reliable_2020} has emerged as a popular benchmark to measure adversarial robustness due to its fixed hyperparameters, automatic convergence checks, and diversity of attacks. The four primary adversarial attacks in the ensemble are 1) untargeted Auto-PGD with cross-entropy loss; 2) targeted Auto-PGD with Difference of Logits Ratio (DLR) loss; 3) Fast Adaptive Boundary (FAB) \cite{fab}; and 4) Square Attack \cite{square}. \\\\


% Adversarial examples are small noise perturbations that when added to an image in the dataset, changes the prediction of the model. The noise is restricted to be in a small range $\lvert \lvert \delta \rvert\rvert_{p}<\epsilon$, where $\delta$ is the perturbation, $p$ is the norm and $\epsilon$ is the limit of the size of perturbations. Since the perturbations are limited to very small changes, they are mostly imperceptible for humans and don't carry semantic meaning.     

% The existence of adversarial examples was first discovered in \cite{szegedy_intriguing_2014} and it has since been widely studied how to generate them \cite{croce_reliable_2020} and defend against them \cite{madry_towards_2019, shafahi_adversarial_2019, wong_fast_2020}. 

% \input{dareDEVALII/Figure_code/adversarial_examples}


% \textbf{Our contribution II: The privacy-robustness feature tradeoff.}

% %We uncover a previously unknown mechanism that directly links training data exposure vulnerabilities to the well-studied robust–non-robust feature tradeoff from the adversarial examples literature. 
% To probe these phenomena, we conduct the first systematic evaluation of the robustness of memorization/MIA defenses to adversarial examples. Our analysis reveals that state-of-the-art privacy defenses do not primarily protect against reconstruction by reducing direct data–model dependency, as widely assumed. Instead, they operate by reshaping the learned feature basis. Specifically, they protect privacy by unintentionally suppressing reliance on ``robust features'' (i.e., generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics), and in some cases, replacing them with ``non-robust features'' (i.e., features that generalize well but are imperceptible to humans and unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}. This shift yields a tradeoff: suppressing robust features strips semantically meaningful information from the model but degrades accuracy, while replacing robust features with non-robust features recovers accuracy at the cost of brittleness, leaving models vulnerable to adversarial examples. Although robust–non-robust feature reliance is heavily studied in adversarial robustness, our work is the first to show its central role in training data privacy vulnerabilities. 


%  \textcolor{red}{[make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with Adversarial Examples]}


==> dareDEVALII/Sections/old_SEC_INTRO_2ndcut.tex <==


\section{Introduction}


A foundational goal of contemporary machine learning is to learn \emph{generalizable} model parameters from the training data without \emph{exposing} training data examples to leakage. However, it is well known that virtually all modern architectures obtain generalizable performance only at the cost of encoding a substantial amount of sensitive information about their training examples. This tradeoff defines a critical research frontier in terms of the efficiency of current training regimes and learned representations. It also compromises model privacy by providing a key practical vulnerability that is exploited by myriad new attacks.




% \textbf{Training data exposure reveals fundamental gaps in learning.} 

% Venn diagram First, in the era of billion dollar training expenditures, backpropagating to learn idiosyncratic, ungeneralizable training example information reflects a fundamental learning inefficiency that continues to accrue costs when ungeneralizable parameters are called at inference time \textcolor{red}{[Cite a bunch of papers]}.







% The tendency of contemporary machine learning models to expose their private training data has recently emerged as a critical research and security frontier. A foundational goal of machine learning is to obtain an \emph{efficient} and \emph{generalizable} set of model parameters. However, it is well-known that virtually all modern architectures also unintentionally encode a substantial amount of sensitive information about their training data. This tradeoff reveals a fundamental deficit in terms of the efficiency of current training regimes and learned representations. It also compromises model privacy by providing a key practical vulnerability that is exploited by myriad new attacks.

\textbf{Training data exposure reveals fundamental gaps in learning.} % Venn diagram

 \textbf{Training data exposure undermines privacy in ML deployments.}
Second, training data exposure underlies a rapidly expanding class of practical privacy attacks that reconstruct private training data from real-world machine learning deployments simply by querying models or inspecting their parameters. Recent variants of training data attacks apply not only to CNN's, but also to LLM's, diffusion models, multimodal models, etc. \textcolor{red}{[Cite membership inference, attribute inference, carlini's extraction attacks on text LLM's and on stable diffusion].}



\textbf{Model inversion attacks (MIA's) probe and exploit training data exposure.} 
In particular, model inversion attacks (MIA's) have become a mainstream tool for studying and evaluating training data exposure. Unlike more conservative attacks that merely test for the presence of some exposed training examples, MIAs test the degree to which a powerful attacker armed with white-box model access and significant computational resources can reconstruct the full set of class-level features for each class in the training data. 

\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }



%While the success of MIA's demonstrates the existence of memorized training examples in contemporary models, 
While MIA's lower-bound the extent to which training data is vulnerable to reconstruction, they do not explain what aspect of trained models encodes this vulnerability, or how to prevent it. \textcolor{purple}{This raises a fundamental question:}


\begingroup
\addtolength\leftmargini{-0.15in} % shrink quote margin
\begin{quote}
%\vspace{-2mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null\\[-2.5mm]
\begin{center}
\vspace{-5mm}
 \textit{How is the training data exposure vulnerability encoded in contemporary models?}
 \vspace{-1mm}
\end{center}
\vspace{-2.5mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null
%\vspace{-2mm}
\end{quote}
\endgroup


\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }

\textbf{The prevailing `training data exposure = memorization' theory.} 

% Edit this following DP paragraph bc DP is basically in the memorization vein since it's about how much the global statistic shares info about its component observations
\textbf{Classical privacy frameworks like DP do not explain the training data exposure that MIA's exploit.}
While classical privacy frameworks such as Differential Privacy (DP) \cite{dwork2006differential, dwork2014algorithmic} offer provable guarantees against training example exposure \citep{hayes_bounding_2023}, they do not explain why it arises in contemporary learning settings. 
DP was designed to protect the privacy of individual training examples while releasing parameters that characterize in-sample group-level descriptive statistics. These competing goals have a direct information-theoretic tradeoff. 
% DP was designed to control the direct information-theoretic tradeoff between the privacy of individual training examples we want to protect and the accuracy of in-sample group-level statistics we want to release.
However, the same direct tradeoff does not obviously apply to releasing model parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning).
%It does not directly apply when releasing parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning), where it is not obvious how such a tradeoff applies. 
As a result, extending DP-based protections to learning applications may be sufficient to protect the training data from exposure, but they may be unnecessary for this goal, and their very high computational and accuracy costs render them practically inapplicable in large-scale learning deployments.

\textbf{Recent learning theory underscores a theoretic deficit.}
To address the theoretic gap left by DP, a very recent stream of theoretic work seeks novel noise-based techniques that upper-bound the degree to which training data can be reconstructed by any unbiased estimator. Nonetheless, as we demonstrate, that approach may provide a false sense of security: 
\textcolor{red}{\textbf{FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein} have recent bounds that also use noise and try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we crush this hope with our DropLayer mask and PPA/IFGMI use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it? Or below?}




\textbf{State-of-the-art defenses theorize that MIA's reveal and exploit memorization in the form of direct data-to-model dependencies.}
An influential recent line of algorithms have obtained practically performant defenses against training data exposure/MIA, and argued that their practical performance can be attributed to their shared theoretic hypothesis that MIA vulnerability arises from direct and excessive informational/correlative dependency between training inputs and the model’s internal representations or outputs \citep{wang_improving_2020, peng_bilateral_2022, ho_model_nodate}. 

To mitigate this hypothesized dependency, Mutual Information Defense (MID) \citep{wang_improving_2020} introduces a regularizer that reduces mutual information between the training examples and intermediate feature representations, arguing that this ``limit[s] the redundant information about the model input contained in the prediction" so that MIA's cannot ``exploit this correlation.'' Building on this idea, the current state-of-the-art Bilateral Dependency Optimizer (BiDO) algorithm \citep{peng_bilateral_2022} penalizes a kernel-based informational dependency measure (HSIC) between training examples and intermediate embeddings, arguing that this ``limits redundant information propagated from the inputs to the latent representations that can be exploited by the [MIA] adversary.'' 

Similarly, the recent and highly performant TL-DMI approach \citep{ho_model_nodate} advances a ``main hypothesis...that a model with fewer parameters encoding sensitive information from private training dataset'' contains less memorization vulnerable to MIA. This hypothesis is credited with the impressive practical performance of TL-DMI---a transfer-learning based approach that uses the training examples only for fine-tuning later layers of a pre-trained/public model.

The same hypothesis appears again in \textsc{SCA} \citep{dibbo_improving_2024}, which argues that the relevant training data vulnerability is reduced by directly ``control[ling] the amount of irrelevant private information encoded in a model's intermediate representations'', e.g., via sparse coding.

In sum, state-of-the-art defenses advance the theoretic argument that they obtain their practical performance against MIA by reducing memorization defined as informational dependency between training examples and the target model's latent representations/outputs.


\textcolor{red}{[DP-SGD Goodfellow $\rightarrow$ Hayes? Steinke? Guo on encodings? FAIR paper?]}



\textbf{Our contribution I: \  Challenging the theoretic bases of contemporary memorization/MIA defenses.}

In this paper, we challenge this foundational theoretic hypothesis.

\begin{enumerate}
\item First, we show that contemporary defenses that claim to prevent memorization/ MIA by reducing training-data-to-model dependency % do not in fact reduce this dependency, and may in fact increase it, even according to their own metrics. 
 \emph{do  not in fact reduce this dependency}, and may in fact increase it, in some cases even according to their own metrics.
%
\item  We construct a novel mask-based model that decimates input–output dependency by deleting $98\%$ of input pixels, and show it remains \emph{highly vulnerable} to MIA.
\textcolor{red}{Maybe consider adding FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we crush this hope with our DropLayer mask experiment that is an ineffective defense BECAUSE PPA/IFGMI use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it?}
%
\item Conversely, we show that a model that is said to perfectly memorize its training dataset is \emph{less} vulnerable to MIA than these state-of-the-art defenses.




\end{enumerate}

In sum, our experiments show that the main theoretic approach in memorization/MIA defense, while well-motivated, is incomplete; state-of-the-art memorization/MIA defenses, we argue, obtain their impressive performance by a different theoretic mechanism.

\textbf{Our contribution II:\\ The Invertability--Adversarial-Example tradeoff.}
 
 We probe these counterintuitive findings and discover a surprising result: 
 %recent defenses against inversion attacks actually work in part by unintentionally encouraging models to rely on what are elsewhere canonically known as “non-robust” features in the context of research on adversarial examples---that is, 
 recent defenses against inversion attacks actually work in part by unintentionally encouraging models to rely on what are elsewhere canonically known as “non-robust” features in the context of research on adversarial examples---that is, features that are generalizable, but imperceptible to humans and unstable under perturbation \citep{ilyas_adversarial_2019}\textcolor{red}{[Cite Ilya 2019, 2016, szegedy intriguing 2013, and the most influential follow-up papers from after Ilya 2019]}. “Non-robust” features are extremely well-studied in the context of adversarial examples and model robustness, but they are not known to be fundamentally connected to memorization/MIA.


% This shift disrupts gradient-based MIA attacks (which now face a fractured loss landscape), but it comes at a cost: the resulting `defended' models are substantially more vulnerable to adversarial examples. We provide the first systematic evaluation of adversarial robustness across MIA defenses, revealing this overlooked tradeoff.

To demonstrate this phenomenon, we conduct the first systematic evaluation of the robustness of memorization/MIA defenses to adversarial examples. 
 By unintentionally promoting this shift, MIA defenses disrupt gradient-based MIA attacks (which now face a fractured loss landscape), \textcolor{red}{[will be revised per July 24 mtng] and also reduce models' reliance on "robust features" that humans find visually/semantically meaningful, and that are captured in MIA reconstruction similarity metrics. This means that dependency-based MIA defenses obtain their performance at a previously overlooked cost: MIA defenses cause models to become far more vulnerable to adversarial examples.}


 \textcolor{red}{[make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with Adversarial Examples]}]


% To probe these counterintuitive results, we analyze the resulting models’ feature space geometry. Our findings suggest that instead of working by reducing training data dependency, recent defenses unintentionally work by “unsmoothing” the target model's feature space, forcing MIA attack gradients to traverse a volatile and brittle loss landscape reminiscent of overfitting.


\textbf{Our contribution III: \ \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining \\(\textsc{AT-AT}~\ATATicon) for superior memorization/MIA defense.}

If recent memorization/MIA defenses work by unintentionally `nonrobustifying' the model's feature space, then it stands to reason that we could obtain superior defense performance by deliberately exploiting this mechanism. To accomplish this, we design a novel class of memorization/MIA defenses that balance model accuracy with gradient steps that reverse standard adversarial training designed to promote robustness to adversarial examples. 
% "reverse"? maybe something more explicit/clear.
This simple technique allows us to deliberately compel models to learn non-robust-but-generalizable features that are semantically meaningless to humans (and thus limit visual reconstruction similarity under MIA), but that generalize as well as vanilla CNNs' features.

\textcolor{red}{non-robust features}

\textcolor{orange}{We call our approach \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining (\textsc{AT-AT}~\ATATicon)}

We show that our anti-adversarial approach outperforms baselines in terms of both model accuracy and standard MIA defense metrics \textcolor{red}{[PLACEHOLDER for specific outperformance factors or something impressive]} across various standard CNN architectures, datasets, and reconstruction metrics. As with other defenses, this performance comes at the cost of increased vulnerability to adversarial examples. However, in our case, this vulnerability cost is a tunable parameter, offering a new design axis for privacy-robust models.




\textbf{Codebase and Replication Materials.} \textcolor{red}{[Maybe include in intro since it's great marketing/we have a great codebase, it will look strong/confident since we are calling ppl out.}



\textbf{Questions for July 28 mtng.} \textcolor{purple}{Do we want to continue with the "available defenses claim to work via dependency reduction but all actually work via shifting models to rely on non-robust features, so we can exploit this deliberately with AT-AT" framing? Or do we want to more conservatively say "[Just] The best defense TL-DMI seems to work via shifting models to rely on non-robust features, and we notice that vanilla adversarial training does the opposite, so let's exploit this to do AT-AT" framing?}


\textbf{Some framing notes from July 28 mtng.} \textcolor{orange}{
Consider the Venn diagram of features that describe Adams (like an Adam class centroid in a perfect GAN) and the features that describe Adam's centroid in a good classifier. The former are descriptive; the latter are descriminative. You can have descriminative features that are a very small subset of the descriptive ones (small Venn overlap). Or maybe descriminative features are just a strict subset. Plug and play paper talks about features that matter to faces.\\
%
By doing non-robust features, we search for features in a small $\epsilon$ ball ergo humans cannot perceive and don't care. In practice, ATTACKS DONT CONVERGE but even if they do, we leak an imperceptible noise.\\\\
%
- HSIC is unrelated. Could be that HSIC doesn't capture the appropriate dependency measure, OR that dependency is just the wrong story. Suppose HSIC is just a bad measure, so then DropLayer should reduce dependency. BUT that doesn't work! So we need a new story. Should leave DropLayer and Permutation OUT of the HSIC table. \\\\
%
ALL Defenses are dropping robust features. Some (TL-DMI) are replacing them with non-robust to make up the accuracy. In the AutoAttack table, the accuracy under adv examples captures this...it either gets the example wrong because it sucks at classifying or because it was vulnerable to a small noise.\\\\
%
Adam: in intro talk less about screwing up gradients. Talk more about non-robust features.\\\\
%
Need to introduce and out-of-scope-ify the Neg-LS and Trap-MID or skip-connection defenses are like gradient masking. Trap-MID appendix is the only place they tried against PPA and it sucked and they had to cherry pick aka fine tune)\\\\
The new story is that dependency-based defenses delete robust features, and either take the concomitant accuracy penalty (BiDO) or replace them with non-robust features (TL-DMI).
}



\textbf{Paper organization.} \textcolor{red}{PLACEHOLDER.}

\section{\textcolor{red}{Preliminaries}} \textcolor{red}{PLACEHOLDER.}
\textbf{Threat model.}  \textcolor{red}{- white box because (1) we care about evaluating memorization in target models, and (2) we want strong defenses that are practically effective under strong adversaries with minimal assumptions.\\-Our experiments focus on vision because it's the central MIA research stream, though we intend to expand this in future work, and we include a codebase designed to facilitate this expansion }


\section{Model inversion attacks}
Consider a private training dataset $\mathcal{D}_{priv}=\{x_i,y_i\}_{i=1}^{N}$, where $x_i\in\mathbb{R}^{d_X}$, $y_i\in\{0,1\}^C$, and each $(x_i,y_i)$ are sampled i.i.d. from a joint distribution $\mathbb{P}_{XY}$. Let $T:\mathbb{R}^{d_X}\to\{0,1\}^C$ be a target model trained on $\mathcal{D}_{priv}$ that the adversary wishes to attack. To conduct a model inversion attack, an adversary seeks a new `inverted' model \textcolor{red}{$\hat{\mathcal{I}}_T$ [do we elsewhere denote it by something else? What do the best other ppl use? I like $\hat{\mathcal{I}}_T$ or maybe $\hat{T}'$]} that maps outputs of $T$, such as $T$'s softmax layer or intermediate outputs, back to the corresponding training examples in $\mathcal{D}_{priv}$. The adversary then queries $\hat{\mathcal{I}}_T$ to `predict' $T$'s private training examples. 

\textcolor{red}{note:    The goal in model inversion is to infer the class \emph{centroids} on the data manifold defined on all pixels/features. privacy leakage exists to the extent that these centroids permit reconstruction of features we `care about' (rather than features that are class-descriminative-but not-otherwise-interesting stuff... \ \ The goal of Model Inversion Defense is to build models that infer decision boundaries without leaking information about the training examples via their class centroids, or that are impervious to having their class centroids re-inferred by an attacker.}

Early MIA's trained the inverted model $\hat{\mathcal{I}}_T$ from scratch by using SGD to directly optimize reconstructions of individual training examples \citep{fredrikson2015model}. However, this approach suffers from various optimization complexities when applied to contemporary vision architectures like deep CNN's. Therefore, recent state-of-the-art attacks simplify optimization by adopting an `image prior'---that is, by restricting the search space of training example reconstructions to the image outputs of a domain-relevant GAN, and conducting SGD-based optimization on the GAN's input noise vectors instead of directly on the high-dimensional images' feature space \cite{zhang_secret_2020}. More specifically, GAN-based MIA's optimize a latent noise vector $\hat{z} \in Z$ such that the resultant GAN-generated image is classified as class $c$ maximized confidence by the target model $T$:
%
$$\min_{\hat{z}} \mathcal{L}(T, G, D, \hat{z}, c)$$ 
%
where $\mathcal{L}$ is a standard loss function (e.g. cross-entropy) to maximize the confidence of the GAN-generated image on class $c$,  given pretrained GAN generator $G:Z \to X_{prior}$ and GAN discriminator $D$. Recent attacks on facial recognition classifiers take advantage of pretrained GANs like StyleGAN to perform far more efficient and accurate training data reconstructions \citep{struppek_plug_2022, qiu_closer_2024}. \textcolor{red}{[Mention in the body of the paper that App. \ref{mia-related-work-supp} gives details of SOTA MIA attacks.]}

==> dareDEVALII/Sections/old_SEC_INTRO_3rdcut.tex <==


\section{Introduction}


A foundational goal of contemporary machine learning is to learn \emph{generalizable} model parameters from the training data without \emph{exposing} training data examples to leakage. However, it is well known that virtually all modern architectures obtain generalizable performance only at the cost of encoding a substantial amount of sensitive information about their training examples. This tradeoff defines a critical research frontier in terms of the efficiency of current training regimes and learned representations. It also compromises model privacy by providing a key practical vulnerability that is exploited by myriad new attacks.




% \textbf{Training data exposure reveals fundamental gaps in learning.} 

% Venn diagram First, in the era of billion dollar training expenditures, backpropagating to learn idiosyncratic, ungeneralizable training example information reflects a fundamental learning inefficiency that continues to accrue costs when ungeneralizable parameters are called at inference time \textcolor{red}{[Cite a bunch of papers]}.







% The tendency of contemporary machine learning models to expose their private training data has recently emerged as a critical research and security frontier. A foundational goal of machine learning is to obtain an \emph{efficient} and \emph{generalizable} set of model parameters. However, it is well-known that virtually all modern architectures also unintentionally encode a substantial amount of sensitive information about their training data. This tradeoff reveals a fundamental deficit in terms of the efficiency of current training regimes and learned representations. It also compromises model privacy by providing a key practical vulnerability that is exploited by myriad new attacks.

\textbf{Training data exposure reveals fundamental gaps in learning.} % Venn diagram

 \textbf{Training data exposure undermines privacy in ML deployments.}
Second, training data exposure underlies a rapidly expanding class of practical privacy attacks that reconstruct private training data from real-world machine learning deployments simply by querying models or inspecting their parameters. Recent variants of training data attacks apply not only to CNN's, but also to LLM's, diffusion models, multimodal models, etc. \textcolor{red}{[Cite membership inference, attribute inference, carlini's extraction attacks on text LLM's and on stable diffusion].}



\textbf{Model inversion attacks (MIA's) probe and exploit training data exposure.} 
In particular, model inversion attacks (MIA's) have become a mainstream tool for studying and evaluating training data exposure. Unlike more conservative attacks that merely test for the presence of some exposed training examples, MIAs test the degree to which a powerful attacker armed with white-box model access and significant computational resources can reconstruct the full set of class-level features for each class in the training data. 

\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }



%While the success of MIA's demonstrates the existence of memorized training examples in contemporary models, 
While MIA's lower-bound the extent to which training data is vulnerable to reconstruction, they do not explain what aspect of trained models encodes this vulnerability, or how to prevent it. \textcolor{purple}{This raises a fundamental question:}


\begingroup
\addtolength\leftmargini{-0.15in} % shrink quote margin
\begin{quote}
%\vspace{-2mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null\\[-2.5mm]
\begin{center}
\vspace{-5mm}
 \textit{How is the training data exposure vulnerability encoded in contemporary models?}
 \vspace{-1mm}
\end{center}
\vspace{-2.5mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null
%\vspace{-2mm}
\end{quote}
\endgroup


\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }

\textbf{The prevailing `training data exposure = memorization' theory.} 

% Edit this following DP paragraph bc DP is basically in the memorization vein since it's about how much the global statistic shares info about its component observations
\textbf{Classical privacy frameworks like DP do not explain the training data exposure that MIA's exploit.}
While classical privacy frameworks such as Differential Privacy (DP) \cite{dwork2006differential, dwork2014algorithmic} offer provable guarantees against training example exposure \citep{hayes_bounding_2023}, they do not explain why it arises in contemporary learning settings. 
DP was designed to protect the privacy of individual training examples while releasing parameters that characterize in-sample group-level descriptive statistics. These competing goals have a direct information-theoretic tradeoff. 
% DP was designed to control the direct information-theoretic tradeoff between the privacy of individual training examples we want to protect and the accuracy of in-sample group-level statistics we want to release.
However, the same direct tradeoff does not obviously apply to releasing model parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning).
%It does not directly apply when releasing parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning), where it is not obvious how such a tradeoff applies. 
As a result, extending DP-based protections to learning applications may be sufficient to protect the training data from exposure, but they may be unnecessary for this goal, and their very high computational and accuracy costs render them practically inapplicable in large-scale learning deployments.

\textbf{Recent learning theory underscores a theoretic deficit.}
To address the theoretic gap left by DP, a very recent stream of theoretic work seeks novel noise-based techniques that upper-bound the degree to which training data can be reconstructed by any unbiased estimator. Nonetheless, as we demonstrate, that approach may provide a false sense of security: 
\textcolor{red}{\textbf{FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein} have recent bounds that also use noise and try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we crush this hope with our DropLayer mask and PPA/IFGMI use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it? Or below?}




\textbf{State-of-the-art defenses theorize that MIA's reveal and exploit memorization in the form of direct data-to-model dependencies.}
An influential recent line of algorithms have obtained practically performant defenses against training data exposure/MIA, and argued that their practical performance can be attributed to their shared theoretic hypothesis that MIA vulnerability arises from direct and excessive informational/correlative dependency between training inputs and the model’s internal representations or outputs \citep{wang_improving_2020, peng_bilateral_2022, ho_model_nodate}. 

To mitigate this hypothesized dependency, Mutual Information Defense (MID) \citep{wang_improving_2020} introduces a regularizer that reduces mutual information between the training examples and intermediate feature representations, arguing that this ``limit[s] the redundant information about the model input contained in the prediction" so that MIA's cannot ``exploit this correlation.'' Building on this idea, the current state-of-the-art Bilateral Dependency Optimizer (BiDO) algorithm \citep{peng_bilateral_2022} penalizes a kernel-based informational dependency measure (HSIC) between training examples and intermediate embeddings, arguing that this ``limits redundant information propagated from the inputs to the latent representations that can be exploited by the [MIA] adversary.'' 

Similarly, the recent and highly performant TL-DMI approach \citep{ho_model_nodate} advances a ``main hypothesis...that a model with fewer parameters encoding sensitive information from private training dataset'' contains less memorization vulnerable to MIA. This hypothesis is credited with the impressive practical performance of TL-DMI---a transfer-learning based approach that uses the training examples only for fine-tuning later layers of a pre-trained/public model.

The same hypothesis appears again in \textsc{SCA} \citep{dibbo_improving_2024}, which argues that the relevant training data vulnerability is reduced by directly ``control[ling] the amount of irrelevant private information encoded in a model's intermediate representations'', e.g., via sparse coding.

In sum, state-of-the-art defenses advance the theoretic argument that they obtain their practical performance against MIA by reducing memorization defined as informational dependency between training examples and the target model's latent representations/outputs.


\textcolor{red}{[DP-SGD Goodfellow $\rightarrow$ Hayes? Steinke? Guo on encodings? FAIR paper?]}



\textbf{Our contribution I: \  Challenging the theoretic bases of contemporary memorization/MIA defenses.}

In this paper, we challenge this foundational theoretic hypothesis.

\begin{enumerate}
\item First, we show that contemporary defenses that claim to prevent memorization/ MIA by reducing training-data-to-model dependency % do not in fact reduce this dependency, and may in fact increase it, even according to their own metrics. 
 \emph{do  not in fact reduce this dependency}, and may in fact increase it, in some cases even according to their own metrics.
%
\item  We construct a novel mask-based model that decimates input–output dependency by deleting $98\%$ of input pixels, and show it remains \emph{highly vulnerable} to MIA.
\textcolor{red}{Maybe consider adding FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we crush this hope with our DropLayer mask experiment that is an ineffective defense BECAUSE PPA/IFGMI use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it?}
%
\item Conversely, we show that a model that is said to perfectly memorize its training dataset is \emph{less} vulnerable to MIA than these state-of-the-art defenses.




\end{enumerate}

In sum, our experiments show that the main theoretic approach in memorization/MIA defense, while well-motivated, is incomplete; state-of-the-art memorization/MIA defenses, we argue, obtain their impressive performance by a different theoretic mechanism.

\textbf{Our contribution II:\\ The Invertability--Adversarial-Example tradeoff.}
 
 We probe these counterintuitive findings and discover a surprising result: 
 %recent defenses against inversion attacks actually work in part by unintentionally encouraging models to rely on what are elsewhere canonically known as “non-robust” features in the context of research on adversarial examples---that is, 
 recent defenses against inversion attacks actually work in part by unintentionally encouraging models to rely on what are elsewhere canonically known as “non-robust” features in the context of research on adversarial examples---that is, features that are generalizable, but imperceptible to humans and unstable under perturbation \citep{ilyas_adversarial_2019}\textcolor{red}{[Cite Ilya 2019, 2016, szegedy intriguing 2013, and the most influential follow-up papers from after Ilya 2019]}. “Non-robust” features are extremely well-studied in the context of adversarial examples and model robustness, but they are not known to be fundamentally connected to memorization/MIA.


% This shift disrupts gradient-based MIA attacks (which now face a fractured loss landscape), but it comes at a cost: the resulting `defended' models are substantially more vulnerable to adversarial examples. We provide the first systematic evaluation of adversarial robustness across MIA defenses, revealing this overlooked tradeoff.

To demonstrate this phenomenon, we conduct the first systematic evaluation of the robustness of memorization/MIA defenses to adversarial examples. 
 By unintentionally promoting this shift, MIA defenses disrupt gradient-based MIA attacks (which now face a fractured loss landscape), \textcolor{red}{[will be revised per July 24 mtng] and also reduce models' reliance on "robust features" that humans find visually/semantically meaningful, and that are captured in MIA reconstruction similarity metrics. This means that dependency-based MIA defenses obtain their performance at a previously overlooked cost: MIA defenses cause models to become far more vulnerable to adversarial examples.}


 \textcolor{red}{[make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with Adversarial Examples]}]


% To probe these counterintuitive results, we analyze the resulting models’ feature space geometry. Our findings suggest that instead of working by reducing training data dependency, recent defenses unintentionally work by “unsmoothing” the target model's feature space, forcing MIA attack gradients to traverse a volatile and brittle loss landscape reminiscent of overfitting.


\textbf{Our contribution III: \ \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining \\(\textsc{AT-AT}~\ATATicon) for superior memorization/MIA defense.}

If recent memorization/MIA defenses work by unintentionally `nonrobustifying' the model's feature space, then it stands to reason that we could obtain superior defense performance by deliberately exploiting this mechanism. To accomplish this, we design a novel class of memorization/MIA defenses that balance model accuracy with gradient steps that reverse standard adversarial training designed to promote robustness to adversarial examples. 
% "reverse"? maybe something more explicit/clear.
This simple technique allows us to deliberately compel models to learn non-robust-but-generalizable features that are semantically meaningless to humans (and thus limit visual reconstruction similarity under MIA), but that generalize as well as vanilla CNNs' features.

\textcolor{red}{non-robust features}

\textcolor{orange}{We call our approach \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining (\textsc{AT-AT}~\ATATicon)}

We show that our anti-adversarial approach outperforms baselines in terms of both model accuracy and standard MIA defense metrics \textcolor{red}{[PLACEHOLDER for specific outperformance factors or something impressive]} across various standard CNN architectures, datasets, and reconstruction metrics. As with other defenses, this performance comes at the cost of increased vulnerability to adversarial examples. However, in our case, this vulnerability cost is a tunable parameter, offering a new design axis for privacy-robust models.




\textbf{Codebase and Replication Materials.} \textcolor{red}{[Maybe include in intro since it's great marketing/we have a great codebase, it will look strong/confident since we are calling ppl out.}



\textbf{Questions for July 28 mtng.} \textcolor{purple}{Do we want to continue with the "available defenses claim to work via dependency reduction but all actually work via shifting models to rely on non-robust features, so we can exploit this deliberately with AT-AT" framing? Or do we want to more conservatively say "[Just] The best defense TL-DMI seems to work via shifting models to rely on non-robust features, and we notice that vanilla adversarial training does the opposite, so let's exploit this to do AT-AT" framing?}


\textbf{Some framing notes from July 28 mtng.} \textcolor{orange}{
Consider the Venn diagram of features that describe Adams (like an Adam class centroid in a perfect GAN) and the features that describe Adam's centroid in a good classifier. The former are descriptive; the latter are descriminative. You can have descriminative features that are a very small subset of the descriptive ones (small Venn overlap). Or maybe descriminative features are just a strict subset. Plug and play paper talks about features that matter to faces.\\
%
By doing non-robust features, we search for features in a small $\epsilon$ ball ergo humans cannot perceive and don't care. In practice, ATTACKS DONT CONVERGE but even if they do, we leak an imperceptible noise.\\\\
%
- HSIC is unrelated. Could be that HSIC doesn't capture the appropriate dependency measure, OR that dependency is just the wrong story. Suppose HSIC is just a bad measure, so then DropLayer should reduce dependency. BUT that doesn't work! So we need a new story. Should leave DropLayer and Permutation OUT of the HSIC table. \\\\
%
ALL Defenses are dropping robust features. Some (TL-DMI) are replacing them with non-robust to make up the accuracy. In the AutoAttack table, the accuracy under adv examples captures this...it either gets the example wrong because it sucks at classifying or because it was vulnerable to a small noise.\\\\
%
Adam: in intro talk less about screwing up gradients. Talk more about non-robust features.\\\\
%
Need to introduce and out-of-scope-ify the Neg-LS and Trap-MID or skip-connection defenses are like gradient masking. Trap-MID appendix is the only place they tried against PPA and it sucked and they had to cherry pick aka fine tune)\\\\
The new story is that dependency-based defenses delete robust features, and either take the concomitant accuracy penalty (BiDO) or replace them with non-robust features (TL-DMI).
}



\textbf{Paper organization.} \textcolor{red}{PLACEHOLDER.}

\section{\textcolor{red}{Preliminaries}} \textcolor{red}{PLACEHOLDER.}
\textbf{Threat model.}  \textcolor{red}{- white box because (1) we care about evaluating memorization in target models, and (2) we want strong defenses that are practically effective under strong adversaries with minimal assumptions.\\-Our experiments focus on vision because it's the central MIA research stream, though we intend to expand this in future work, and we include a codebase designed to facilitate this expansion }


\section{Model inversion attacks}
Consider a private training dataset $\mathcal{D}_{priv}=\{x_i,y_i\}_{i=1}^{N}$, where $x_i\in\mathbb{R}^{d_X}$, $y_i\in\{0,1\}^C$, and each $(x_i,y_i)$ are sampled i.i.d. from a joint distribution $\mathbb{P}_{XY}$. Let $T:\mathbb{R}^{d_X}\to\{0,1\}^C$ be a target model trained on $\mathcal{D}_{priv}$ that the adversary wishes to attack. To conduct a model inversion attack, an adversary seeks a new `inverted' model \textcolor{red}{$\hat{\mathcal{I}}_T$ [do we elsewhere denote it by something else? What do the best other ppl use? I like $\hat{\mathcal{I}}_T$ or maybe $\hat{T}'$]} that maps outputs of $T$, such as $T$'s softmax layer or intermediate outputs, back to the corresponding training examples in $\mathcal{D}_{priv}$. The adversary then queries $\hat{\mathcal{I}}_T$ to `predict' $T$'s private training examples. 

\textcolor{red}{note:    The goal in model inversion is to infer the class \emph{centroids} on the data manifold defined on all pixels/features. privacy leakage exists to the extent that these centroids permit reconstruction of features we `care about' (rather than features that are class-descriminative-but not-otherwise-interesting stuff... \ \ The goal of Model Inversion Defense is to build models that infer decision boundaries without leaking information about the training examples via their class centroids, or that are impervious to having their class centroids re-inferred by an attacker.}

Early MIA's trained the inverted model $\hat{\mathcal{I}}_T$ from scratch by using SGD to directly optimize reconstructions of individual training examples \citep{fredrikson2015model}. However, this approach suffers from various optimization complexities when applied to contemporary vision architectures like deep CNN's. Therefore, recent state-of-the-art attacks simplify optimization by adopting an `image prior'---that is, by restricting the search space of training example reconstructions to the image outputs of a domain-relevant GAN, and conducting SGD-based optimization on the GAN's input noise vectors instead of directly on the high-dimensional images' feature space \cite{zhang_secret_2020}. More specifically, GAN-based MIA's optimize a latent noise vector $\hat{z} \in Z$ such that the resultant GAN-generated image is classified as class $c$ maximized confidence by the target model $T$:
%
$$\min_{\hat{z}} \mathcal{L}(T, G, D, \hat{z}, c)$$ 
%
where $\mathcal{L}$ is a standard loss function (e.g. cross-entropy) to maximize the confidence of the GAN-generated image on class $c$,  given pretrained GAN generator $G:Z \to X_{prior}$ and GAN discriminator $D$. Recent attacks on facial recognition classifiers take advantage of pretrained GANs like StyleGAN to perform far more efficient and accurate training data reconstructions \citep{struppek_plug_2022, qiu_closer_2024}. \textcolor{red}{[Mention in the body of the paper that App. \ref{mia-related-work-supp} gives details of SOTA MIA attacks.]}

==> dareDEVALII/Sections/old_SEC_INTRO_EPISODE_VII_the_force_awakens.tex <==
\textcolor{green}{NOTES: training privacy vulnerability is ascribed to memorization across various SOTA models like LLM, diffusion, classification, etc.\\\\
% 
Memorization can refer to a variety of related concepts but in the context of MI, defenses are trying to minimize the explicit dependency of training data that are “rote encoded” into the model such inputs and embeddings have high joint HSIC, MI, etc.\\\\
% 
In the appendix, we can hide a paragraph of quotes about memorization since some reviewer will certainly attack some aspect of the fact that the concept of memorization is vague, and it’s not clear that a fully memorized model relates to a high HSIC model or something.
}

\textcolor{purple}{
A dominant view in privacy research is that models leak information about their private training data because they memorize it. This premise underlies recent theoretical bounds and many practical defenses against reconstruction attacks. At the same time, a recent stream of results has linked memorization to the performance of modern architectures. This work conjectures that strong generalization may require near-total memorization of the training set for classic learning settings CITES as well as novel paradigms like LLM's and diffusion \citep{carlini_extracting_2023, shah_does_2025}. These claims suggest an uncomfortable tradeoff: the mechanism believed to drive privacy exposure is also theorized to drive next-generation performance.\\\\
%
In this paper, we show that this view is incomplete. In a surprising series of experiments, we find that: (1) state-of-the-art reconstruction defenses widely believed to work by reducing data-to-model dependency do not reduce standard memorization metrics, sometimes they increase them; (2) models that perfectly memorize their training sets can nonetheless be resistant to model inversion attacks; and (3) models trained without access to 98\% of input pixels—settings where recent information-theoretic results guarantee unreconstructability under standard unbiased estimator assumptions—remain highly vulnerable to modern inversion attacks. Together, these findings indicate that memorization alone does not explain training-data reconstruction.\\\\
%
We propose a different mechanism: feature basis. Among the most celebrated results in machine learning is that adversarial examples are not bugs, but non-robust features \citep{ilyas_adversarial_2019}. These features are predictive and generalizable, yet visually imperceptible and unstable to small perturbations. We argue that these properties make them ideal instruments for privacy-preserving learning, where the goal is to classify accurately without encoding visually meaningful information that attackers can reconstruct. More specifically, we argue that current state-of-the-art privacy defenses already unintentionally work in part by shifting models’ feature basis away from robust, human-aligned features, and in some cases toward non-robust features. Our argument challenges the widely held view that they instead work only by reducing memorization. Second, we show that this shift toward non-robust features can be induced deliberately to obtain superior privacy.\\\\
%
Building on this insight, we introduce Anti-Adversarial Training (AT-AT), a defense that explicitly tunes the feature basis. Unlike standard adversarial training, which promotes reliance on robust features, AT-AT applies targeted updates that suppress robust features and encourage non-robust—but still generalizable—features that hinder visual reconstruction. Across standard CNN benchmarks and evaluation metrics for model inversion, AT-AT achieves stronger protection than state-of-the-art defenses while matching or improving accuracy. As expected, shifting toward non-robust features increases vulnerability to adversarial examples, but in our framework this cost is a controllable parameter, revealing a practical privacy–robustness tradeoff.\\\\
}



\textcolor{gray}{
Among the most celebrated results in machine learning is the finding that adversarial examples are not bugs, but `non-robust features' \citep{ilyas_adversarial_2019}. In other words, adversarial examples reveal features that are generalizable and class-discriminative, but visually imperceptible to humans. In this paper, we argue that these properties make them ideal instruments for privacy-preserving learning, where the goal is to classify accurately without encoding visually meaningful information that can be exploited for training-data reconstruction.\\\\
%
More specifically, we first argue that current state-of-the-art training data privacy defenses already unintentionally work in part by shifting the model's feature basis away from robust features, and in some cases, towards non-robust features. Our argument challenges the widely held view that they work only by reducing memorization. Second, we show that we can deliberately induce this shift towards non-robust features to obtain superior privacy.
}



==> dareDEVALII/Sections/old_SEC_INTRO_IV.tex <==


\section{Introduction}

% The tendency of contemporary machine learning models to expose their private training data has recently emerged as a critical performance and security frontier.

A foundational goal of contemporary machine learning is to learn \emph{generalizable} model parameters from the training data without \emph{exposing} training data examples to leakage. However, it is well-known that virtually all modern architectures obtain generalizable performance only at the cost of encoding a substantial amount of sensitive information about their training examples.  



\textbf{Understanding this training data encoding and exposure is expected to be a key to next-generation model performance.} % Venn diagram 
A variety of recent work shows that this tradeoff is deeply connected to the efficiency of current training regimes and the performance of contemporary architectures.
%Multiple research streams advance conflicting views on whether the encoding and exposure of training data in model parameters hinders or enhances performance. 
% In classic ML, backpropagating to capture idiosyncratic, ungeneralizable training data details is a well-known performance pitfall that is extensively studied in the context of overfitting. However, in the context of novel generative paradigms such as diffusion models, influential recent work has conjectured that stronger performance may require \emph{more} training data exposure, up to and including rote memorization of the training set \citep[e.g.,][]{carlini2023extracting, c.f., shah2025memorization}. Reconciling these perspectives is key to understanding the mechanics that will shape the next generation of high-performance models.
For example, in the context of novel generative paradigms such as diffusion models, influential recent work has conjectured that stronger performance may require \emph{more} training data exposure, up to and including rote memorization of the training set \citep[e.g.,][]{carlini2023extracting, c.f., shah2025memorization}. 
\textcolor{orange}{and LLM's? https://arxiv.org/abs/2205.10770}
\textcolor{blue}{and Apple research generic ML stuff: https://dl.acm.org/doi/pdf/10.1145/3406325.3451131}
\textcolor {green}{and self supervised learning: https://arxiv.org/pdf/2401.12233}
\textcolor{red}{maybe: https://arxiv.org/html/2507.04782v1}
These conjectures stand in contrast to classic ML research on overfitting, where backpropagating to capture idiosyncratic, ungeneralizable training data details is a well-studied as a performance pitfall. Reconciling these perspectives is key to understanding the mechanics that will shape the next generation of high-performance models.


 \textbf{Training data exposure undermines privacy in ML deployments.}
Training data exposure also underlies a rapidly expanding class of practical privacy attacks that reconstruct private training data from real-world machine learning deployments simply by querying models or inspecting their parameters. Recent variants of training data attacks apply not only to CNN's, but also to LLM's, diffusion models, multimodal models, etc. \textcolor{red}{[Cite membership inference, attribute inference, carlini's extraction attacks on text LLM's and on stable diffusion].}




\textbf{Model inversion attacks (MIA's) probe and exploit training data exposure.} 
In particular, model inversion attacks (MIA's) have become a mainstream tool for studying and evaluating training data exposure. Unlike more conservative attacks that merely test for the presence of some exposed training examples, MIAs test the degree to which a powerful attacker armed with white-box model access and significant computational and data resources can reconstruct information from the training examples. While early MIA's applied SGD to directly optimize reconstructions of individual training examples \citep{fredrikson2015model}, contemporary MIA's leverage state-of-the-art pretrained models to attempt to infer the full set of class-level characteristics for each class in the training data. 


\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }


However, while MIA's lower-bound the extent to which training data information is vulnerable to reconstruction, they do not explain what aspect of trained models encodes this vulnerability, or how to prevent it. This raises a fundamental question:


\begingroup
\addtolength\leftmargini{-0.15in} % shrink quote margin
\begin{quote}
%\vspace{-2mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null\\[-2.5mm]
\begin{center}
\vspace{-5mm}
 \textit{What properties of learned representations encode vulnerability to training data leakage and reconstruction, and how can they be controlled?}
 \vspace{-1mm}
\end{center}
\vspace{-2.5mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null
%\vspace{-2mm}
\end{quote}
\endgroup


\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }

\textbf{The prevailing `training data exposure = memorization' theory.} 


\textbf{State-of-the-art defenses theorize that MIA's reveal and exploit memorization in the form of direct data-to-model dependencies.}
An influential recent line of algorithms have obtained practically performant defenses against training data exposure/MIA, and it is widely believed that their practical performance can be attributed to their shared theoretic hypothesis that MIA vulnerability arises from direct and excessive informational/correlative dependency between training inputs and the model’s internal representations or outputs \citep{wang_improving_2020, peng_bilateral_2022, ho_model_nodate}. 

To mitigate this hypothesized dependency, Mutual Information Defense (MID) \citep{wang_improving_2020} introduces a regularizer that reduces mutual information between the training examples and intermediate feature representations, arguing that this ``limit[s] the redundant information about the model input contained in the prediction" so that MIA's cannot ``exploit this correlation.'' Building on this idea, the current state-of-the-art Bilateral Dependency Optimizer (BiDO) algorithm \citep{peng_bilateral_2022} penalizes a kernel-based informational dependency measure (HSIC) between training examples and intermediate embeddings, arguing that this ``limits redundant information propagated from the inputs to the latent representations that can be exploited by the [MIA] adversary.'' 

Similarly, the recent and highly performant TL-DMI approach \citep{ho_model_nodate} advances a ``main hypothesis...that a model with fewer parameters encoding sensitive information from private training dataset'' contains less memorization vulnerable to MIA. This hypothesis is credited with the impressive practical performance of TL-DMI---a transfer-learning based approach that uses the training examples only for fine-tuning later layers of a pre-trained/public model.

The same hypothesis appears again in \textsc{SCA} \citep{dibbo_improving_2024}, which argues that the relevant training data vulnerability is reduced by directly ``control[ling] the amount of irrelevant private information encoded in a model's intermediate representations'', e.g., by sparse-coding training examples before they are seen by the model, and also sparse-coding intermediate layers.

In sum, state-of-the-art defenses advance the theoretic argument that they obtain their practical performance against MIA by reducing memorization defined as informational dependency between training examples and the target model's latent representations/outputs.


\textcolor{red}{[DP-SGD Goodfellow $\rightarrow$ Hayes? Steinke? Guo on encodings? FAIR paper?]}



\textbf{Our contribution I: \  Challenging the theoretic bases of contemporary memorization/MIA defenses.}

In this paper, we challenge this foundational hypothesis.

\begin{enumerate}
\item First, we show that contemporary defenses that are widely believed to prevent memorization/MIA by reducing training-data-to-model dependency % do not in fact reduce this dependency, and may in fact increase it, even according to their own metrics. 
 \emph{do  not in fact reduce this dependency}, and may in fact increase it, in some cases even according to their own metrics.
%
\item  We construct a novel mask-based model that decimates memorization qua input–output dependency by deleting $98\%$ of input pixels, such that the model never sees them (and thus cannot memorize them), and we show it remains \emph{highly vulnerable} to MIA.
\textcolor{red}{Maybe consider adding FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we crush this hope with our DropLayer mask experiment that is an ineffective defense BECAUSE PPA/IFGMI use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it?}
%
\item Conversely, we show that a model that is said to completely memorize its training dataset is \emph{less} vulnerable to MIA than these state-of-the-art defenses.




\end{enumerate}

In sum, our experiments show that the main theoretic approach in memorization/MIA defense, while well-motivated, is incomplete; state-of-the-art memorization/MIA defenses, we argue, obtain their impressive performance by a different theoretic mechanism.

% \textbf{Our contribution II:\\ The Invertability--Adversarial-Example tradeoff.}
 
%  We probe these counterintuitive findings and discover a surprising result: 
%  Recent defenses hinder reconstruction in part by unintentionally shifting models away from what are known in the adversarial examples literature as “robust features" and, in some cases, toward ``non-robust features" (i.e., features that are generalizable, but imperceptible to humans and unstable under perturbation). \citep{ilyas_adversarial_2019}\textcolor{red}{[Cite Ilya 2019, 2016, szegedy intriguing 2013, and the most influential follow-up papers from after Ilya 2019]}. “Non-robust” features are extremely well-studied in the context of adversarial examples and model robustness, but they are not known to be fundamentally connected to memorization/MIA.

% \textbf{Our Contribution II: The Privacy–Robustness Feature Tradeoff.}

% Our results reveal a previously unrecognized mechanism by which state-of-the-art defenses alter the feature basis of learned representations, establishing a direct link to canonical findings in adversarial example robustness. Specifically, we find that recent defenses hinder reconstruction in part suppressing their model's reliance on robust features (i.e., features that are stable under human-imperceptible perturbations and that align with human-interpretable semantics), and in some cases, replacing them with non-robust features (i.e., features that generalize well but are imperceptible to humans and highly unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}.

% Our results reveal a previously unrecognized mechanism by which state-of-the-art defenses against privacy leakage alter the feature basis of learned representations, thereby establishing a direct link to canonical findings in adversarial example robustness. Contrary to the prevailing view that these defenses primarily protect against reconstruction by reducing direct data–model dependency, we find that they actually hinder reconstructions by reshaping the learned representation space: they suppress reliance on ``robust features'' (i.e., generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics), and in some cases, replacing them with ``non-robust features'' (i.e., features that generalize well but are imperceptible to humans and unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}. This shift has a dual effect: suppressing robust features hurts model accuracy. Replacing robust features with non-robust ones compensates for the accuracy loss, at the cost of brittleness, leaving models far more vulnerable to adversarial examples. While robust vs. non-robust feature reliance is extensively studied in adversarial example research, its role as a governing factor in training data exposure vulnerability has not previously been identified.

\textbf{Our contribution II: The privacy-robustness feature tradeoff.}

We uncover a previously unknown mechanism that directly links training data exposure vulnerabilities to the well-studied robust–non-robust feature tradeoff from adversarial robustness. To probe this phenomenon, we conduct the first systematic evaluation of the robustness of memorization/MIA defenses to adversarial examples. Our analysis reveals that state-of-the-art privacy defenses do not primarily protect against reconstruction by reducing direct data–model dependency, as widely assumed. Instead, they operate by reshaping the learned feature basis. Specifically, they protect privacy by unintentionally suppressing reliance on ``robust features'' (i.e., generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics), and in some cases, replacing them with ``non-robust features'' (i.e., features that generalize well but are imperceptible to humans and unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}. This shift yields a tradeoff: suppressing robust features strips semantically meaningful information from the model but degrades accuracy, while replacing robust features with non-robust features recovers accuracy at the cost of brittleness, leaving models vulnerable to adversarial examples. Although robust–non-robust feature reliance is heavily studied in adversarial robustness, our work is the first to show its central role in training data privacy vulnerabilities. 

% We uncover a previously unknown mechanism that directly links training data exposure vulnerabilities to the well-studied robust–non-robust feature tradeoff from adversarial robustness. State-of-the-art privacy defenses do not primarily protect against reconstruction by reducing direct data–model dependency, as widely assumed. Instead, they operate by reshaping the learned feature basis: unintentionally suppressing robust features—generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics—and, in some cases, replacing them with non-robust features—features that generalize well but are imperceptible to humans and unstable under perturbation \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}.



%
 % By unintentionally promoting this shift, MIA defenses disrupt gradient-based MIA attacks (which now face a fractured loss landscape), \textcolor{red}{[will be revised per July 24 mtng] and also reduce models' reliance on "robust features" that humans find visually/semantically meaningful, and that are captured in MIA reconstruction similarity metrics. This means that dependency-based MIA defenses obtain their performance at a previously overlooked cost: MIA defenses cause models to become far more vulnerable to adversarial examples.}


 \textcolor{red}{[make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with Adversarial Examples]}]




\textbf{Our contribution III: \ \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining \\(\textsc{AT-AT}~\ATATicon) for superior privacy/MIA defense.}

If recent memorization/MIA defenses work by unintentionally `nonrobustifying' the model's feature space, then it stands to reason that we could obtain superior defense performance by deliberately exploiting this mechanism. 
%
To accomplish this, we introduce  \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining (\textsc{AT-AT}~\ATATicon), a novel class of memorization/MIA defenses that balance model accuracy with gradient steps that reverse standard adversarial training.  
Rather than promoting robustness to adversarial perturbations, \textsc{AT-AT} applies targeted gradient updates that suppress reliance on robust features, compelling the model to instead learn non-robust—but still generalizable—features that are semantically meaningless to humans and thereby hinder visual reconstruction under MIA.
% "reverse"? maybe something more explicit/clear.
% This simple technique allows us to deliberately compel models to learn non-robust-but-generalizable features that are semantically meaningless to humans (and thus limit visual reconstruction similarity under MIA), but that generalize as well as vanilla CNNs' features.

% \textcolor{red}{non-robust features}

We show that our anti-adversarial approach outperforms baselines in terms of \emph{both} model accuracy and standard MIA defense metrics \textcolor{red}{[PLACEHOLDER for specific outperformance factors or something impressive]} across various standard CNN architectures, datasets, and reconstruction metrics. As with other defenses, this performance comes at the cost of increased vulnerability to adversarial examples. However, in our case, this vulnerability cost is a tunable parameter, offering a new design axis for privacy-robust models.



% Edit this following DP paragraph bc DP is basically in the memorization vein since it's about how much the global statistic shares info about its component observations
\textbf{Privacy implications}
Our results indicate that learning too many descriptive features is a privacy vulnerability distinct from anything that can reasonably be called “memorization.” In this view, a model does not leak information like a camera that stores pixel-perfect images of its training data, but rather like a crime eyewitness: even without taking pictures, the witness can recall and describe enough private details for a skilled sketch artist armed with prior information about faces (i.e., the MIA attacker) to reconstruct a convincing likeness.

%Reconstruction vulnerability is present even absent seeing pixels.


For completeness, we note that another stream of recent defenses in the literature do not seek to address the underlying privacy vulnerability at all, but instead interfere with specific MIA attack implementations (e.g., by making the loss landscape unamenable to gradients taken in the most popular MIA attacks).\textbf{red}{label smoothing; trapdoor}. %We include the most popular of these defenses in our experiments, but they are otherwise outside our scope, as they target the mechanics of specific attacks rather than seeking to explore the underlying privacy vulnerability.





\textbf{Classical privacy frameworks like DP do not explain the training data exposure that MIA's exploit.}
While classical privacy frameworks such as Differential Privacy (DP) \cite{dwork2006differential, dwork2014algorithmic} offer provable guarantees against training example exposure \citep{hayes_bounding_2023}, they do not explain why it arises in contemporary learning settings. 
DP was designed to protect the privacy of individual training examples while releasing parameters that characterize in-sample group-level descriptive statistics. These competing goals have a direct information-theoretic tradeoff. 
% DP was designed to control the direct information-theoretic tradeoff between the privacy of individual training examples we want to protect and the accuracy of in-sample group-level statistics we want to release.
However, the same direct tradeoff does not obviously apply to releasing model parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning).
%It does not directly apply when releasing parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning), where it is not obvious how such a tradeoff applies. 
As a result, extending DP-based protections to learning applications may be sufficient to protect the training data from exposure, but they may be unnecessary for this goal, and their very high computational and accuracy costs render them practically inapplicable in large-scale learning deployments.

\textbf{Recent learning theory underscores a theoretic deficit.}
To address the theoretic gap left by DP, a very recent stream of theoretic work seeks novel noise-based techniques that upper-bound the degree to which training data can be reconstructed by any unbiased estimator. Nonetheless, as we demonstrate, that approach may provide a false sense of security: 
\textcolor{red}{\textbf{FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein} have recent bounds that also use noise and try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we show this is practically invalid because our DropLayer mask obtains this bound but is totally vulnerable to PPA/IFGMI, as they use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it? Or below?}


\subsection{notes from slack}
\textcolor{purple}{
I think we will need to be explicit as to what we mean by 'memorization'. We need to back up the claims that 1) there is a prevailing view that memorization drives training data exposure; 2) one can reasonably call the approaches of MID, BiDO, and TL-DMI some form of memorization reduction; 3) our DropLayer and Permutation models decrease and increase memorization, respectively.\\\\
%
We argue that memorization is not the whole story for understanding privacy leakage through models, using model inversion attacks as a case study\\\\
%
"By only focusing on memorization, privacy researchers risk failing to defend properly against certain classes of privacy attacks..."\\\\
%
Previous MIA defenses have focused on a data-to-model dependency that intuitively is related to memorization, but we show that this approach is wrong for model inversion, this is not what makes defenses successful\\\\
%
Instead, we propose that MIA defenses focus on adversarially non-robust features... (describe contributions more)\\\\
%
MIA works well on ideal models with powerful learned representations, in some sense these models are easy to 'traverse'\\\\
%
This is similar to the recent papers [cite, cite] that shows that explainable/interpretable models are more privacy leaking\\\\
%
'Ideal models' likely have similar vulnerabilities in other fields, this should continue to be investigated as an orthogonal (or opposing) axis to 'level of memorization'\\\\
%
For this statement, I like the thought experiment of police sketches. That situation is the human equivalent of a model inversion attack. I.e, the artist (StyleGAN) with a strong face prior that can generate headshot representation of a person, and the witness (target model), that keeps directing the artist closer to the suspect (class representative image).\\\\
%
From this we can see that a witness need not memorize any individual image they have seen of said person, as long as they have a meaningful learned representation of that person.\\\\
Therefore, we can say that defending against model inversion is the antithesis of powerful learned representations and good deep learning practices. 
}

\textbf{Codebase and Replication Materials.} \textcolor{red}{[Maybe include in intro since it's great marketing/we have a great codebase, it will look strong/confident since we are calling ppl out.}



\textbf{Questions for July 28 mtng.} \textcolor{purple}{Do we want to continue with the "available defenses claim to work via dependency reduction but all actually work via shifting models to rely on non-robust features, so we can exploit this deliberately with AT-AT" framing? Or do we want to more conservatively say "[Just] The best defense TL-DMI seems to work via shifting models to rely on non-robust features, and we notice that vanilla adversarial training does the opposite, so let's exploit this to do AT-AT" framing?}


\textbf{Some framing notes from July 28 mtng.} \textcolor{orange}{
Consider the Venn diagram of features that describe Adams (like an Adam class centroid in a perfect GAN) and the features that describe Adam's centroid in a good classifier. The former are descriptive; the latter are descriminative. You can have descriminative features that are a very small subset of the descriptive ones (small Venn overlap). Or maybe descriminative features are just a strict subset. Plug and play paper talks about features that matter to faces.\\
%
By doing non-robust features, we search for features in a small $\epsilon$ ball ergo humans cannot perceive and don't care. In practice, ATTACKS DONT CONVERGE but even if they do, we leak an imperceptible noise.\\\\
%
- HSIC is unrelated. Could be that HSIC doesn't capture the appropriate dependency measure, OR that dependency is just the wrong story. Suppose HSIC is just a bad measure, so then DropLayer should reduce dependency. BUT that doesn't work! So we need a new story. Should leave DropLayer and Permutation OUT of the HSIC table. \\\\
%
ALL Defenses are dropping robust features. Some (TL-DMI) are replacing them with non-robust to make up the accuracy. In the AutoAttack table, the accuracy under adv examples captures this...it either gets the example wrong because it sucks at classifying or because it was vulnerable to a small noise.\\\\
%
Adam: in intro talk less about screwing up gradients. Talk more about non-robust features.\\\\
%
Need to introduce and out-of-scope-ify the Neg-LS and Trap-MID or skip-connection defenses are like gradient masking. Trap-MID appendix is the only place they tried against PPA and it sucked and they had to cherry pick aka fine tune)\\\\
The new story is that dependency-based defenses delete robust features, and either take the concomitant accuracy penalty (BiDO) or replace them with non-robust features (TL-DMI).
}



\textbf{Paper organization.} \textcolor{red}{PLACEHOLDER.}

\section{\textcolor{red}{Preliminaries}} \textcolor{red}{PLACEHOLDER.}
\textbf{Threat model.}  \textcolor{red}{- white box because (1) we care about evaluating memorization in target models, and (2) we want strong defenses that are practically effective under strong adversaries with minimal assumptions.\\-Our experiments focus on vision because it's the central MIA research stream, though we intend to expand this in future work, and we include a codebase designed to facilitate this expansion }


\section{Model inversion attacks}
The objective of model inversion attacks is to generate images representing a class of the dataset that ideally is closely resembling images of the dataset. The success of the attack is determined by the confidence of the target model (AvgConf), the accuracy of an independently trained evaluation model (AttAcc@1 \& AttAcc@5) and the $L^2$ distance between the VGGFace2 embeddings of the generated images and the images of the class. Importantly, the image need not be a perfect reconstruction of any individual image in the training data, but aims to create a class representative images or class centroids. \textcolor{red}{I like starting with a natural language explanation before the math, and the metrics can be explained here.}   

Formally, MIA's consider a private training dataset $\mathcal{D}_{priv}=\{x_i,y_i\}_{i=1}^{N}$, where $x_i\in\mathbb{R}^{d_X}$, $y_i\in\{0,1\}^C$, and each $(x_i,y_i)$ are sampled i.i.d. from a joint distribution $\mathbb{P}_{XY}$. Let $T:\mathbb{R}^{d_X}\to\{0,1\}^C$ be a target model trained on $\mathcal{D}_{priv}$ that the adversary wishes to attack. To conduct a model inversion attack, an adversary seeks a new `inverted' model \textcolor{red}{$\hat{\mathcal{I}}_T$ [do we elsewhere denote it by something else? What do the best other ppl use? I like $\hat{\mathcal{I}}_T$ or maybe $\hat{T}'$]} that maps outputs of $T$, such as $T$'s softmax layer or intermediate outputs, back to the corresponding training examples in $\mathcal{D}_{priv}$. The adversary then queries $\hat{\mathcal{I}}_T$ to `predict' $T$'s private training examples. 

\textcolor{red}{note:    The goal in model inversion is to infer the class \emph{centroids} on the data manifold defined on all pixels/features. privacy leakage exists to the extent that these centroids permit reconstruction of features we `care about' (rather than features that are class-descriminative-but not-otherwise-interesting stuff... \ \ The goal of Model Inversion Defense is to build models that infer decision boundaries without leaking information about the training examples via their class centroids, or that are impervious to having their class centroids re-inferred by an attacker.}

Early MIA's trained the inverted model $\hat{\mathcal{I}}_T$ from scratch by using SGD to directly optimize reconstructions of individual training examples \citep{fredrikson2015model}. However, this approach suffers from various optimization complexities when applied to contemporary vision architectures like deep CNN's. Therefore, recent state-of-the-art attacks simplify optimization by adopting an `image prior'---that is, by restricting the search space of training example reconstructions to the image outputs of a domain-relevant GAN, and conducting SGD-based optimization on the GAN's input noise vectors instead of directly on the high-dimensional images' feature space \cite{zhang_secret_2020}. More specifically, GAN-based MIA's optimize a latent noise vector $\hat{z} \in Z$ such that the resultant GAN-generated image is classified as class $c$ maximized confidence by the target model $T$:
%
$$\min_{\hat{z}} \mathcal{L}(T, G, D, \hat{z}, c)$$ 
%
where $\mathcal{L}$ is a standard loss function (e.g. cross-entropy) to maximize the confidence of the GAN-generated image on class $c$,  given pretrained GAN generator $G:Z \to X_{prior}$ and GAN discriminator $D$. Recent attacks on facial recognition classifiers take advantage of pretrained GANs like StyleGAN to perform far more efficient and accurate training data reconstructions \citep{struppek_plug_2022, qiu_closer_2024}. \textcolor{red}{[Mention in the body of the paper that App. \ref{mia-related-work-supp} gives details of SOTA MIA attacks.]}

==> dareDEVALII/Sections/old_SEC_INTRO_V.tex <==


\section{Introduction}

% The tendency of contemporary machine learning models to expose their private training data has recently emerged as a critical performance and security frontier.

% A foundational goal of contemporary machine learning is to learn \emph{generalizable} model parameters from the training data without \emph{exposing} training data examples to leakage. However, it is well-known that virtually all modern architectures obtain generalizable performance only at the cost of encoding a substantial amount of sensitive information about their training examples.


A foundational goal of contemporary machine learning is to learn \emph{generalizable} model parameters from the training data. However, it is well-known that virtually all modern architectures obtain generalizable performance only at the cost of encoding and exposing a substantial amount of sensitive information about their training examples.



\textbf{Understanding this training data encoding and exposure is expected to be a key to next-generation model performance.} % Venn diagram 
A variety of recent work shows that this tradeoff is deeply connected to the efficiency of current training regimes and the performance of contemporary architectures.
%Multiple research streams advance conflicting views on whether the encoding and exposure of training data in model parameters hinders or enhances performance. 
% In classic ML, backpropagating to capture idiosyncratic, ungeneralizable training data details is a well-known performance pitfall that is extensively studied in the context of overfitting. However, in the context of novel generative paradigms such as diffusion models, influential recent work has conjectured that stronger performance may require \emph{more} training data exposure, up to and including rote memorization of the training set \citep[e.g.,][]{carlini2023extracting, c.f., shah2025memorization}. Reconciling these perspectives is key to understanding the mechanics that will shape the next generation of high-performance models.
For example, influential recent work has conjectured that stronger performance may require \emph{more} training data exposure, up to and including rote memorization of the training set, both for vanilla CNN's and for novel paradigms such as LLM's and diffusion models \citep[e.g.,][]{carlini2023extracting, c.f., shah2025memorization}. 
\textcolor{orange}{and LLM's? https://arxiv.org/abs/2205.10770}
\textcolor{blue}{and Apple research generic ML stuff: https://dl.acm.org/doi/pdf/10.1145/3406325.3451131}
\textcolor {green}{and self supervised learning: https://arxiv.org/pdf/2401.12233}
\textcolor{red}{maybe: https://arxiv.org/html/2507.04782v1}
\textcolor{blue}{rasmus's google 2021 paper: https://arxiv.org/abs/1906.05271}
These conjectures stand in contrast to classic ML research on overfitting, where backpropagating to capture idiosyncratic, ungeneralizable training data details is well-studied as a performance pitfall. Reconciling these perspectives is key to understanding the mechanics that will shape the next generation of high-performance models.


 \textbf{Training data exposure undermines privacy in ML deployments.}
Training data exposure also underlies a rapidly expanding class of practical privacy attacks that reconstruct private training data from real-world machine learning deployments simply by querying models or inspecting their parameters. Recent variants of training data attacks apply not only to CNN's, but also to LLM's, diffusion models, multimodal models, etc. \textcolor{red}{[Cite membership inference, attribute inference, carlini's extraction attacks on text LLM's and on stable diffusion].}




\textbf{Model inversion attacks (MIA's) probe and exploit training data exposure.} 
In particular, model inversion attacks (MIA's) have become a mainstream tool for studying and evaluating training data exposure. Unlike more conservative attacks that merely test for the presence of some exposed training examples, MIAs test the degree to which a powerful attacker armed with white-box model access and significant computational and data resources can reconstruct information from the training examples. While early MIA's applied SGD to directly optimize reconstructions of individual training examples \citep{fredrikson2015model}, contemporary MIA's leverage state-of-the-art pretrained models to attempt to infer the full set of class-level characteristics for each class in the training data. 


\textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }


However, while MIA's lower-bound the extent to which training data information is vulnerable to reconstruction, they do not explain what aspect of trained models encodes this vulnerability, or how to prevent it. This raises a fundamental question:


\begingroup
\addtolength\leftmargini{-0.15in} % shrink quote margin
\begin{quote}
%\vspace{-2mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null\\[-2.5mm]
\begin{center}
\vspace{-5mm}
 \textit{What properties of learned representations encode vulnerability to training data leakage and reconstruction, and how can they be controlled?}
 \vspace{-1mm}
\end{center}
\vspace{-2.5mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null
%\vspace{-2mm}
\end{quote}
\endgroup


% \textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }

\textbf{The prevailing `training data exposure = memorization' theory.} %Across various paradigms ranging from classification to LLM's and diffusion, it has become an aphorism to that `models memorize training data'


\textbf{State-of-the-art defenses theorize that MIA's reveal and exploit memorization in the form of direct data-to-model dependencies.}
Motivated by this prevailing idea, an influential recent line of algorithms have obtained practically performant defenses against training data exposure/MIA, and it is widely believed that their practical performance can be attributed to their shared theoretic hypothesis that MIA vulnerability arises from direct and excessive informational/correlative dependency between training inputs and the model’s internal representations or outputs \citep{wang_improving_2020, peng_bilateral_2022, ho_model_nodate}. 

To mitigate this hypothesized dependency, Mutual Information Defense (MID) \citep{wang_improving_2020} introduces a regularizer that reduces mutual information between the training examples and intermediate feature representations, arguing that this ``limit[s] the redundant information about the model input contained in the prediction" so that MIA's cannot ``exploit this correlation.'' Building on this idea, the current state-of-the-art Bilateral Dependency Optimizer (BiDO) algorithm \citep{peng_bilateral_2022} penalizes a kernel-based informational dependency measure (HSIC) between training examples and intermediate embeddings, arguing that this ``limits redundant information propagated from the inputs to the latent representations that can be exploited by the [MIA] adversary.'' 

Similarly, the recent and highly performant TL-DMI approach \citep{ho_model_nodate} advances a ``main hypothesis...that a model with fewer parameters encoding sensitive information from private training dataset'' contains less memorization vulnerable to MIA. This hypothesis is credited with the impressive practical performance of TL-DMI---a transfer-learning based approach that uses the training examples only for fine-tuning later layers of a pre-trained/public model.


The same hypothesis appears again in \textsc{SCA} \citep{dibbo_improving_2024}, which argues that the relevant MIA training data reconstruction vulnerability is reduced by directly “jettison[ing] unnecessary private information in the input image,” e.g. by sparse-coding training images before they are seen by the model, and by also “jettison[ing]…unnecessary private information from downstream layers” to attempt to preclude high-fidelity memorization of the inputs, rather than disincentivizing it via the loss function as in \citep{}\textcolor{red}{MID, BIDO}.

In sum, state-of-the-art defenses advance the theoretic argument that they obtain their practical performance against MIA by reducing memorization defined as informational dependency between training examples and the target model's latent representations/outputs.


\textcolor{red}{[DP-SGD Goodfellow $\rightarrow$ Hayes? Steinke? Guo on encodings? FAIR paper?]}

% \textcolor{orange}{adam should remember to say that these defenses are well-motivated and well-grounded in recent theoretical intuitions...to soften the blow :)}


\textbf{Our contribution I: \  Challenging the theoretic bases of contemporary memorization/MIA defenses.}

In this paper, we challenge this foundational hypothesis. Specifically, we motivate our algorithm by first presenting three surprising experiments that indicate that the memorization dependency view is inadequate to explain MIA reconstruction vulnerability:

\begin{enumerate}
\item \textbf{Reconstruction defenses do not reduce memorization metrics.} First, we show that contemporary defenses that are widely believed to prevent memorization/MIA by reducing training-data-to-model dependency % do not in fact reduce this dependency, and may in fact increase it, even according to their own metrics. 
 \emph{do  not in fact reduce this dependency}, and may in fact increase it, in some cases even according to their own metrics.
%
% \item  \textbf{Low memorization can yield extensive reconstruction, contra recent information-theoretic privacy bounds.} We construct a novel mask-based model that decimates memorization qua input–output dependency by training without allowing the model to see $98\%$ of input pixels (such that each training example is bounded below 2\% memorization in the worst-case), and we show it remains \emph{highly vulnerable} to extensive MIA reconstruction. This is particularly surprising, because we can prove that for these masked 98\% of training data pixels, the Hammersley–Chapman–Robbins (HCR) bound implies an arbitrarily high lower bound on the variance of any unbiased reconstruction estimator—i.e., MIA attacks successfully reconstruct data that is provably impossible to reconstruct under the standard unbiasedness assumption used in recent privacy theory \citep{hannun2021cramer}.

% \item \textbf{Low memorization can yield extensive reconstruction, contra recent information-theoretic privacy bounds.}
% We construct a novel mask-based model that decimates memorization qua input–output dependency by training without allowing the model to see $98\%$ of input pixels (so each training example contains at most $2$\% of its pixels in the worst case).
% % For these masked pixels, we show via the Hammersley–Chapman–Robbins (HCR) bound developed in very recent privacy theory that any reconstruction estimator has  arbitrarily large error bounds, thus reconstruction of 98\% of the data should be impossible, under the standard unbiasedness assumption \citep{hannun2021cramer}.
% % We show that the $98\%$ of masked pixels are provably unreconstructable under standard unbiasedness assumptions using the Hammersley–Chapman–Robbins (HCR) bounds developed in very recent privacy theory  \citep{hannun2021cramer}.
% These 98\% of masked pixels are provably unreconstructable under standard unbiasedness assumptions according to Hammersley–Chapman–Robbins (HCR) bounds developed in very recent privacy theory \citep{hannun2021cramer}.
% Yet in practice, the data remains \emph{highly vulnerable} to extensive MIA reconstruction, showing that recent bounds do not protect against a salient leakage mode of MIA attacks.

\item \textbf{Low memorization can yield extensive reconstruction, contra recent information-theoretic privacy bounds.}
We construct a novel mask-based model that decimates memorization qua input–output dependency by training without allowing the model to see $98\%$ of input pixels (so each training example contains at most $2\%$ of its pixels in the worst case).
Very recent privacy theory allows us to show that these pixels are provably unreconstructable under standard unbiased reconstuction estimator assumptions (via Hammersley-Chapman-Robbins bounds).
Yet in practice, the model remains \emph{highly vulnerable} to extensive MIA reconstruction, revealing that recent bounds do not protect against a salient leakage mode exploited by modern attacks.

\textcolor{red}{Maybe consider adding FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we crush this hope with our DropLayer mask experiment that is an ineffective defense BECAUSE PPA/IFGMI use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it?}
%
%\item Models trained without seeing 98% of the training data pixels can be \emph{highly vulnerable} to extensive MIA reconstruction.
\item \textbf{High memorization can yield low reconstruction.} Conversely, we show that models that perfectly memorize their training dataset are \emph{less vulnerable} to MIA reconstruction than state-of-the-art MIA defenses.
%
\end{enumerate}

In sum, our experiments show that the main theoretic approach in memorization/MIA defense, while well-motivated, is incomplete; state-of-the-art memorization/MIA defenses, we argue, obtain their impressive performance by a different theoretic mechanism.

% \textbf{Our contribution II:\\ The Invertability--Adversarial-Example tradeoff.}
 
%  We probe these counterintuitive findings and discover a surprising result: 
%  Recent defenses hinder reconstruction in part by unintentionally shifting models away from what are known in the adversarial examples literature as “robust features" and, in some cases, toward ``non-robust features" (i.e., features that are generalizable, but imperceptible to humans and unstable under perturbation). \citep{ilyas_adversarial_2019}\textcolor{red}{[Cite Ilya 2019, 2016, szegedy intriguing 2013, and the most influential follow-up papers from after Ilya 2019]}. “Non-robust” features are extremely well-studied in the context of adversarial examples and model robustness, but they are not known to be fundamentally connected to memorization/MIA.

% \textbf{Our Contribution II: The Privacy–Robustness Feature Tradeoff.}

% Our results reveal a previously unrecognized mechanism by which state-of-the-art defenses alter the feature basis of learned representations, establishing a direct link to canonical findings in adversarial example robustness. Specifically, we find that recent defenses hinder reconstruction in part suppressing their model's reliance on robust features (i.e., features that are stable under human-imperceptible perturbations and that align with human-interpretable semantics), and in some cases, replacing them with non-robust features (i.e., features that generalize well but are imperceptible to humans and highly unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}.

% Our results reveal a previously unrecognized mechanism by which state-of-the-art defenses against privacy leakage alter the feature basis of learned representations, thereby establishing a direct link to canonical findings in adversarial example robustness. Contrary to the prevailing view that these defenses primarily protect against reconstruction by reducing direct data–model dependency, we find that they actually hinder reconstructions by reshaping the learned representation space: they suppress reliance on ``robust features'' (i.e., generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics), and in some cases, replacing them with ``non-robust features'' (i.e., features that generalize well but are imperceptible to humans and unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}. This shift has a dual effect: suppressing robust features hurts model accuracy. Replacing robust features with non-robust ones compensates for the accuracy loss, at the cost of brittleness, leaving models far more vulnerable to adversarial examples. While robust vs. non-robust feature reliance is extensively studied in adversarial example research, its role as a governing factor in training data exposure vulnerability has not previously been identified.

\textbf{Our contribution II: The privacy-robustness feature tradeoff.}

We uncover a previously unknown mechanism that directly links training data exposure vulnerabilities to the well-studied robust–non-robust feature tradeoff from adversarial robustness. To probe this phenomenon, we conduct the first systematic evaluation of the robustness of memorization/MIA defenses to adversarial examples. Our analysis reveals that state-of-the-art privacy defenses do not primarily protect against reconstruction by reducing direct data–model dependency, as widely assumed. Instead, they operate by reshaping the learned feature basis. Specifically, they protect privacy by unintentionally suppressing reliance on ``robust features'' (i.e., generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics), and in some cases, replacing them with ``non-robust features'' (i.e., features that generalize well but are imperceptible to humans and unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}. This shift yields a tradeoff: suppressing robust features strips semantically meaningful information from the model but degrades accuracy, while replacing robust features with non-robust features recovers accuracy at the cost of brittleness, leaving models vulnerable to adversarial examples. Although robust–non-robust feature reliance is heavily studied in adversarial robustness, our work is the first to show its central role in training data privacy vulnerabilities. 

% We uncover a previously unknown mechanism that directly links training data exposure vulnerabilities to the well-studied robust–non-robust feature tradeoff from adversarial robustness. State-of-the-art privacy defenses do not primarily protect against reconstruction by reducing direct data–model dependency, as widely assumed. Instead, they operate by reshaping the learned feature basis: unintentionally suppressing robust features—generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics—and, in some cases, replacing them with non-robust features—features that generalize well but are imperceptible to humans and unstable under perturbation \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}.



%
 % By unintentionally promoting this shift, MIA defenses disrupt gradient-based MIA attacks (which now face a fractured loss landscape), \textcolor{red}{[will be revised per July 24 mtng] and also reduce models' reliance on "robust features" that humans find visually/semantically meaningful, and that are captured in MIA reconstruction similarity metrics. This means that dependency-based MIA defenses obtain their performance at a previously overlooked cost: MIA defenses cause models to become far more vulnerable to adversarial examples.}


 \textcolor{red}{[make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with Adversarial Examples]}




\textbf{Our contribution III: \ \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining \\(\textsc{AT-AT}~\ATATicon) for superior privacy/MIA defense.}

If recent memorization/MIA defenses work by unintentionally `nonrobustifying' the model's feature space, then it stands to reason that we could obtain superior defense performance by deliberately exploiting this mechanism. 
%
To accomplish this, we introduce  \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining (\textsc{AT-AT}~\ATATicon), a novel class of memorization/MIA defenses that balance model accuracy with gradient steps that reverse standard adversarial training.  
Rather than promoting robustness to adversarial perturbations, \textsc{AT-AT} applies targeted gradient updates that suppress reliance on robust features, compelling the model to instead learn non-robust—but still generalizable—features that are semantically meaningless to humans and thereby hinder visual reconstruction under MIA.
% "reverse"? maybe something more explicit/clear.
% This simple technique allows us to deliberately compel models to learn non-robust-but-generalizable features that are semantically meaningless to humans (and thus limit visual reconstruction similarity under MIA), but that generalize as well as vanilla CNNs' features.

% \textcolor{red}{non-robust features}

We show that our anti-adversarial approach outperforms baselines in terms of \emph{both} model accuracy and standard MIA defense metrics \textcolor{red}{[PLACEHOLDER for specific outperformance factors or something impressive]} across various standard CNN architectures, datasets, and reconstruction metrics. As with other defenses, this performance comes at the cost of increased vulnerability to adversarial examples. However, in our case, this vulnerability cost is a tunable parameter, offering a new design axis for privacy-robust models.



% Edit this following DP paragraph bc DP is basically in the memorization vein since it's about how much the global statistic shares info about its component observations
\textbf{Privacy implications}
Our results indicate that learning too many descriptive features is a privacy vulnerability distinct from anything that can reasonably be called “memorization.” In this view, a model does not leak information solely like a camera that stores pixel-perfect images of its training data, but also like a crime eyewitness: even without taking pictures, the witness can recall and describe enough private details for a skilled sketch artist armed with prior information about faces (i.e., the MIA attacker) to reconstruct a convincing likeness. 

\textcolor{purple}{
This perspective has four implications. First, eliminating rote memorization does not guarantee privacy, as descriptive-feature leakage can persist in its absence. Second, if recent work is correct in suggesting that rote memorization can confer performance benefits, then such benefits may be attainable without incurring all of the privacy risks that memorization is widely assumed to entail. On the other hand, our results suggest that there may be an inherent privacy vulnerability associated with powerful and robust learned representations. As such, `good' models may be inherently privacy compromising, beyond any specific aspects of how they encode data. This intuition is consistent with recent notions that more interpretable/explainable models are less private. Finally, our results provide intuition regarding why classic DP guarantees are widely regarded as unsuccessful at preventing MIA, since DP degrades by correlated data, and robust features are correlations rather than idiosyncracies of specific training examples. 
%
(1) Eliminating rote memorization does not guarantee privacy, as descriptive-feature leakage can persist absent memorization.
(2) If memorization can improve performance as recently theorized, then such benefits might be achievable without the privacy cost it is assumed to entail.
(3) Powerful, robust representations may be inherently privacy-compromising, such that `good’ models may leak data regardless of how they encode it. %consistent with recent suggestions that more interpretable models tend to be less private.
(4) Our results help explain why classic DP often fails to stop MIAs: DP degrades with correlated data, and robust features are correlations, not idiosyncrasies of specific examples.
(5) FAIR papers are not a realistic path forward because we get guarantees and they don't help in practice. 
}

%Reconstruction vulnerability is present even absent seeing pixels.


For completeness, we note that another stream of recent defenses in the literature do not seek to address the underlying privacy vulnerability at all, but instead interfere with specific MIA attack implementations (e.g., by making the loss landscape unamenable to gradients taken in the most popular MIA attacks).\textcolor{green}{negLS;RoLSS;}\textcolor{red}{label smoothing; trapdoor}. %We include the most popular of these defenses in our experiments, but they are otherwise outside our scope, as they target the mechanics of specific attacks rather than seeking to explore the underlying privacy vulnerability.





\textbf{Classical privacy frameworks like DP do not explain the training data exposure that MIA's exploit.}
While classical privacy frameworks such as Differential Privacy (DP) \cite{dwork2006differential, dwork2014algorithmic} offer provable guarantees against training example exposure \citep{hayes_bounding_2023}, they do not explain why it arises in contemporary learning settings. 
DP was designed to protect the privacy of individual training examples while releasing parameters that characterize in-sample group-level descriptive statistics. These competing goals have a direct information-theoretic tradeoff. 
% DP was designed to control the direct information-theoretic tradeoff between the privacy of individual training examples we want to protect and the accuracy of in-sample group-level statistics we want to release.
However, the same direct tradeoff does not obviously apply to releasing model parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning).
%It does not directly apply when releasing parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning), where it is not obvious how such a tradeoff applies. 
As a result, extending DP-based protections to learning applications may be sufficient to protect the training data from exposure, but they may be unnecessary for this goal, and their very high computational and accuracy costs render them practically inapplicable in large-scale learning deployments.

\textbf{Recent learning theory underscores a theoretic deficit.}
To address the theoretic gap left by DP, a very recent stream of theoretic work seeks novel noise-based techniques that upper-bound the degree to which training data can be reconstructed by any unbiased estimator. Nonetheless, as we demonstrate, that approach may provide a false sense of security: 
\textcolor{red}{\textbf{FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein} have recent bounds that also use noise and try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we show this is practically invalid because our DropLayer mask obtains this bound but is totally vulnerable to PPA/IFGMI, as they use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it? Or below?}


\subsection{notes from slack}
\textcolor{purple}{
I think we will need to be explicit as to what we mean by 'memorization'. We need to back up the claims that 1) there is a prevailing view that memorization drives training data exposure; 2) one can reasonably call the approaches of MID, BiDO, and TL-DMI some form of memorization reduction; 3) our DropLayer and Permutation models decrease and increase memorization, respectively.\\\\
%
We argue that memorization is not the whole story for understanding privacy leakage through models, using model inversion attacks as a case study\\\\
%
"By only focusing on memorization, privacy researchers risk failing to defend properly against certain classes of privacy attacks..."\\\\
%
Previous MIA defenses have focused on a data-to-model dependency that intuitively is related to memorization, but we show that this approach is wrong for model inversion, this is not what makes defenses successful\\\\
%
Instead, we propose that MIA defenses focus on adversarially non-robust features... (describe contributions more)\\\\
%
MIA works well on ideal models with powerful learned representations, in some sense these models are easy to 'traverse'\\\\
%
This is similar to the recent papers [cite, cite] that shows that explainable/interpretable models are more privacy leaking\\\\
%
'Ideal models' likely have similar vulnerabilities in other fields, this should continue to be investigated as an orthogonal (or opposing) axis to 'level of memorization'\\\\
%
For this statement, I like the thought experiment of police sketches. That situation is the human equivalent of a model inversion attack. I.e, the artist (StyleGAN) with a strong face prior that can generate headshot representation of a person, and the witness (target model), that keeps directing the artist closer to the suspect (class representative image).\\\\
%
From this we can see that a witness need not memorize any individual image they have seen of said person, as long as they have a meaningful learned representation of that person.\\\\
Therefore, we can say that defending against model inversion is the antithesis of powerful learned representations and good deep learning practices. 
}

\textbf{Codebase and Replication Materials.} \textcolor{red}{[Maybe include in intro since it's great marketing/we have a great codebase, it will look strong/confident since we are calling ppl out.}



\textbf{Questions for July 28 mtng.} \textcolor{purple}{Do we want to continue with the "available defenses claim to work via dependency reduction but all actually work via shifting models to rely on non-robust features, so we can exploit this deliberately with AT-AT" framing? Or do we want to more conservatively say "[Just] The best defense TL-DMI seems to work via shifting models to rely on non-robust features, and we notice that vanilla adversarial training does the opposite, so let's exploit this to do AT-AT" framing?}


\textbf{Some framing notes from July 28 mtng.} \textcolor{orange}{
Consider the Venn diagram of features that describe Adams (like an Adam class centroid in a perfect GAN) and the features that describe Adam's centroid in a good classifier. The former are descriptive; the latter are descriminative. You can have descriminative features that are a very small subset of the descriptive ones (small Venn overlap). Or maybe descriminative features are just a strict subset. Plug and play paper talks about features that matter to faces.\\
%
By doing non-robust features, we search for features in a small $\epsilon$ ball ergo humans cannot perceive and don't care. In practice, ATTACKS DONT CONVERGE but even if they do, we leak an imperceptible noise.\\\\
%
- HSIC is unrelated. Could be that HSIC doesn't capture the appropriate dependency measure, OR that dependency is just the wrong story. Suppose HSIC is just a bad measure, so then DropLayer should reduce dependency. BUT that doesn't work! So we need a new story. Should leave DropLayer and Permutation OUT of the HSIC table. \\\\
%
ALL Defenses are dropping robust features. Some (TL-DMI) are replacing them with non-robust to make up the accuracy. In the AutoAttack table, the accuracy under adv examples captures this...it either gets the example wrong because it sucks at classifying or because it was vulnerable to a small noise.\\\\
%
Adam: in intro talk less about screwing up gradients. Talk more about non-robust features.\\\\
%
Need to introduce and out-of-scope-ify the Neg-LS and Trap-MID or skip-connection defenses are like gradient masking. Trap-MID appendix is the only place they tried against PPA and it sucked and they had to cherry pick aka fine tune)\\\\
The new story is that dependency-based defenses delete robust features, and either take the concomitant accuracy penalty (BiDO) or replace them with non-robust features (TL-DMI).
}



\textbf{Paper organization.} \textcolor{red}{PLACEHOLDER.}

\section{\textcolor{red}{Preliminaries}} \textcolor{red}{PLACEHOLDER.}
\textbf{Threat model.}  \textcolor{red}{- white box because (1) we care about evaluating memorization in target models, and (2) we want strong defenses that are practically effective under strong adversaries with minimal assumptions.\\-Our experiments focus on vision because it's the central MIA research stream, though we intend to expand this in future work, and we include a codebase designed to facilitate this expansion }


\section{Model inversion attacks}
The objective of model inversion attacks is to generate images representing a class of the dataset that ideally is closely resembling images of the dataset. The success of the attack is determined by the confidence of the target model (AvgConf), the accuracy of an independently trained evaluation model (AttAcc@1 \& AttAcc@5) and the $L^2$ distance between the VGGFace2 embeddings of the generated images and the images of the class. Importantly, the image need not be a perfect reconstruction of any individual image in the training data, but aims to create a class representative images or class centroids. \textcolor{red}{Maybe we can start with a natural language explanation before the math like this, and the metrics can be explained here.}   

Formally, MIA's consider a private training dataset $\mathcal{D}_{priv}=\{x_i,y_i\}_{i=1}^{N}$, where $x_i\in\mathbb{R}^{d_X}$, $y_i\in\{0,1\}^C$, and each $(x_i,y_i)$ are sampled i.i.d. from a joint distribution $\mathbb{P}_{XY}$. Let $T:\mathbb{R}^{d_X}\to\{0,1\}^C$ be a target model trained on $\mathcal{D}_{priv}$ that the adversary wishes to attack. To conduct a model inversion attack, an adversary seeks a new `inverted' model \textcolor{red}{$\hat{\mathcal{I}}_T$ [do we elsewhere denote it by something else? What do the best other ppl use? I like $\hat{\mathcal{I}}_T$ or maybe $\hat{T}'$]} that maps outputs of $T$, such as $T$'s softmax layer or intermediate outputs, back to the corresponding training examples in $\mathcal{D}_{priv}$. The adversary then queries $\hat{\mathcal{I}}_T$ to `predict' $T$'s private training examples. 

\textcolor{red}{note:    The goal in model inversion is to infer the class \emph{centroids} on the data manifold defined on all pixels/features. privacy leakage exists to the extent that these centroids permit reconstruction of features we `care about' (rather than features that are class-descriminative-but not-otherwise-interesting stuff... \ \ The goal of Model Inversion Defense is to build models that infer decision boundaries without leaking information about the training examples via their class centroids, or that are impervious to having their class centroids re-inferred by an attacker.}

Early MIA's trained the inverted model $\hat{\mathcal{I}}_T$ from scratch by using SGD to directly optimize reconstructions of individual training examples \citep{fredrikson2015model}. However, this approach suffers from various optimization complexities when applied to contemporary vision architectures like deep CNN's. Therefore, recent state-of-the-art attacks simplify optimization by adopting an `image prior'---that is, by restricting the search space of training example reconstructions to the image outputs of a domain-relevant GAN, and conducting SGD-based optimization on the GAN's input noise vectors instead of directly on the high-dimensional images' feature space \cite{zhang_secret_2020}. More specifically, GAN-based MIA's optimize a latent noise vector $\hat{z} \in Z$ such that the resultant GAN-generated image is classified as class $c$ maximized confidence by the target model $T$:
%
$$\min_{\hat{z}} \mathcal{L}(T, G, D, \hat{z}, c)$$ 
%
where $\mathcal{L}$ is a standard loss function (e.g. cross-entropy) to maximize the confidence of the GAN-generated image on class $c$,  given pretrained GAN generator $G:Z \to X_{prior}$ and GAN discriminator $D$. Recent attacks on facial recognition classifiers take advantage of pretrained GANs like StyleGAN to perform far more efficient and accurate training data reconstructions \citep{struppek_plug_2022, qiu_closer_2024}. \textcolor{red}{[Mention in the body of the paper that App. \ref{mia-related-work-supp} gives details of SOTA MIA attacks.]}

==> dareDEVALII/Sections/old_SEC_INTRO_VI_A_NEW_HOPE.tex <==

% training privacy vulnerability is ascribed to memorization across various SOTA models like LLM, diffusion, classification, etc.

% Memorization can refer to a variety of related concepts but in the context of MI, defenses are trying to minimize the explicit dependency of training data that are “rote encoded” into the model such inputs and embeddings have high joint HSIC, MI, etc.

% In the appendix, we can hide a paragraph of quotes about memorization since some reviewer will certainly attack some aspect of the fact that the concept of memorization is vague, and it’s not clear that a fully memorized model relates to a high HSIC model or something.



\textcolor{orange}{correlation causation thing}




\textcolor{purple}{Among the most celebrated results in ML is the finding that adversarial examples are not bugs, but non-robust features \citep{ilyas_adversarial_2019}. In other words, adversarial examples reveal features that are generalizable and discriminatory of the classes we want to learn, but visually imperceptible to humans. Our argument in this paper is that these properties make them ideal instruments for privacy-preserving learning, where our goal is to classify accurately without encoding visually meaningful information that is vulnerable to visual reconstructions.}

\section{Introduction}

\textbf{\textcolor{red}{Rewriting this as it mentions memorization a lot incorrectly}}

A foundational goal of contemporary machine learning is to learn \emph{generalizable} model parameters from the training data. However, it is well-known that virtually all modern architectures obtain generalizable performance only at the cost of encoding and exposing a substantial amount of sensitive information about their training examples.


\textbf{Understanding training data encoding and exposure is a key to next-generation model performance.} % Venn diagram 
A variety of recent research shows that this tradeoff is deeply connected to the performance of contemporary architectures.
For example, influential recent work has conjectured that obtaining stronger performance may require rote memorization of the training set, not only for vanilla CNNs, but also for novel paradigms such as LLM's and diffusion models \citep[e.g.,][]{carlini_extracting_2023, c.f., shah_does_2025}. 
\begin{enumerate}
    \item \citep{tirumala_memorization_2022} -- LLMs
    \item \citep{brown_when_2021} -- Apple researh generic ML
    \item \citep{wang_memorization_2024} -- Self-supervised learning
    \item \citep{du_reason_2025} -- preprint "Reason to Rote"
    \item \citep{feldman_does_2020} -- "short tale about long tail", theoretical paper for classification models
\end{enumerate}
These conjectures stand in contrast to classic ML research on overfitting, where training to encode idiosyncratic, ungeneralizable training data details is well-studied as a performance pitfall. Reconciling these perspectives is key to understanding the mechanics that will shape the next generation of high-performance models.


 \textbf{Training data exposure undermines privacy in ML deployments.}
Training data encoding and exposure also underlies a rapidly expanding class of practical privacy attacks that reconstruct private training data from real-world machine learning deployments simply by querying models or inspecting their parameters. Recent variants of training data attacks apply not only to CNN's, but also to LLM's, diffusion models, multimodal models, etc. \textcolor{red}{[Cite membership inference, attribute inference, carlini's extraction attacks on text LLM's and on stable diffusion].}




\textbf{Model inversion attacks (MIA's) probe and exploit training data exposure.} 
In particular, model inversion attacks (MIA's) have become a mainstream tool for studying and evaluating training data exposure. Unlike more conservative attacks that merely test for the presence of some exposed training examples, MIAs test the degree to which a powerful attacker armed with white-box model access and significant computational and data resources can reconstruct information from the training examples. While early MIA's applied SGD to directly optimize reconstructions of individual training examples \citep{fredrikson_model_2015}, contemporary MIA's leverage state-of-the-art pretrained models to attempt to infer the full set of class-level characteristics for each class in the training data. 


\textcolor{red}{[we should also cite \citep{haim_reconstructing_2022} (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }


However, while MIA's lower-bound the extent to which training data information is vulnerable to reconstruction, they do not explain what aspect of a model encodes this vulnerability, or how to prevent it. This raises a fundamental question:


\begingroup
\addtolength\leftmargini{-0.15in} % shrink quote margin
\begin{quote}
%\vspace{-2mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null\\[-2.5mm]
\begin{center}
\vspace{-4.5mm}
 \textit{What properties of learned representations encode vulnerability to training data leakage and reconstruction, and how can they be controlled?}
 \vspace{-0.5mm}
\end{center}
\vspace{-2.5mm}
\noindent\hfill$\diamond\ \diamond\ \diamond$\hfill\null
%\vspace{-2mm}
\end{quote}
\endgroup


% \textcolor{red}{[we should also cite haim2022reconstructing (Niv Haim's NeurIPS'22 paper) and some of the papers that responded to it]}
% @article{haim2022reconstructing,
%   title={Reconstructing training data from trained neural networks},
%   author={Haim, Niv and Vardi, Gal and Yehudai, Gilad and Shamir, Ohad and Irani, Michal},
%   journal={Advances in Neural Information Processing Systems},
%   volume={35},
%   pages={22911--22924},
%   year={2022}
% }

\textbf{The prevailing `memorization $\rightarrow$ training data exposure' theory.} 
\textbf{\textcolor{red}{PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER}}


\textbf{Defenses theorize that MIA's reveal and exploit memorization in the form of direct data-to-model dependencies.}
An influential recent line of algorithms have obtained practically performant defenses against training data exposure/MIA, and it is widely believed that their practical performance can be attributed to their shared theoretic hypothesis that MIA vulnerability arises from direct and excessive informational/correlative dependency between training inputs and the model’s internal representations or outputs \citep{wang_improving_2020, peng_bilateral_2022, ho_model_2024}. 

To mitigate this hypothesized dependency, Mutual Information Defense (MID) \citep{wang_improving_2020} introduces a regularizer that reduces mutual information between the training examples and intermediate feature representations, arguing that this ``limit[s] the redundant information about the model input contained in the prediction" so that MIA's cannot ``exploit this correlation.'' Building on this idea, the current state-of-the-art Bilateral Dependency Optimizer (BiDO) algorithm \citep{peng_bilateral_2022} penalizes a kernel-based informational dependency measure (HSIC) between training examples and intermediate embeddings, arguing that this ``limits redundant information propagated from the inputs to the latent representations that can be exploited by the [MIA] adversary.'' 

Similarly, the recent and highly performant TL-DMI approach \citep{ho_model_2024} advances a ``main hypothesis...that a model with fewer parameters encoding sensitive information from private training dataset'' contains less memorization vulnerable to MIA. This hypothesis is credited with the impressive practical performance of TL-DMI---a transfer-learning based approach that uses the training examples only for fine-tuning later layers of a pre-trained/public model. \textcolor{orange}{\textbf{Check this. They may just say that they try to drop the information that is relevant to MIA. In that case we can say that they are careful not to state that this info is memorized, but it is widely believed by practitioners that it is memorized info not non-robust info. Need to check.}}


The same hypothesis appears again in \textsc{SCA} \citep{dibbo_improving_2024}, which argues that the relevant MIA training data reconstruction vulnerability is reduced by directly “jettison[ing] unnecessary private information in the input image,” e.g. by sparse-coding training images before they are seen by the model, and by also “jettison[ing]…unnecessary private information from downstream layers” to attempt to preclude high-fidelity memorization of the inputs, rather than disincentivizing it via the loss function as in \citet{peng_bilateral_2022,wang_improving_2020}.

In sum, state-of-the-art defenses advance the theoretic argument that they obtain their practical performance against MIA by reducing memorization defined as informational dependency between training examples and the target model's latent representations/outputs.


\textcolor{red}{[DP-SGD Goodfellow \citep{abadi_deep_2016}$\rightarrow$ Hayes \citep{hayes_bounding_2023}? Steinke\citep{steinke_reasoning_2020}? Guo on encodings\citep{guo_bounding_2022}? FAIR papers \citep{hannun_measuring_2021, chaudhuri_guarantees_2024}?]}

\textcolor{orange}{adam should remember to say that these defenses are well-motivated and well-grounded in recent theoretical intuitions...to soften the blow :)}


\textbf{Our contribution I: \  Challenging the theoretic bases of contemporary memorization/MIA defenses.}

In this paper, we challenge this foundational hypothesis. Specifically, we motivate our algorithm by first presenting three surprising experiments that indicate that the memorization dependency view is inadequate to explain MIA reconstruction vulnerability:

\begin{enumerate}
\item \textbf{Reconstruction defenses do not reduce memorization metrics.} First, we show that contemporary defenses that are widely believed to prevent memorization/MIA by reducing training-data-to-model dependency % do not in fact reduce this dependency, and may in fact increase it, even according to their own metrics. 
 \emph{do  not in fact reduce this dependency}, and may in fact increase it, in some cases even according to their own metrics.
%
% \item  \textbf{Low memorization can yield extensive reconstruction, contra recent information-theoretic privacy bounds.} We construct a novel mask-based model that decimates memorization qua input–output dependency by training without allowing the model to see $98\%$ of input pixels (such that each training example is bounded below 2\% memorization in the worst-case), and we show it remains \emph{highly vulnerable} to extensive MIA reconstruction. This is particularly surprising, because we can prove that for these masked 98\% of training data pixels, the Hammersley–Chapman–Robbins (HCR) bound implies an arbitrarily high lower bound on the variance of any unbiased reconstruction estimator—i.e., MIA attacks successfully reconstruct data that is provably impossible to reconstruct under the standard unbiasedness assumption used in recent privacy theory \citep{hannun2021cramer}.

% \item \textbf{Low memorization can yield extensive reconstruction, contra recent information-theoretic privacy bounds.}
% We construct a novel mask-based model that decimates memorization qua input–output dependency by training without allowing the model to see $98\%$ of input pixels (so each training example contains at most $2$\% of its pixels in the worst case).
% % For these masked pixels, we show via the Hammersley–Chapman–Robbins (HCR) bound developed in very recent privacy theory that any reconstruction estimator has  arbitrarily large error bounds, thus reconstruction of 98\% of the data should be impossible, under the standard unbiasedness assumption \citep{hannun2021cramer}.
% % We show that the $98\%$ of masked pixels are provably unreconstructable under standard unbiasedness assumptions using the Hammersley–Chapman–Robbins (HCR) bounds developed in very recent privacy theory  \citep{hannun2021cramer}.
% These 98\% of masked pixels are provably unreconstructable under standard unbiasedness assumptions according to Hammersley–Chapman–Robbins (HCR) bounds developed in very recent privacy theory \citep{hannun2021cramer}.
% Yet in practice, the data remains \emph{highly vulnerable} to extensive MIA reconstruction, showing that recent bounds do not protect against a salient leakage mode of MIA attacks.

\item \textbf{High memorization can yield low reconstruction.} We show that models that perfectly memorize their training dataset are \emph{less vulnerable} to MIA reconstruction than state-of-the-art MIA defenses.

% \item \textbf{Low memorization can yield extensive reconstruction, contra recent information-theoretic privacy bounds.}
% We construct a novel mask-based model that decimates memorization qua input–output dependency by training without allowing the model to see $97\%$ of input pixels (so each training example contains at most $<$3\% of its pixels).
% Very recent privacy theory allows us to show that these pixels are provably unreconstructable under standard unbiased reconstuction estimator assumptions (via Hammersley-Chapman-Robbins bounds).
% Yet in practice, the model remains \emph{highly vulnerable} to extensive MIA reconstruction, revealing that recent bounds do not protect against a salient leakage mode exploited by modern attacks.
[shailen commented out the suggestion to add FAIR bounds since it's in already - 9/21]

%
%\item Models trained without seeing 98% of the training data pixels can be \emph{highly vulnerable} to extensive MIA reconstruction.

%
\end{enumerate}

In sum, our motivating experiments show that the main theoretic approach in memorization/MIA defense is incomplete; state-of-the-art memorization/MIA defenses obtain their impressive performance by a different theoretic mechanism.

% \textbf{Our contribution II:\\ The Invertability--Adversarial-Example tradeoff.}
 
%  We probe these counterintuitive findings and discover a surprising result: 
%  Recent defenses hinder reconstruction in part by unintentionally shifting models away from what are known in the adversarial examples literature as “robust features" and, in some cases, toward ``non-robust features" (i.e., features that are generalizable, but imperceptible to humans and unstable under perturbation). \citep{ilyas_adversarial_2019}\textcolor{red}{[Cite Ilya 2019, 2016, szegedy intriguing 2013, and the most influential follow-up papers from after Ilya 2019]}. “Non-robust” features are extremely well-studied in the context of adversarial examples and model robustness, but they are not known to be fundamentally connected to memorization/MIA.

% \textbf{Our Contribution II: The Privacy–Robustness Feature Tradeoff.}

% Our results reveal a previously unrecognized mechanism by which state-of-the-art defenses alter the feature basis of learned representations, establishing a direct link to canonical findings in adversarial example robustness. Specifically, we find that recent defenses hinder reconstruction in part suppressing their model's reliance on robust features (i.e., features that are stable under human-imperceptible perturbations and that align with human-interpretable semantics), and in some cases, replacing them with non-robust features (i.e., features that generalize well but are imperceptible to humans and highly unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}.

% Our results reveal a previously unrecognized mechanism by which state-of-the-art defenses against privacy leakage alter the feature basis of learned representations, thereby establishing a direct link to canonical findings in adversarial example robustness. Contrary to the prevailing view that these defenses primarily protect against reconstruction by reducing direct data–model dependency, we find that they actually hinder reconstructions by reshaping the learned representation space: they suppress reliance on ``robust features'' (i.e., generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics), and in some cases, replacing them with ``non-robust features'' (i.e., features that generalize well but are imperceptible to humans and unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}. This shift has a dual effect: suppressing robust features hurts model accuracy. Replacing robust features with non-robust ones compensates for the accuracy loss, at the cost of brittleness, leaving models far more vulnerable to adversarial examples. While robust vs. non-robust feature reliance is extensively studied in adversarial example research, its role as a governing factor in training data exposure vulnerability has not previously been identified.

\textbf{Our contribution II: The privacy-robustness feature tradeoff.}

%We uncover a previously unknown mechanism that directly links training data exposure vulnerabilities to the well-studied robust–non-robust feature tradeoff from the adversarial examples literature. 
To probe these phenomena, we conduct the first systematic evaluation of the robustness of memorization/MIA defenses to adversarial examples. Our analysis reveals that state-of-the-art privacy defenses do not primarily protect against reconstruction by reducing direct data–model dependency, as widely assumed. Instead, they operate by reshaping the learned feature basis. Specifically, they protect privacy by unintentionally suppressing reliance on ``robust features'' (i.e., generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics), and in some cases, replacing them with ``non-robust features'' (i.e., features that generalize well but are imperceptible to humans and unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy_intriguing_2014, }\textcolor{orange}{[add ilyas2016, post-2019-cites]}. This shift yields a tradeoff: suppressing robust features strips semantically meaningful information from the model but degrades accuracy, while replacing robust features with non-robust features recovers accuracy at the cost of brittleness, leaving models vulnerable to adversarial examples. Although robust–non-robust feature reliance is heavily studied in adversarial robustness, our work is the first to show its central role in training data privacy vulnerabilities. 

% We uncover a previously unknown mechanism that directly links training data exposure vulnerabilities to the well-studied robust–non-robust feature tradeoff from adversarial robustness. State-of-the-art privacy defenses do not primarily protect against reconstruction by reducing direct data–model dependency, as widely assumed. Instead, they operate by reshaping the learned feature basis: unintentionally suppressing robust features—generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics—and, in some cases, replacing them with non-robust features—features that generalize well but are imperceptible to humans and unstable under perturbation \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}.



%
 % By unintentionally promoting this shift, MIA defenses disrupt gradient-based MIA attacks (which now face a fractured loss landscape), \textcolor{red}{[will be revised per July 24 mtng] and also reduce models' reliance on "robust features" that humans find visually/semantically meaningful, and that are captured in MIA reconstruction similarity metrics. This means that dependency-based MIA defenses obtain their performance at a previously overlooked cost: MIA defenses cause models to become far more vulnerable to adversarial examples.}


 % \textcolor{red}{[make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with Adversarial Examples]}




\textbf{Our contribution III: \ \underline{A}n\underline{t}i-\underline{A}dversarial \underline{T}raining \\(\textsc{AT-AT}~\ATATicon) for superior privacy/MIA defense.}

If recent privacy/MIA defenses work by unintentionally `nonrobustifying' the model's feature space, then it stands to reason that we could obtain superior defense performance by deliberately exploiting this mechanism. 
%
To accomplish this, we introduce  introduce \textbf{\underline{A}}n\textbf{\underline{t}}i \textbf{\underline{A}}dversarial \textbf{\underline{T}}raining (\textbf{AT-AT}~\ATATiconMINI), a novel class of memorization/MIA defense training regimes that balance model accuracy with gradient steps that reverse standard adversarial training.  
Rather than promoting robustness to adversarial perturbations, \textsc{AT-AT} applies targeted gradient updates that suppress reliance on robust features, compelling the model to instead learn non-robust—but still generalizable—features that are semantically meaningless to humans and thereby hinder visual reconstruction under MIA.
% "reverse"? maybe something more explicit/clear.
% This simple technique allows us to deliberately compel models to learn non-robust-but-generalizable features that are semantically meaningless to humans (and thus limit visual reconstruction similarity under MIA), but that generalize as well as vanilla CNNs' features.

% \textcolor{red}{non-robust features}

We show that our anti-adversarial approach outperforms baselines in terms of \emph{both} model accuracy and standard MIA defense metrics \textcolor{red}{[PLACEHOLDER for specific outperformance factors or something impressive]} across various standard CNN architectures, datasets, and reconstruction metrics. As with other defenses, this performance comes at the cost of increased vulnerability to adversarial examples. However, in our case, this vulnerability cost is a tunable parameter, offering a new design axis for privacy-robust models.



% Edit this following DP paragraph bc DP is basically in the memorization vein since it's about how much the global statistic shares info about its component observations
\textbf{Privacy implications}
Our results indicate that learning too many descriptive features is a privacy vulnerability distinct from anything that can reasonably be called “memorization.” In this view, a model does not leak information solely like a camera that stores pixel-perfect images of its training data, but also like a crime eyewitness: even without taking pictures, the witness can recall and describe enough private details for a skilled sketch artist armed with prior information about faces (i.e., the MIA attacker) to reconstruct a convincing likeness. 

\textbf{Implications for private learning.}
This perspective has four implications. First, eliminating rote memorization does not guarantee privacy, as descriptive-feature leakage can persist in its absence. Second, if recent work is correct in suggesting that rote memorization can confer performance benefits, then such benefits may be attainable without incurring all of the privacy risks that memorization is widely assumed to entail. On the other hand, our results suggest that there may be an inherent privacy vulnerability associated with powerful and robust learned representations. As such, `good' models may be inherently privacy compromising, beyond any specific aspects of how they encode data. This intuition is consistent with recent notions that more interpretable/explainable models are less private. 

\textbf{Implications for privacy theory.}
Finally, our results provide intuition regarding why classic DP guarantees are widely regarded as unsuccessful at preventing MIA, since DP degrades by correlated data, and robust features are correlations rather than idiosyncracies of specific training examples. Similarly, they also show that reconstruction attacks violate the assumptions and protections promised by recent privacy bounds.


% Finally, recent privacy theory that emphasizes information-theoretic bounds on  reconstruction variance, while elegant, may provide a false sense of security under practical attack settings. 
% %
% (1) Eliminating rote memorization does not guarantee privacy, as descriptive-feature leakage can persist absent memorization.
% (2) If memorization can improve performance as recently theorized, then such benefits might be achievable without the privacy cost it is assumed to entail.
% (3) Powerful, robust representations may be inherently privacy-compromising, such that `good’ models may leak data regardless of how they encode it. %consistent with recent suggestions that more interpretable models tend to be less private.
% (4) Our results help explain why classic DP often fails to stop MIAs: DP degrades with correlated data, and robust features are correlations, not idiosyncrasies of specific examples.
% (5) FAIR papers are not a realistic path forward because we get guarantees and they don't help in practice. 
% }

%Reconstruction vulnerability is present even absent seeing pixels.

\textcolor{red}{THIS MOVES TO EXPERIMENT BASELINES SECTION}
For completeness, we note that another stream of recent defenses in the literature do not seek to address the underlying privacy vulnerability at all, but instead interfere with specific MIA attack implementations (e.g., by making the loss landscape unamenable to gradients taken in the most popular MIA attacks).\textcolor{green}{negLS;RoLSS;}\textcolor{red}{ label smoothing; trapdoor}.



%We include the most popular of these defenses in our experiments, but they are otherwise outside our scope, as they target the mechanics of specific attacks rather than seeking to explore the underlying privacy vulnerability.





% \textbf{Classical privacy frameworks like DP do not explain the training data exposure that MIA's exploit.}
% While classical privacy frameworks such as Differential Privacy (DP) \cite{dwork2006differential, dwork2014algorithmic} offer provable guarantees against training example exposure \citep{hayes_bounding_2023}, they do not explain why it arises in contemporary learning settings. 
% DP was designed to protect the privacy of individual training examples while releasing parameters that characterize in-sample group-level descriptive statistics. These competing goals have a direct information-theoretic tradeoff. 
% % DP was designed to control the direct information-theoretic tradeoff between the privacy of individual training examples we want to protect and the accuracy of in-sample group-level statistics we want to release.
% However, the same direct tradeoff does not obviously apply to releasing model parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning).
% %It does not directly apply when releasing parameters that discriminate between class distributions out-of-sample (i.e. the goal of learning), where it is not obvious how such a tradeoff applies. 
% As a result, extending DP-based protections to learning applications may be sufficient to protect the training data from exposure, but they may be unnecessary for this goal, and their very high computational and accuracy costs render them practically inapplicable in large-scale learning deployments.

% \textbf{Recent learning theory underscores a theoretic deficit.}
% To address the theoretic gap left by DP, a very recent stream of theoretic work seeks novel noise-based techniques that upper-bound the degree to which training data can be reconstructed by any unbiased estimator. Nonetheless, as we demonstrate, that approach may provide a false sense of security: 
\textcolor{red}{\textbf{FAIRpapers (Hannun'21 on Cramer-Rao bound; Chaudhury'25 on HCR bound;  XIA et al (nonFAIR) CVPR'25 federated paper in same vein}} 
% have recent bounds that also use noise and try to bound against reconstructing specific input or group of inputs GIVEN UNBIASED ESTIMATOR but we show this is practically invalid because our DropLayer mask obtains this bound but is totally vulnerable to PPA/IFGMI, as they use a super biased estimator biased by StyleGAN image priors. Here might be the place to mention it? Or below?}


\subsection{notes from slack}
\textcolor{purple}{
I think we will need to be explicit as to what we mean by 'memorization'. We need to back up the claims that 1) there is a prevailing view that memorization drives training data exposure; 2) one can reasonably call the approaches of MID, BiDO, and TL-DMI some form of memorization reduction; 3) our DropLayer and Permutation models decrease and increase memorization, respectively.\\\\
%
We argue that memorization is not the whole story for understanding privacy leakage through models, using model inversion attacks as a case study\\\\
%
"By only focusing on memorization, privacy researchers risk failing to defend properly against certain classes of privacy attacks..."\\\\
%
Previous MIA defenses have focused on a data-to-model dependency that intuitively is related to memorization, but we show that this approach is wrong for model inversion, this is not what makes defenses successful\\\\
%
Instead, we propose that MIA defenses focus on adversarially non-robust features... (describe contributions more)\\\\
%
MIA works well on ideal models with powerful learned representations, in some sense these models are easy to 'traverse'\\\\
%
This is similar to the recent papers [cite, cite] that shows that explainable/interpretable models are more privacy leaking\\\\
%
'Ideal models' likely have similar vulnerabilities in other fields, this should continue to be investigated as an orthogonal (or opposing) axis to 'level of memorization'\\\\
%
% For this statement, I like the thought experiment of police sketches. That situation is the human equivalent of a model inversion attack. I.e, the artist (StyleGAN) with a strong face prior that can generate headshot representation of a person, and the witness (target model), that keeps directing the artist closer to the suspect (class representative image).\\\\
%
% From this we can see that a witness need not memorize any individual image they have seen of said person, as long as they have a meaningful learned representation of that person.\\\\
We can say that defending against model inversion is the antithesis of powerful learned representations and good deep learning practices. 
}

\textbf{Codebase and Replication Materials.} \textcolor{red}{[Maybe include in intro since it's great marketing/we have a great codebase, it will look strong/confident since we are calling ppl out.}



\textbf{Questions for July 28 mtng.} \textcolor{purple}{Do we want to continue with the "available defenses claim to work via dependency reduction but all actually work via shifting models to rely on non-robust features, so we can exploit this deliberately with AT-AT" framing? Or do we want to more conservatively say "[Just] The best defense TL-DMI seems to work via shifting models to rely on non-robust features, and we notice that vanilla adversarial training does the opposite, so let's exploit this to do AT-AT" framing?}


\textbf{Some framing notes from July 28 mtng.} \textcolor{orange}{
Consider the Venn diagram of features that describe Adams (like an Adam class centroid in a perfect GAN) and the features that describe Adam's centroid in a good classifier. The former are descriptive; the latter are descriminative. You can have descriminative features that are a very small subset of the descriptive ones (small Venn overlap). Or maybe descriminative features are just a strict subset. Plug and play paper talks about features that matter to faces.\\
%
By doing non-robust features, we search for features in a small $\epsilon$ ball ergo humans cannot perceive and don't care. In practice, ATTACKS DONT CONVERGE but even if they do, we leak an imperceptible noise.\\\\
%
- HSIC is unrelated. Could be that HSIC doesn't capture the appropriate dependency measure, OR that dependency is just the wrong story. Suppose HSIC is just a bad measure, so then DropLayer should reduce dependency. BUT that doesn't work! So we need a new story. Should leave DropLayer and Permutation OUT of the HSIC table. \\\\
%
ALL Defenses are dropping robust features. Some (TL-DMI) are replacing them with non-robust to make up the accuracy. In the AutoAttack table, the accuracy under adv examples captures this...it either gets the example wrong because it sucks at classifying or because it was vulnerable to a small noise.\\\\
%
Adam: in intro talk less about screwing up gradients. Talk more about non-robust features.\\\\
%
Need to introduce and out-of-scope-ify the Neg-LS and Trap-MID or skip-connection defenses are like gradient masking. Trap-MID appendix is the only place they tried against PPA and it sucked and they had to cherry pick aka fine tune)\\\\
The new story is that dependency-based defenses delete robust features, and either take the concomitant accuracy penalty (BiDO) or replace them with non-robust features (TL-DMI).
}



\textbf{Paper organization.} \textcolor{red}{PLACEHOLDER.}

\section{\textcolor{red}{Preliminaries}} \textcolor{red}{PLACEHOLDER.}
\textbf{Threat model.}  \textcolor{red}{- white box because (1) we care about evaluating memorization in target models, and (2) we want strong defenses that are practically effective under strong adversaries with minimal assumptions.\\-Our experiments focus on vision because it's the central MIA research stream, though we intend to expand this in future work, and we include a codebase designed to facilitate this expansion }


\section{Model inversion attacks}
The objective of model inversion attacks is to generate images representing a class of the dataset that ideally is closely resembling images of the dataset. The success of the attack is determined by the confidence of the target model (AvgConf), the accuracy of an independently trained evaluation model (AttAcc@1 \& AttAcc@5) and the $L^2$ distance between the VGGFace2 embeddings of the generated images and the images of the class. Importantly, the image need not be a perfect reconstruction of any individual image in the training data, but aims to create a class representative images or class centroids. \textcolor{red}{Maybe we can start with a natural language explanation before the math like this, and the metrics can be explained here.}   

Formally, MIA's consider a private training dataset $\mathcal{D}_{priv}=\{x_i,y_i\}_{i=1}^{N}$, where $x_i\in\mathbb{R}^{d_X}$, $y_i\in\{0,1\}^C$, and each $(x_i,y_i)$ are sampled i.i.d. from a joint distribution $\mathbb{P}_{XY}$. Let $T:\mathbb{R}^{d_X}\to\{0,1\}^C$ be a target model trained on $\mathcal{D}_{priv}$ that the adversary wishes to attack. To conduct a model inversion attack, an adversary seeks a new `inverted' model \textcolor{red}{$\hat{\mathcal{I}}_T$ [do we elsewhere denote it by something else? What do the best other ppl use? I like $\hat{\mathcal{I}}_T$ or maybe $\hat{T}'$]} that maps outputs of $T$, such as $T$'s softmax layer or intermediate outputs, back to the corresponding training examples in $\mathcal{D}_{priv}$. The adversary then queries $\hat{\mathcal{I}}_T$ to `predict' $T$'s private training examples. 

\textcolor{red}{note:    The goal in model inversion is to infer the class \emph{centroids} on the data manifold defined on all pixels/features. privacy leakage exists to the extent that these centroids permit reconstruction of features we `care about' (rather than features that are class-descriminative-but not-otherwise-interesting stuff... \ \ The goal of Model Inversion Defense is to build models that infer decision boundaries without leaking information about the training examples via their class centroids, or that are impervious to having their class centroids re-inferred by an attacker.}

Early MIA's trained the inverted model $\hat{\mathcal{I}}_T$ from scratch by using SGD to directly optimize reconstructions of individual training examples \citep{fredrikson_model_2015}. However, this approach suffers from various optimization complexities when applied to contemporary vision architectures like deep CNN's. Therefore, recent state-of-the-art attacks simplify optimization by adopting an `image prior'---that is, by restricting the search space of training example reconstructions to the image outputs of a domain-relevant GAN, and conducting SGD-based optimization on the GAN's input noise vectors instead of directly on the high-dimensional images' feature space \citep{zhang_secret_2020}. More specifically, GAN-based MIA's optimize a latent noise vector $\hat{z} \in Z$ such that the resultant GAN-generated image is classified as class $c$ maximized confidence by the target model $T$:
%
$$\min_{\hat{z}} \mathcal{L}(T, G, D, \hat{z}, c)$$ 
%
where $\mathcal{L}$ is a standard loss function (e.g. cross-entropy) to maximize the confidence of the GAN-generated image on class $c$,  given pretrained GAN generator $G:Z \to X_{prior}$ and GAN discriminator $D$. Recent attacks on facial recognition classifiers take advantage of pretrained GANs like StyleGAN to perform far more efficient and accurate training data reconstructions \citep{struppek_plug_2022, qiu_closer_2024}. \textcolor{red}{[Mention in the body of the paper that App. \ref{app:mia-related-work-supp} gives details of SOTA MIA attacks.]}

==> dareDEVALII/Sections/old_SEC_INTRO_firstcut.tex <==
\section{Introduction}
A foundational goal of contemporary machine learning is to learn \emph{generalizable} model parameters from the training data without \emph{memorizing} idiosyncratic or sensitive details that may later be leaked. However, it is well known that virtually all contemporary architectures obtain generalizable performance only at the cost of some training data memorization. This tradeoff is a key research frontier both because it is a central impediment to more efficient learning, and also because it enables a new generation of practical privacy attacks, such as model inversion, that reconstruct private training data merely by querying  the trained model. 


\textbf{Memorization is a key impediment to more optimal models.}  In the era of $10$-figure training expenditures, backpropagating to learn idiosyncratic and ungeneralizable training sample information reflects a funamental inefficiency that continues to accrue costs each time the ungeneralizable parameters are called at inference time.



% Memorization remains poorly understood in theory. In particular, the guarantees and intuitions of well-developed conventional privacy theories such as Differential Privacy (DP) \cite{dwork2006differential, dwork2014algorithmic} have only limited applicability to the memorization problem due to a deep objective misalignment between their problem formulation and the contemporary ML setting. Specifically, classical privacy frameworks such as differential privacy  aim to protect the privacy of individual in-sample observations while learning group-level properties of the \emph{in-sample population}. These two goals compete in a manner that can be formally described in a direct information-theoretic tradeoff between the privacy of individual samples and the accuracy of the inferred group-level statistic. 

% In contrast, the training data memorization problem accrues while attempting to learn parameters that generalize to the out-of-sample population. Therefore, there is no obvious direct tradeoff by which out-of-sample accuracy necessitates bearing a cost of memorization. \textcolor{red}{As a result, while conventional privacy theory-based techniques can provably provide protection against memorization during training via, e.g., DP-SGD \cite{abadi_deep_2016}, and also against post hoc training data reconstruction \cite{hayes_bounding_2023}, these techniques may be unnecessarily costly, as accurate out-of-sample predictions may be obtainable absent the release of in-sample aggregates they were designed to protect. In practice, it is well-known that DP-SGD-based memorization defenses are impractically costly in terms of computation and model accuracy. As such, these techniques are not used in large scale applications}


\textcolor{red}{[DP-SGD Goodfellow $\rightarrow$ Hayes? Steinke? Guo on encodings?]}





% Memorization remains poorly understood in theory. While classical privacy frameworks such as Differential Privacy (DP) \cite{dwork2006differential, dwork2014algorithmic} offer provable guarantees against memorization \citep{hayes_bounding_2023}, they were designed to protect the privacy of individual training examples while releasing in-sample group-level statistics, which entails a direct information-theoretic tradeoff. In contrast, the training data memorization problem arises when seeking parameters that generalize out-of-sample where no direct tradeoff necessarily exists. As a result, the high computational and accuracy costs of DP-based techniques may be unnecessary to address memorization, and these techniques are not used in large scale applications


Memorization remains poorly understood in theory. While classical privacy frameworks such as Differential Privacy (DP) \cite{dwork2006differential, dwork2014algorithmic} offer provable guarantees against memorization \citep{hayes_bounding_2023}, they were designed to protect the privacy of individual training examples while releasing parameters that characterize in-sample group-level statistics, not parameters that discriminate between classes in out-of-sample distributions. As a result, the high computational and accuracy costs of DP-based techniques may be unnecessary to address the training data memorization problem, and these techniques are not used in large scale applications.


 Consequently, empirical techniques remain the dominant approach for both studying memorization and detecting memorization-based privacy risks in deployed models.




\textbf{Memorization undermines the privacy of ML deployments.}
Second, memorization underlies a rapidly expanding class of practical privacy attacks on real-world machine learning systems. 


\textbf{We call our approach \textsc{AnTi-Adversarial Training (AT-AT).}~\ATATicon}


==> dareDEVALII/Sections/old_SEC_MotivatingExperiments.tex <==





% \section{\textcolor{red}{Three experiments challenge the memorization theory of reconstruction/MIA defense}}

\section{Three experiments overturn the memorization = exposure view}
If training data exposure to MIA were explained by memorization, formalized as information dependency, then three basic hypotheses would hold:
\begin{enumerate}
    \item Effective defenses would reduce information dependency measures of memorization;
    \item A model that totally memorizes the training data would be vulnerable to MIA;
    \item Models trained without seeing
98\% of the training data pixels (i.e. where memorization is upper bounded at 2\%) would be largely robust to MIA reconstruction.
\end{enumerate}
Our goal in this section is to show experimentally that each of these hypotheses is false. Therefore, the prevailing view that memorization drives training data exposure to reconstruction attacks is incomplete.



% \textbf{Reconstruction defenses do not reduce memorization metrics.} First, we show that contemporary defenses that are widely believed to work by reducing training-data-to-model dependency 
%  \emph{do  not in fact reduce this dependency}, and may in fact increase it, in some cases even according to their own metrics. The Hilbert-Schmidt Independency Criterion (HSIC) \cite{hutchison_measuring_2005} is the standard metric of dependency between inputs and intermediate embeddings in the MIA defense literature, and the only such metric that can be computed for a generic model. The best known defenses that explicitly attempt to disincentivize dependency (BiDO and BiDO+) do so by penalizing HSIC in their loss functions \citep{peng_bilateral_2022, peng_unknown-aware_2025}. Per \cite{peng_bilateral_2022}, HSIC measures the scale of nonlinear dependencies in random variables $X$ and $Y$ as follows: First, nonlinear feature transformations $\phi,\psi$ are created such that $\phi(X)$ and $\psi(Y)$ are members of reproducing kernel Hilbert spaces $\mathcal{F}$ and $\mathcal{G}$, respectively; then, HSIC$(X,Y)$ is computed as the Hilbert-Schmidt norm of the cross-covariance between these features (see Appendix \textcolor{orange}{REF} for details): $$\text{HSIC}(X,Y)=\left \lVert\mathbb{E}[\phi(X)\psi(Y)^\top]-\mathbb{E}[\phi(X)]\mathbb{E}[\psi(Y)]^\top\right\rVert_{HS}^2.$$ 


% To measure how defenses affect HSIC, we train ResNet-18 and ResNet-152 models on FaceScrub in \textcolor{red}{[the same setup as above?]}. Table \ref{table:hsic-r18} reports average HSIC across the validation set using the exact implementation of the HSIC from \cite{peng_bilateral_2022}. We measure model inversion robustness by the top-1 attack accuracy of PPA \cite{struppek_plug_2022} on 75 randomly chosen target classes. \textcolor{orange}{Do we still use 75?}

% As Table \ref{table:hsic-r18} shows [TODO update table], all recent model inversion defenses, including BiDO models trained with standard $(x, \lambda_y)=(0.05, 0.5)$, NegLS, and TL-DMI fail to decrease HSIC$(X,Z_i)$ for all typically used \textcolor{orange}{what does typically used mean here?} intermediate embeddings $Z_i$. We then attempted to deliberately lower HSIC by experimenting with BiDO's weight on HSIC in its loss function, including BiDO$(0.1, 0)$, BiDO$(0.01, 0)$, and BiDO$(0.001, 0)$. These models succeed in lowering HSIC$(X, Z_j)$ for most values of $j$, but provide no significant advantage over the undefended model against a Plug-and-Play attack. In sum, HSIC is orthogonal to defense against MIA. 


\subsection{Effective reconstruction defenses do not reduce memorization (information dependency metrics).}  First, we show that contemporary defenses that are widely believed to work by reducing training-data-to-model dependency \emph{do  not in fact reduce this dependency by a statistically significant amount}, and may in fact increase it, in some cases even according to their own metrics. 
 In the defense literature, the Hilbert–Schmidt Independence Criterion (HSIC) \citep{hutchison_measuring_2005} is the standard dependency metric that can be computed for an arbitrary model. Defenses such as BiDO and BiDO+ \citep{peng_bilateral_2022, peng_unknown-aware_2025} explicitly penalize HSIC between inputs $X$ and intermediate embeddings $Z_j$:
 %
 $$\text{HSIC}(X,Z_j)=\left \lVert\mathbb{E}[\phi(X)\psi(Z_j)^\top]-\mathbb{E}[\phi(X)]\mathbb{E}[\psi(Z_j)]^\top\right\rVert_{HS}^2$$ 
 %
Where nonlinear feature transformations $\phi,\psi$ are created such that $\phi(X)$, $\psi(Z_j)$ are members of reproducing kernel Hilbert spaces $\mathcal{F}$, $\mathcal{G}$, respectively, and $\left \lVert \cdot \right\rVert_{HS}^2$ denotes the Hilbert-Schmidt norm.
%
%

\textcolor{purple}{To measure how defenses affect HSIC, we train ResNet-18 and ResNet-152 models on FaceScrub in the experimental setup described in \textcolor{orange}{REF}. Table \ref{tab:hsic-fs-body} reports average HSIC across the train set using the exact implementation of the HSIC from \cite{peng_bilateral_2022}; see extended results in App. \ref{app:hsic-extended-results}. We measure model inversion robustness by the top-1 attack accuracy of PPA \cite{struppek_plug_2022}.}

\input{dareDEVALII/Tables/HSIC_FS_full}
% \input{dareDEVALII/Tables/HSIC_FS_BiDO_hyp}

\textbf{(Non-) Correlation Results.} all recent model inversion defenses, including BiDO models trained with standard $(\lambda_x, \lambda_y)=(0.05, 0.5)$, NegLS, and TL-DMI fail to decrease HSIC$(X,Z_i)$ for all standard intermediate embeddings $Z_i$ where HSIC is measured. 

\textbf{(Non-) Causal Results.} BiDO$(\lambda_x, \lambda_y)$ allows us to manipulate the weights $\lambda_x$ on HSIC and $\lambda_y$ on accuracy, respectively directly in its loss. We leverage this to experimentally lower HSIC by choosing (BiDO($0.1$, $0$), BiDO($0.01$, $0$), and BiDO($\lambda_1$=$0.001$, $0$)) (see App. \ref{app:hsic-extended-results}). These experimental `HSIC treatment' models succeed in lowering HSIC$(X, Z_i)$ for most values of $i$ compared to `standard' BiDO($\lambda_1$=$0.5$, $0.5$) models, implying reduced memorization/information dependency, but they provide \emph{worse} defense against reconstructions. In sum, reducing HSIC does not cause privacy under MIA. 
\textcolor{orange}{\textbf{It's weird to set $\lambda_y$=0 according to their paper so we will have to be careful how exactly we word this. Maybe we can be vague and defer to appendix?}}

% OLS Joint test: Using car::linearHypothesis with HC3 gives a robust Wald F-test of the null that all four HSIC coefficients are zero. Result: 
% F(4,7)=1.61,p=0.27
% F(4,7)=1.61,p=0.27. This is the most conservative frequentist test under the OLS framework given the sample size.

% 2. Beta Regression (logit link)


% Why use it: Unlike OLS, Beta regression respects the bounded support and models the mean–precision structure. You also reported the dispersion (“phi”), which was significant, indicating nontrivial precision effects.

% Interpretation: In the joint Beta model, HSIC
% Z1
% Z1
% 

%  showed a nominal 
% p=0.047
% p=0.047, but the other HSIC terms were null.

% 3. Joint Tests in the Beta Framework

% You did two kinds:

% Likelihood Ratio (LR) Test: lrtest compared the full beta regression (with HSIC terms) to a restricted intercept-only model.

% Assumptions: Relies on the model’s MLE being well-specified; uses chi-square asymptotics.

% Result: 
% χ2(4)=5.05,p=0.28
% χ
% 2
% (4)=5.05,p=0.28. So no joint evidence that HSIC terms improve fit.

% Wald Chi-square Test (on mean coefficients): car::linearHypothesis tested whether all HSIC coefficients equal zero, using the model-based covariance for the mean submodel.

% Assumptions: Approximate chi-square under large sample asymptotics, less robust to small 
% n
% n.

% Result: 
% χ2(4)=5.70,p=0.22
% χ
% 2
% (4)=5.70,p=0.22. Again, no significance.

% 4. Why Run Both OLS and Beta?

% OLS with robust SEs: provides a model-agnostic check (no distributional assumptions beyond finite variance).

% Beta regression: provides a distribution-appropriate check for proportions.

% Agreement across both increases confidence that the null result (no HSIC effect) is not an artifact of modeling choice.
\subsection{A model that fully memorized the dataset is not vulnerable to model inversion}
%
\textbf{High memorization can yield low reconstruction.} \textcolor{orange}{Finally}, we show that models that perfectly memorize their training dataset are \emph{less vulnerable} to MIA reconstruction than state-of-the-art MIA defenses. Specifically, based on seminal works of \citep{zhang_understanding_2017} and \citep{zhang_understanding_2021}, it is now well-known that deep networks can learn to (almost) perfectly classify training data when the labels are randomly permuted, yielding full memorization of the training set. \textcolor{red}{say dependency?} However,  \autoref{table:perm} shows that PPA is completely ineffective against the permuted model, as it fails to converge to any high-confidence image. Thus, full memorization does not increase privacy leakage under MIA. \textcolor{orange}{I would like to say this in a way that focuses on dependency. Do we have HSIC for permutation model?}
\textcolor{red}{Also we say that permutation is less vulnerable than other baseline defenses, but we don't include them in the table, and we don't report confidence in the later table where we do include them? So either we should add this, or add a note, or add App., or we need to change the way we phrase this result here and in the intro.} 
%
\input{dareDEVALII/Tables/Permutation-test}
%
\subsection{Low memorization can yield extensive reconstruction.} 
%
We construct a mask-based model that hides over \sout{98\%} \textcolor{orange}{97\%} of the pixels in training data images from the model during training with a loss of only a few percentage points of test set accuracy. Three example applications of this mask is shown in Fig. \ref{fig:lasso-orig-and-masked}. We create these masks using a novel \textit{lasso-based mask layer}; see details in App. \ref{app:masklayer}. For a given model, the same mask is applied to all images before being passed to the model during training, rendering the masked pixels \emph{completely unseen} by the model throughout training. 

To measure the effect of this mask on MIA robustness, we train ResNet-18 and ResNet-152 models on FaceScrub according to the same experimental setup in section \textcolor{orange}{REF}. Table \ref{table:drop-layer} compares PPA reconstruction on our mask-based model versus vanilla undefended ResNets. We also compare against an undefended model trained with early stopping to provide a baseline with accuracy identical to our masked model's accuracy, \sout{as it is known} \textcolor{orange}{in line with the common observation} that less accurate models are naturally more robust to MIAs (see e.g. \citet{struppek_be_2024}).
%
\input{dareDEVALII/Figure_code/lasso_original_and_masked}
%
\textbf{Results.} Despite hiding over \sout{98\%} \textcolor{orange}{97\%} of the pixels in training data from the image, PPA still obtains reconstructions that are classified as their original class \sout{in $>$} \textcolor{orange}{over} 50\% of the time. When controlling for accuracy, our mask-based model is responsible for a meager $15$\% additional loss in \emph{top-1} attack accuracy compared to an undefended model, and the minimum FaceNet distance [\textcolor{orange}{how to talk about this metric?}] is actually larger for the undefended model. SOTA defense TL-DMI \cite{ho_model_2024} achieves a much more impressive performance at a similar test accuracy, allowing for a top-1 attack accuracy of 16.3\% and 21.9\% for ResNet-152 and ResNet-18, respectively, as well as a lower minimum FaceNet distance. Fig. \ref{fig:lasso-orig-and-masked} shows some examples of successful attack-generated images when targeting our mask-based ResNet-18 model.
%
\input{dareDEVALII/Tables/DropLayer}
%
\textbf{Recent theoretical advances in data privacy do not explain mask-based model performance.} [see drafting in \ref{draft:droplayer}]
%

==> dareDEVALII/Sections/old_algorithm-AT-AT-wallpaperOVERLAYwrapped.tex <==
% % Preamble (if not already present)
% \usepackage{wrapfig}
% \usepackage{caption}   % for \captionof
% \usepackage{algorithmic} % or algpseudocode, whichever you use

% --- Right-wrapped AT-AT "algorithm" ---
\begin{wrapfigure}{r}{0.48\textwidth}   % side & width
  \vspace{-\baselineskip}               % pull tight to paragraph start
  \setlength{\intextsep}{6pt}
  \setlength{\columnsep}{14pt}

  \begin{minipage}{0.48\textwidth}      % FIXED width; no varwidth
    \begin{AlgWithBGfaint}{dareDEVALII/Figures/ATATiconV4.png}

      % Algorithm-like caption (no number). Remove 'labelformat=empty' to number.
      {\captionsetup{type=algorithm, labelformat=empty}
       \captionof{algorithm}{\textbf{Anti-Adversarial Training (AT-AT)~\ATATicon}}
      }
      % Add to List of Algorithms:
      \addcontentsline{loa}{algorithm}{AT-AT}

      \begin{algorithmic}
        \INPUT  Data $\mathcal{D}$, Model $\mathcal{M}(\theta,\lambda)$ \\
        \STATE \textbf{for} $(x,y) \in \mathcal{D}$ \textbf{do}
        \STATE \ \ $y' \sim \text{Uniform}(C\setminus y)$
        \STATE \ \ $x_{\text{adv}} \gets \min\limits_{\lVert x'-x\rVert_\infty\le\varepsilon}\!
                    \mathcal{L}_\mathcal{M}(x',y') \quad\#\,\textsc{PGD}$
        \STATE \ \ $\mathcal{L} \gets
          \underbrace{\mathcal{L}_\mathcal{M}(x,y)}_{\text{vanilla}}
          + \lambda \cdot
          \underbrace{\mathcal{L}_\mathcal{M}(x_{\text{adv}},y')}_{\text{anti-adv.}}$
        \STATE \ \ $\theta \gets \theta - \alpha \nabla_\theta \mathcal{L}$
        \STATE \textbf{return} $\mathcal{M}$
      \end{algorithmic}

      \label{alg:ATAT}
    \end{AlgWithBGfaint}
  \end{minipage}

  \vspace{-\baselineskip}
\end{wrapfigure}


==> dareDEVALII/Sections/old_algorithm-AT-AT-wallpapered.tex <==
%
%
%
\begin{AlgWithBG}{dareDEVALII/Figures/ATATiconV4.png}
\begin{algorithm}[H]
\caption*{\textbf{Anti-Adversarial Training (AT-AT)~\ATATicon}} % NOTE caption vs caption* asterisk
%
\addcontentsline{loa}{algorithm}{AT-AT}
%
\begin{algorithmic}
    	\INPUT  Dataset $\mathcal{D}$,  \ Model $\mathcal{M}$ with params. $\theta$,  \ $\lambda$ \\
        %
    	\STATE \textbf{for} $(x,y) \in \mathcal{D}$ \textbf{do} \\
        %
        % \STATE \ \ \ \ $t \overset{uar}{\sim} [C]$
        \STATE \ \ \ \ $y' \sim \text{Uniform}(C\setminus y)$\\ % {y} denotes a set of y's rather than a singleton element y in combinatorics/optimization
        %
        \STATE \ \ \ \ $x_{\text{adv}} \gets \min\limits_{||x'-x||_{\infty}\le\varepsilon} \mathcal{L}_\mathcal{M} (x',y')$ \ \ \# Solved via $l_\infty$ \textsc{PGD} \\
        %
        \STATE \ \ \ \ \ $\mathcal{L} \gets 
        \underbrace{\mathcal{L}_\mathcal{M} (x,y)}_{\text{vanilla}} \ \ \ + \ \ \ \lambda  \cdot \underbrace{\mathcal{L}_\mathcal{M} (x_{\text{adv}}, y')}_{\text{anti-adv.}}  $ \\
        %
        \STATE \ \ \ \ \ $\theta \gets \theta - \alpha \nabla_\theta \mathcal{L}$
        %
        \STATE \textbf{return} \ \   $\mathcal{M}$
        %
  \end{algorithmic}
  \label{alg:ATAT}
\end{algorithm}
\end{AlgWithBG}

==> dareDEVALII/Sections/old_autoattack_sec_backup.tex <==
%
%
%

\section{The \{privacy leakage, accuracy, adversarial robustness\} tradeoff}
\label{sec-autoattack}
%
\textcolor{blue}{Reminder: Drop the nodefs (once we have many more) and re-run so we don't dominate regression. Report both.\\}
%
Our goal in this section is to describe a previously unobserved three-way \{privacy leakage, accuracy, adversarial robustness\} tradeoff that characterizes the performance of memorization dependency-based MIA defenses on the main architectures and datasets used to benchmark privacy attacks and defenses in recent work. We accomplish this by presenting the first systematic tests of the robustness of MIA defenses to a very different attack vector: adversarial examples. These tests allow us to consider the accuracy and privacy of MIA defenses against the robustness of their feature bases, which has not yet been measured comparatively. 

% Adversarial examples are small noise perturbations that when added to an image in the dataset, changes the prediction of the model. The noise is restricted to be in a small range $\lvert \lvert \delta \rvert\rvert_{p}<\epsilon$, where $\delta$ is the perturbation, $p$ is the norm and $\epsilon$ is the limit of the size of perturbations. Since the perturbations are limited to very small changes, they are mostly imperceptible for humans and don't carry semantic meaning.     

% The existence of adversarial examples was first discovered in \cite{szegedy_intriguing_2014} and it has since been widely studied how to generate them \cite{croce_reliable_2020} and defend against them \cite{madry_towards_2019, shafahi_adversarial_2019, wong_fast_2020}. 


%
%
% Top of page pics banner of woman with various autoattack noises epsilon vals
\input{dareDEVALII/Figure_code/adversarial_examples_mini_banner}
%
%
\textbf{Tradeoff experimental setup.} Following seminal work by \citep{carlini_evaluating_2019, croce_reliable_2020}, and others, a scholarly consensus has emerged regarding the design elements necessary to ensure the rigor of experiments that measure robustness to adversarial examples. This includes testing models under a diverse variety of attacks and a broad range of constraints $\epsilon$ on the magnitude of feasible adversarial perturbations. We carefully follow these design elements here. Specifically, we report worst-case accuracy on adversarial examples across all attacks in the AutoAttack ensemble, and also separately report accuracy for each of its four constituent attacks: untargeted Auto-PGD with cross-entropy loss; targeted Auto-PGD with Difference of Logits Ratio (DLR) loss; Fast Adaptive Boundary (FAB) \cite{fab}; and Square Attack \cite{square}. \textcolor{red}{!Fix attack citations.}   We find that all models under consideration have identical $0\%$ accuracy under AutoAttack with standard $\epsilon=8/255$ (i.e. $0.031$), which renders model comparisons uninformative. Thus we also recompute attacks with smaller perturbations: $\epsilon\in \{0.031, 0.0025, 0.0005, 0.00001\}$. Fig. \ref{fig:adv-images-banner} shows an example of each. 

\textbf{\textcolor{red}{Currently assuming that all defenses, architectures, datasets, and also PPA and AttackAcc@1 have already been introduced in the motivating experiments. Also assuming that adversarial examples and non-robust features have been described above. Maybe not and maybe not, respectively? Revisit.}}

\textbf{Tradeoff raw results tables.} Table \ref{tab:leakage-accuracy-robustness} presents privacy leakage (PPA Attack@1), test accuracy on clean images, and the worst-case robust accuracy under under AutoAttack adversarial examples (across all constituent attacks) with various perturbation magnitudes $\epsilon$. We also report disaggregated robust accuracy results in Appendices \textcolor{red}{REF, REF, REF, REF}.

Across Table \ref{tab:leakage-accuracy-robustness}, the \{privacy leakage, accuracy, adversarial robustness\} tradeoff is qualitatively noticeable for the undefended model (NoDef) and all defenses that attempt to reduce memorization (MID, BiDO, TL-DMI). Specifically, less privacy leakage (lower Attack@1) corresponds to \emph{worse} clean test accuracy and \emph{worse} robust accuracy under all AutoAttacks. 


\textbf{Estimating the \{privacy leakage, accuracy, adversarial robustness\} tradeoff.} To obtain a principled test of the explanatory strength of the  tradeoff, we estimate simple linear regression models of the following form. This allows us to explicitly test the degree to which a model's privacy leakage (PPA Attack@1) is a simple linear combination of its clean test accuracy and its robust accuracy:
%
% \begin{align}
%     \text{Leakage}_{\text{Attack@1}} = 
%     \beta_0 + 
%     \beta_1 \text{TestAcc} + 
%     \beta_2 \text{Acc}_{\epsilon\text{=}0.0025} + \beta_3 \text{Acc}_{\epsilon\text{=}0.0005} + \beta_4 \text{Acc}_{\epsilon\text{=}0.00001}
%     \label{OLS}
% \end{align}
%
% \begin{align}
% \text{Leakage}_{\text{Attack@1}} &= 
%     \beta_0 + 
%     \beta_1 \text{TestAcc} &\text{ \emph{(Clean accuracy only)};}\\
%     %
%     \text{Leakage}_{\text{Attack@1}} &= 
%     \beta_0 + 
%     \beta_1 \text{TestAcc} + 
%     \beta_2 \text{Acc}_{\epsilon\text{=}0.0025} &\text{\emph{(Clean \& robust at $\epsilon\text{=}0.0025$ only)};}\\
%     %
%     \text{Leakage}_{\text{Attack@1}} &= 
%     \beta_0 + 
%     \beta_1 \text{TestAcc} + 
%     \beta_2 \text{Acc}_{\epsilon\text{=}0.0025} + \beta_3 \text{Acc}_{\epsilon\text{=}0.0005} + \beta_4 \text{Acc}_{\epsilon\text{=}0.00001} &\text{\emph{(All predictors).}}
%     \label{OLS}
% \end{align}
%
%
%
%
%
% \begin{align}
% \text{Leakage}_{\text{Attack@1}} &=
%   \beta_0 + \beta_1 \,\text{TestAcc}
%   \tag*{\emph{(Clean accuracy only)}}\\
% %
% \text{Leakage}_{\text{Attack@1}} &=
%   \beta_0 + \beta_1 \,\text{TestAcc} + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
%   \tag*{\emph{(Clean \& robust at $\epsilon$=$0.0025$ only)}}\\
% %
% \text{Leakage}_{\text{Attack@1}} &=
%   \beta_0 + \beta_1 \,\text{TestAcc} + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
%   + \beta_3 \,\text{Acc}_{\epsilon=0.0005} + \beta_4 \,\text{Acc}_{\epsilon=0.00001}
%   \tag*{\emph{(All predictors)}}
% \end{align}
%
%
%
\begin{align}
\text{Leakage}_{\text{Attack@1}} &=
  \beta_0 + \beta_1 \,\text{TestAcc}
   \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad 
   \text{\emph{(Clean accuracy only)}} \label{eq:OLSclean}\\
%
\text{Leakage}_{\text{Attack@1}} &=
  \beta_0 + \beta_1 \,\text{TestAcc} + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
   \quad \quad \quad \quad \quad \quad \quad \quad \ \
   \text{\emph{(Clean \& robust at $\epsilon\text{=}0.0025$ only)}} \label{eq:OLSrobust}\\
%
\text{Leakage}_{\text{Attack@1}} &=
  \beta_0 + \beta_1 \,\text{TestAcc} + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
  + \beta_3 \,\text{Acc}_{\epsilon=0.0005} + \beta_4 \,\text{Acc}_{\epsilon=0.00001}
   \quad \ \ \text{\emph{(All predictors)}} \label{eq:OLSall}
\end{align}
% \[
% \begin{alignedat}{2}
% \text{Leakage}_{\text{Attack@1}} &= \beta_0 + \beta_1 \,\text{TestAcc}
%   &\quad& \text{\emph{(Clean accuracy only)}};\\
% \text{Leakage}_{\text{Attack@1}} &= \beta_0 + \beta_1 \,\text{TestAcc}
%   + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
%   &\quad& \text{\emph{(Clean \& robust at $\epsilon$=$0.0025$ only)}};\\
% \text{Leakage}_{\text{Attack@1}} &= \beta_0 + \beta_1 \,\text{TestAcc}
%   + \beta_2 \,\text{Acc}_{\epsilon=0.0025}
%   + \beta_3 \,\text{Acc}_{\epsilon=0.0005}
%   + \beta_4 \,\text{Acc}_{\epsilon=0.00001}
%   &\quad& \text{\emph{(All predictors).}}
% \end{alignedat}
% \]
%
We are careful to also estimate alternative Beta regression variants of each of the above models with appropriate distributional assumptions to capture the fact that the response variable (PPA Attack@1) is bounded in $[0,1]$:
%
% Technically, the response variable (PPA Attack@1) is bounded in $[0,1]$, this we also consider a Beta regression variation of the above model that conveys the appropriately bounded distributional assumption:
%
\begin{align}
    \text{Leakage}_{\text{Attack@1}} &\sim \text{Beta}(\mu_j \phi, \ (1 - \mu_j) \phi)   \nonumber\\
    g(\mu_j) &=     
    \beta_0 + 
    \beta_1 \text{TestAcc} 
       \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad 
   \text{\emph{(Clean accuracy only)}} \label{eq:betaclean}\\
    %
    g(\mu_j) &= 
    \beta_0 + 
    \beta_1 \text{TestAcc} + 
    \beta_2 \text{Acc}_{\epsilon\text{=}0.0025}    \quad \quad \quad \quad \quad \quad \quad \quad \quad
   \text{\emph{(Clean \& robust at $\epsilon\text{=}0.0025$ only)}} \label{eq:betarobust}\\
    % 
    g(\mu_j) &= 
    \beta_0 + 
    \beta_1 \text{TestAcc} + 
    \beta_2 \text{Acc}_{\epsilon\text{=}0.0025} + \beta_3 \text{Acc}_{\epsilon\text{=}0.0005} + \beta_4 \text{Acc}_{\epsilon\text{=}0.00001}
    \quad \quad \ \ \text{\emph{(All predictors)}} 
     \label{eq:betaall}
\end{align}
%
Where response PPA Attack@1 is modeled as a beta distribution with mean $\mu_j$ and precision $\phi$, where the mean is linked to predictors via the standard logit link function $g(x)$.


                  
\textbf{Results.}
Across various specifications, linear models show that linear combinations of clean test accuracy and robust accuracy at various AutoAttack $\epsilon$ explain $R^2=94.2\%$ of the variance of privacy leakage, measured by PPA Attack@1. These results are robust to various alternate specifications, robust clustered standard errors (clustered by architecture and/or dataset), etc. See Appendix REFERENCE.

\textbf{Computing \emph{accuracy-adjusted privacy gain}: a new comparison metric for privacy benchmarking}

\textbf{Computing \emph{accuracy-adjusted robustness cost}: a new comparison metric for privacy benchmarking}

We can use these linear models to compute the concrete costs of privacy. For example, 
holding test accuracy constant, reducing leakage (PPA Attack@1) by $1$ percentage point corresponds to a:
\begin{itemize}
    \item  $0.43$ percentage-point decrease (95\% CI: 0.31–0.71 pp) in AutoAttack robust accuracy at $\epsilon=0.0025$;
    \item $1.93$ percentage-point decrease (95\% CI: 1.44–2.94 pp) in AutoAttack robust accuracy at $\epsilon=0.0005$.
\end{itemize}
In other words, each increase in privacy that hurts MIA attacker accuracy by $1\%$ costs the model approximately $2\%$ accuracy under imperceptible adversarial examples ($\epsilon=0.0005$).







%
%
% Main Body AutoAttack Table
\input{dareDEVALII/Tables/AA-bodyofpaper}
%
%
\newpage
\clearpage
%
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{dareDEVALII/Figures/leak_vs_TestAcc.pdf}
    \caption{Leakage (PPA Attack@1) vs. clean test accuracy (see Table \ref{tab:leakage-accuracy-robustness}).}
    \label{fig:leakage_vs_accuracyonly}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{dareDEVALII/Figures/leak_vs_pred_regwall3eps.pdf}
    \caption{Leakage (PPA Attack@1) vs. leakage predicted from a simple linear combination of clean accuracy and robust accuracy (see Table \ref{tab:leakage-accuracy-robustness}). Goodness of fit R^2=0.94.}
    \label{fig:leakage_vs_pred_leakage}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{dareDEVALII/Figures/leak_vs_robustacc.pdf}
    \caption{Leakage (PPA Attack@1) vs. robust accuracy at various AutoAttack$\epsilon$.}
    \label{fig:leakage_vs_each_AdvExEpsilon}
\end{figure}



\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\linewidth]{dareDEVALII/Figures/tradeoffsMarioKart.jpg}
    \caption{Accurate illustration of the tradeoffs between accuracy, robustness, and privacy.}
    \label{fig:tradeoffs-mariokart}
\end{figure}



% As explained by \cite{carlini_evaluating_2019}, adversarial robustness (and, therefore, adversarial vulnerability) is often improperly quantified. To mitigate this issue, \cite{carlini_evaluating_2019} provide a checklist of actions to take to ensure proper evaluation of adversarial robustness, including performing adaptive attacks, applying a diverse set of attacks, and verifying that attacks have converged. In response to this advice, the AutoAttack ensemble \cite{croce_reliable_2020} has emerged as a popular benchmark to measure adversarial robustness due to its fixed hyperparameters, automatic convergence checks, and diversity of attacks. The four primary adversarial attacks in the ensemble are 1) untargeted Auto-PGD with cross-entropy loss; 2) targeted Auto-PGD with Difference of Logits Ratio (DLR) loss; 3) Fast Adaptive Boundary (FAB) \cite{fab}; and 4) Square Attack \cite{square}. \\\\


% Adversarial examples are small noise perturbations that when added to an image in the dataset, changes the prediction of the model. The noise is restricted to be in a small range $\lvert \lvert \delta \rvert\rvert_{p}<\epsilon$, where $\delta$ is the perturbation, $p$ is the norm and $\epsilon$ is the limit of the size of perturbations. Since the perturbations are limited to very small changes, they are mostly imperceptible for humans and don't carry semantic meaning.     

% The existence of adversarial examples was first discovered in \cite{szegedy_intriguing_2014} and it has since been widely studied how to generate them \cite{croce_reliable_2020} and defend against them \cite{madry_towards_2019, shafahi_adversarial_2019, wong_fast_2020}. 

% \input{dareDEVALII/Figure_code/adversarial_examples}


% \textbf{Our contribution II: The privacy-robustness feature tradeoff.}

% %We uncover a previously unknown mechanism that directly links training data exposure vulnerabilities to the well-studied robust–non-robust feature tradeoff from the adversarial examples literature. 
% To probe these phenomena, we conduct the first systematic evaluation of the robustness of memorization/MIA defenses to adversarial examples. Our analysis reveals that state-of-the-art privacy defenses do not primarily protect against reconstruction by reducing direct data–model dependency, as widely assumed. Instead, they operate by reshaping the learned feature basis. Specifically, they protect privacy by unintentionally suppressing reliance on ``robust features'' (i.e., generalizable features that are stable under human-imperceptible perturbations and align with human-interpretable semantics), and in some cases, replacing them with ``non-robust features'' (i.e., features that generalize well but are imperceptible to humans and unstable under perturbation) \citep{ilyas_adversarial_2019, ilyas2016, szegedy2013intriguing, [add-post-2019-cites]}. This shift yields a tradeoff: suppressing robust features strips semantically meaningful information from the model but degrades accuracy, while replacing robust features with non-robust features recovers accuracy at the cost of brittleness, leaving models vulnerable to adversarial examples. Although robust–non-robust feature reliance is heavily studied in adversarial robustness, our work is the first to show its central role in training data privacy vulnerabilities. 


%  \textcolor{red}{[make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with Adversarial Examples]}


==> dareDEVALII/Sections/old_experimental_setup.tex <==
\subsection{Experimental setup}

[commenting out since it's redundant with the experimental setup sections we already have]

% For our main experiments, we train ResNet-18 and ResNet-152 \cite{he_deep_2015} as target models. Following previous MIA literature, we run our experiments on the popular FaceScrub \cite{ng_data-driven_2014} and CelebA \cite{liu_deep_nodate} datasets. As in previous works \cite{struppek_be_2024, struppek_plug_2022, ho_model_nodate}, we include only the 1000 most prevalent classes in the CelebA dataset. We focus on the high-resolution scenario, resizing images to $224 \times 224$, as well as performing [our other standard image processing].

% For our attacks, we use Plug \& Play \cite{struppek_plug_2022} and IF-GMI \cite{qiu_closer_2024}, which are the current state-of-the-art in the white-box, high-resolution scenario that is the focus of our paper. Attacks on models trained on FaceScrub target all classes unless otherwise specified; for models trained on CelebA, we instead target a seeded random subset of 75 of the 1000 classes. As attack time and compute scale roughly linearly with the number of classes targeted, this approach reduces time and compute by over 90\% for our CelebA experiments, while the results are comparable to running on all classes [TODO put example of this in Appendix].


 

==> dareDEVALII/Sections/old_main_results.tex <==
\subsection{Main Results}

\input{dareDEVALII/Tables/FS-ppa}

\input{dareDEVALII/Figure_code/MIA_grid-protocol-MaxConf}
\input{dareDEVALII/Figure_code/MIA_grid}

\input{dareDEVALII/Tables/FS-IF}
\input{dareDEVALII/Tables/CelebA-ppa}

\input{dareDEVALII/Tables/CelebA-IF}

\input{dareDEVALII/Tables/Dogs-ppa}

These results show that ...

==> dareDEVALII/Sections/permutation_experiment.tex <==
\subsection{Permuting the Labels}
Next we conduct an experiment of training and attacking a model that has fully memorized the dataset. We do this by following the methodology of \citet{zhang_understanding_2017}, that shows that deep neural networks can fully fit to random labels, i.e fully memorizing the training data. We do this by permuting the labels, thus destroying any correlation between images and labels. 

We find that we can obtain $+99\%$ train accuracy with this model, and as such have wholly memorized the training data. If memorization is the main driving factor for MIA's, then it would stand to reason that the attacks would work well against this model. Yet, as we see in \autoref{table:perm}, PPA is completely ineffective against the permuted model, as it is not able to converge to any high confidence images on the target. This experiment shows that semantically meaningful features, of which the $100\%$ memorization model have none, are necessary for the MIA's optimization goal to converge.  

\input{dareDEVALII/Tables/Permutation-test}


% \begin{itemize}
%     \item \cite{zhang_understanding_2017} showed that deep CNNs are capable of learning all training data even when the labels are permuted and have no visual meaning
%     \item Such a model with permuted labels can be said to have wholly memorized the training data
%     \item As shown in table \ref{table:perm}, PPA is completely ineffective against the permuted model. While this result is to be expected, it nonetheless highlights how memorization is not important for model inversion.
% \end{itemize}

==> dareDEVALII/Sections/related_work_adversarial_evaluation.tex <==
\subsection{Tradeoff: Experimental Results}

[shailen: commented out since Section 6 discusses this]
% We present a comprehensive evaluation of the adversarial robustness of state-of-the-art model inversion defenses. To measure adversarial robustness, we use the AutoAttack ensemble [add footnote with github link?]; see Appendix \ref{app:adv_eval_setup} for more information on AutoAttack and general best practices on evaluating adversarial robustness. We run AutoAttack with varying $L_\infty$ ball constraints on 1024 examples of the validation set for each of the reported target models. As is standard, we consider an example to be successfully perturbed if any of the four attacks create a mis-classification on that example [TODO wording]. We measure \textit{robust accuracy} as the proportion of unsuccessfully perturbed images to total images, as done in previous works \cite{croce_reliable_2020}\textcolor{orange}{add extra REF here}.

% \emph{Results.} As seen in \autoref{table:small-aa}, TL-DMI, a state of the art defense that claims to reduce \textit{encoded information of training data} by freezing some of the first layers, introduces a significant amount of susceptibility to adversarial attacks. Our hypothesis is that a large part of why TL-DMI works is because of its reliance on non-robust features. 

% \input{dareDEVALII/Tables/TL-non-robustness}

% We use this as motivation for our novel SOTA general model inversion defense, Anti-AT. The following section details the mechanism and experimental results of this defense.

==> dareDEVALII/Sections/related_work_mi_defenses.tex <==
\subsection{Related Work: Model Inversion Defenses}

\subsubsection{General Model Inversion Defenses}

[commented out since it's redundant with intro]
% All previous model inversion defenses that argue for general robustness have focused on limiting the information leakage from the training data into the model. MID \cite{wang_improving_2020} minimizes an approximation to mutual information between inputs and embeddings calculated using variational methods, arguing that since ``[model inversion] adversaries exploit the correlation between the model input and output for successful attacks, our idea for the defense is to limit the redundant information about the model input contained in the prediction". fIn place of mutual information, BiDO \cite{peng_bilateral_2022} instead seeks to minimize a kernel-based dependency measure between input and embedding while adding a second regularizer term that maximizes the dependency between embedding and output; the BiDO authors claim that this approach `` limits redundant information propagated from the inputs to the latent representations which can be exploited by the adversary" \cite{peng_bilateral_2022}. More recently, TL-DMI \cite{ho_model_nodate} freezes the first few layers of the pre-trained target model when fine-tuning on $\mathcal{D}_{priv}$, seeking to ``limit the number of layers encoding sensitive information" from $\mathcal{D}_{priv}$. SCA \cite{dibbo_improving_2024} intersperses sparse coding layers into the target model in order to ``control the amount of irrelevant private information encoded in a model's intermediate representations".

\subsubsection{Specific Model Inversion Defenses}
Other model inversion defenses have instead more directly `disrupted' the MIA optimization process in a specific way. RoLSS and its variants \citep{koh_vulnerability_2024} remove or weaken the target model's skip connections to impede gradient flow during attack optimization. NegLS \citep{struppek_be_2024} employs negative label smoothing to make the target model consistently overconfident in its predictions, taking advantage of the reliance of most MIAs on target model confidence scores. Trap-MID \citep{liu_trap-mid_2024} uses strategies from backdoor attacks to build `trapdoors' during training to mislead the MIA optimization process.

\subsubsection{Connections between Adversarial Examples and Model Inversion}

Cite membership inference/adv. vulnerability paper, MIAs that use adversarial examples, ... this is how what we're doing is different... make sure to cite: J. Wen, S. Yiu, and L. Hui. 2021. Defending against model inversion attack
by adversarial examples. In CSR. ; 2. Shuai Zhou 2023 Boosting Model Inversion Attacks with
Adversarial Examples]

==> dareDEVALII/Sections/related_work_non-robust.tex <==
\subsection{Related work: Adversarially Non-robust Features}

For preliminaries on adversarial examples, see App. \ref{app:adv-prelim}.

\subsubsection{Non-robust Features}
Earlier research has examined non-robust features, most notably the well known theory of non-robust features being highly predictive yet brittle under perturbation \citep{ilyas_adversarial_2019}, thus leading to an adversarial vulnerability. They define the concept of useful, robust, and non-robust features as such:

\begin{itemize}
    \item \textbf{$\rho$-useful features:} a feature $f$ is $\rho$-\textit{useful} for a given dataset $\mathcal{D}$, if it is correlated with the true label, i.e
        \begin{align}
            \mathbb{E}_{(x,y) \sim \mathcal{D}}[y \cdot f(x)] \geq \rho
        \end{align}
        Where $\rho_{\mathcal{D}}(f)$ is the largest $\rho$ for which the feature $f$ is still $\rho$-useful on dataset $\mathcal{D}$.
    
    \item \textbf{$\gamma$-robustly useful features:} $\rho$-useful features are also $\gamma$-robust if they remain $\rho$-useful under a set of permutations $\Delta$, i.e:
        \begin{align}
            \mathbb{E}_{(x, y) \sim \mathcal{D}} \left[ \inf_{\delta \in \Delta(x)} y \cdot f(x + \delta) \right] \geq \gamma
        \end{align}

    \item \textbf{Useful, non-robust features:} Lastly, the useful, non-robust features are the features $f$, that is $\rho$-useful but not $\gamma$-robustly \hl{useful for any $\gamma>0$}.
\end{itemize}
When referencing non-robust features, this is the definition that we are using.  

\subsubsection{Connection between adversarial non robustness and model inversion defense \textbf{(Maybe in discussion instead? Or in here as a motivation)}}

While the connection between adversarial attacks and model inversion attacks might seem tangential, there are some earlier results that indirectly show a potential connection. Before current state of the art attacks, it was discovered that that robust models trained with adversarial training makes rudimentary model inversion attacks become feasible \citep{mejia_robust_2019}. This results indicates that the most simple model inversion attacks requires robust features in order to be a valid target. Since then, model inversion attacks have greatly improved, thus the question remains if this is also the case with state of the art generative MIA's.  

Non-robust features are often described as not being \textit{semantically meaningful}. That is, not understandable or recognizable from a human perspective. Importantly, they are different from spurious correlations in that they are still highly predictive of the correct class. \textcolor{orange}{If we can create a model focusing only on these non-robust features, even if the model inversion attacks converges to a high confidence image, the image will likely not look like the target image for anything but the target model. This effect could significantly lower the privacy risk of the non-robust model.} 

Furthermore, earlier work has found that adversarial robust representations have meaningful interpolations in the latent space and the non-robust features do not \citep{engstrom_adversarial_2019}. Since model inversion attacks rely on a generative prior (GAN), the optimization of the attack can be misled when there isn't a clear connection between directions in the latent space of the GAN's noise vector and the latent space of the target model.    

Another potential connection is the tendency for non-robust features to not transfer to other distributions \citep{salman_adversarially_2020}. This can have an effect on the model inversions optimization, as the feature embeddings of images in the GAN space will be less meaningful.  

Based on this, we investigate adversarial non-robustness of many current state of the art defenses ...





==> dareDEVALII/Tables/FS-Robust.tex <==
\begin{table}[h]
\centering
\caption{\textcolor{red}{\textbf{OLD TABLE has been replaced with formatted table. Updates should go to formatted table.}} ResNet-152 FaceScrub models trained with vanilla adversarial training (Robust). RobAcc (robust accuracy) is measured using APGD-CE over 8 batches of the val set. MIA metrics are measured from PPA on 75 classes.}
\label{tab:robust-FS}
\begin{tabular}{llllllll}
\hline
\textbf{Model Name} & \textbf{TestAcc} & \textbf{RobAcc@.0025} & \textbf{RobAcc@.031} & \textbf{AttAcc@1} & \textbf{AttAcc@5} & \textbf{L2-Face} & \textbf{AvgConf} \\ \hline
R152-NoDef & 0.958 & 0.122 & 0 & 0.881 & 0.982 & 0.781 & 0.859 \\ \cline{1-1}
R152-FS-Robust-eps.01 & 0.921 & 0.887 & 0.011 & 0.555 & 0.812 & 0.827 & 0.531 \\
R152-FS-Robust-eps.031 & 0.885 & 0.86 & 0.2 & 0.407 & 0.696 & 0.856 & 0.386 \\ \hline
\end{tabular}
\end{table}

==> dareDEVALII/Tables/mid-comparison.tex <==
\begin{table}[]
\centering
\caption{}
\label{tab:my-table}
\begin{tabular}{lllll}
\textbf{Model Name} & \textbf{TestAcc} & \textbf{AttAcc@1} & \textbf{AttAcc@5} & \textbf{L2-Face} \\
R152-MID-B.01-HigherLR & 0.935 & 0.578 & 0.831 & 0.92 \\
R152-MID-B.01 & 0.95 & 0.391 & 0.699 & 0.95
\end{tabular}
\end{table}

==> dareDEVALII/archive/ALG_AccelGreedy_v3_icml_camready.tex <==





 In this algorithm, $\mathbf{P}_{|D|\times |V|}$ memoizes the log probability of each word in the data per the current iteration's topic-word assignments $Z$; $\mathbf{p}_{1 \times |D| }$ memoizes the current summed log probability of each document per the current $Z$; $\mathbf{M}_{|D|\times|\Phi|}$ memoizes all current marginal values of links; and $\mathbb{m}$ memoizes each document's best not-yet-added topic and its marginal value in a max-heap, so the best link can be accessed
 in $O(\log|D|).$ We denote by $\odot$ the Hadamard product, and by $\mathbb{1}$ a matrix of $1$'s, and we denote all entries corresponding to document $d$ by e.g. $[d,:]$. We denote by \textsc{Emax}$(a,b)$ the elementwise maximum of $a$ and $b$.





%%%%%%%%%%%%%%%%%%%%%%   FAST INITIALIZATION OF FIRST TOPIC PER DOCUMENT  %%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.3em}

\FloatBarrier  % prevent earlier floats from jumping in front

\begin{algorithm}[H]
\caption*{\textbf{FastInitialize}: \emph{Compute each document's first linked topic.}}
\addcontentsline{loa}{algorithm}{FastInitialize}

\begin{algorithmic}
    \INPUT  Doc-word matrix $\mathbf{D}_{|D|\times|V|}$, topic matrix $\mathbf{\Phi}_{|\Phi| \times |V|}$ \\
    %
    % INITIALIZE
    \STATE  $\mathbf{P}_{|D|\times |V|} \gets \log(\epsilon)\cdot \mathbf{D}$ \\
    \STATE  $\mathbf{p}_{1 \times |D|} \gets \mathbb{1}_{1 \times |V|} \cdot \mathbf{P}^T  $ \\
    \STATE  $\mathbf{M}_{|D|\times|\Phi|}\gets \mathbf{D} \cdot \mathbf{\Phi}^T - \mathbf{P} \cdot \mathbb{1}_{|V|\times |\Phi|}$
    \STATE  $E \gets$ the $|D|$ links $[\tau^*_{d^*=1}\text{$\Rightarrow$} 1], \dots, [\tau^*_{d^*=|D|}\text{$\Rightarrow$} |D|]$ \\ \hphantom{E arro}corresp. to the max value per row of $\mathbf{M}$\\
    \STATE  \textbf{for} link $[t^*\text{$\Rightarrow$} d^*] \in E$ \textbf{do}:
    \STATE  \ \ \ \ \ $\mathbf{P}, \mathbf{p}, \mathbf{M}, \mathbb{m} \gets $\textsc{Update($[\tau^*\text{$\Rightarrow$} d^*], \mathbf{D}, \mathbf{\Phi}, \mathbf{P}, \mathbf{p}, \mathbf{M}, \mathbb{m}$})
    %
            \STATE \textbf{return} \ $E, \mathbf{P}, \mathbf{p}, \mathbf{M}, \mathbb{m}$%,\ \  $Z$ 
            %
  \end{algorithmic}
  \label{alg:FastInit}
\end{algorithm}


%\textcolor{red}{Where $\phi_{phantom}$ is an improper topic with constant small probability on all words, e.g. $[1^{-10}]^{|V|}$}

%%%%%%%%%%%%%%%%%%%%%%   FastGreedy-E-LDA  %%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.8em}

%\vspace{-1em}
\begin{algorithm}[H]
\caption*{\textbf{FastGreedy-E-LDA}: \emph{Main routine.}}
\addcontentsline{loa}{algorithm}{FastGreedy-E-LDA}

\begin{algorithmic}
    	\INPUT  Doc-word matrix $\mathbf{D}_{|D|\times|V|}$, topic matrix $\mathbf{\Phi}_{|\Phi| \times |V|}$, \\ \hphantom{puttt}sparsity upper-bound $\kappa$ \\
     \STATE $E, \mathbf{P}, \mathbf{p}, \mathbf{M}, \mathbb{m} \gets$ \textsc{ FastInitialize}$(\mathbf{D}, \mathbf{\Phi})$\\
     %
     % % RUN THE FOR LOOP
        \STATE \textbf{for} $(\kappa-1)|D|$ steps \textbf{do}\\
           %
           % Add the best topic-doc link to S
           \STATE \ \ \ \ \ $t^*, d^* \gets \text{ the topic and doc. corresp. to \emph{extract }} \max (\mathbb{m})$ \\
           \STATE \ \ \ \  $E \gets [\tau^*\text{$\Rightarrow$} d^*] $ \\
    \STATE  \ \ \ \  $\mathbf{P}, \mathbf{p}, \mathbf{M}, \mathbb{m} \gets $\textsc{Update($[\tau^*\text{$\Rightarrow$} d^*], \mathbf{D}, \mathbf{\Phi}, \mathbf{P}, \mathbf{p}, \mathbf{M}, \mathbb{m}$})
           %
           \STATE \textbf{return} \ $E $%,\ \  $Z$ 
\end{algorithmic}
\label{alg:AccelGreedy}
\end{algorithm}
%$\Phi_R$ stands for realized; X is the random set;
%Where $\mathbb{1}$ is a column vector of $1$'s
%$\odot$ denotes the Hadamard (elementwise) product;




%%%%%%%%%%%%%%%%%%%%%%   Fast memo update   %%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.8em}
\begin{algorithm}[H]
\caption*{\textbf{Update}: \emph{Update the heap  with the current log prob. of $d$ and each word in $d$ after adding a new link to the solution, then update marginal values of each link that includes $d$.}}
\addcontentsline{loa}{algorithm}{UpdateHeap subroutine}
% \textbf{update} log probs. of current $Z$ and marginal values for links to $d$:\\
\begin{algorithmic}
    % \INPUT  Doc-word matrix $\mathbf{D}_{|D|\times|V|}$, topic matrix $\mathbf{\Phi}_{|\Phi| \times |V|}$ \\
    \INPUT  Doc-word matrix $\mathbf{D}_{|D|\times|V|}$, topic matrix $\mathbf{\Phi}_{|\Phi| \times |V|}$, \\ \hphantom{puttt}link $[\tau^*\text{$\Rightarrow$} d^*]$, storage  $\mathbf{P}, \mathbf{p}, \mathbf{M}, \mathbb{m}$\\
    %
    \STATE  $\mathbf{p}[d^*] \gets \mathbf{p}[d^*] + \mathbf{M}[d^*,t^*]$ \\%\textcolor{red}{\text{ Maybe remove this line and just do a prod with a $\mathbf{1}$ when we use \textbf{p} in \textbf{M} line below}}\\
    %
    % Now a loop to update the marginal values for each doc
        \STATE  $\mathbf{P}[d^*,:] \gets \textsc{Emax}( \mathbf{P}[d^*,:], \ \ \  \mathbf{\Phi}[t^*,:] \odot \mathbf{D}[d^*,:]) $ \\
        %
        \STATE $\mathbf{\sigma}_{d^*} \gets \mathbf{\Phi} \odot [\mathbf{D}[d^*,:];\dots;\mathbf{D}[d^*,:] ])$\\
        %
        \STATE $\mathbf{M}[d^*,:] \gets  \mathbb{1}_{|V|\times 1} \cdot \textsc{Emax} ( \mathbf{P}[d^*,:] , \ \  \mathbf{\sigma}_{d^*}) - \mathbf{p}[d^*] $\\
        \STATE $\mathbb{m} \gets insert \max \mathbf{M}[d^*,:]$
        %
   % \STATE $ \mathbb{m}:\mathbb{m}[d^*] \gets insert \max(\mathbf{M}[d^*,:]) $\\
            \STATE \textbf{return} \ $\mathbf{P}, \mathbf{p}, \mathbf{M}, \mathbb{m}$ 
            %
  \end{algorithmic}
  \label{alg:memo}
\end{algorithm}

\FloatBarrier




==> dareDEVALII/archive/ALG_SimpleGreedyAlgorithm.tex <==


\section{Simple Greedy Algorithm}
\label{app:approximationguarantee}


Consider the simple Greedy algorithm that grows the solution set of topic-to-document links $E$ by iteratively adding the link with the greatest marginal contribution to $\dot{f}$. We formalize this algorithm and derive its complexity below. While it is practically infeasible, it has near-optimal global and per-document approximation guarantees. Our optimized \textsc{FastGreedy-E-LDA} algorithm accelerates this simple Greedy algorithm while maintaining the same guarantees.

\begin{algorithm}[H]
%\caption{2-Class Directed Preferential Attachment}
\caption*{\textbf{Simple-Greedy-E-LDA}}
\addcontentsline{loa}{algorithm}{Simple-Greedy-E-LDA}

% \begin{algorithmic}
%     	\INPUT  Corpus $D$, Candidate set of topics $\Phi$, Sparsity constraint upper-bound $\kappa$ \\
%     	\STATE \textbf{initialize} $E \gets \{[\tau_{phantom}\Rightarrow 1], [\tau_{phantom}\Rightarrow 2],\dots\, [\tau_{phantom}\Rightarrow |d|]\}$ %topic-word assignments  $Z_{MAP}:z_{d,i} \gets \phi_{phantom}, \forall [d,i]$\\
%     	\STATE \textbf{for} $t \in \{1,\dots,\kappa|D|\}$ steps \textbf{do}\\
%         %\STATE \ \ \ \ $X \gets$ a random subset of candidate topics $\phi$ in $\Phi\backslash \Phi_{MAP}$
%         \STATE \ \ \ \ \ $[\tau^*\Rightarrow d^*] \gets$ the topic-doc link that adds the highest marginal value,  $\underset{\tau \in \Phi, d\in D}\argmax \  f_{E}([\tau\Rightarrow d])$\\
%         %\STATE $Z \gets \argmax \ \big[ \sum_{d\in D}\sum_{i=1}^{|d|} \ \max_{\tau\in E_d} (\log \phi_\tau[w_{d,i}]) \big]$\\
%         \STATE \ \ \ \ \ $E \gets [\tau^*\Rightarrow d^*]$
%         \STATE \textbf{return} \ \  $E \backslash \{[\tau_{phantom}\Rightarrow 1], [\tau_{phantom}\Rightarrow 2],\dots\, [\tau_{phantom}\Rightarrow |d|]\}$%,\ \  $Z$ 
%   \end{algorithmic}
%   \label{alg:Greedy}
% \end{algorithm}
% %$\Phi_R$ stands for realized; X is the random set; 
% Where $\phi_{phantom}$ is an phantom topic with constant (improper) small probability on all words, e.g. $[1^{-10}]^{|V|}$.


\begin{algorithmic}
    	\INPUT  Corpus $D$, Candidate topic set $\Phi$, Sparsity constraint upper-bound $\kappa$, Phantom topic links $\mathcal{P}$ \\
    	\STATE \textbf{initialize} $E \gets \mathcal{P}$ %topic-word assignments  $Z_{MAP}:z_{d,i} \gets \phi_{phantom}, \forall [d,i]$\\
    	\STATE \textbf{for} $\kappa|D|$ steps \textbf{do}\\
        %\STATE \ \ \ \ $X \gets$ a random subset of candidate topics $\phi$ in $\Phi\backslash \Phi_{MAP}$
        \STATE \ \ \ \ \ $[\tau^*\Rightarrow d^*] \gets$ the topic-doc link that adds the highest marginal value,  $\underset{\tau \in \Phi, d\in D}\argmax \  f_{E}([\tau\Rightarrow d])$\\
        %\STATE $Z \gets \argmax \ \big[ \sum_{d\in D}\sum_{i=1}^{|d|} \ \max_{\tau\in E_d} (\log \phi_\tau[w_{d,i}]) \big]$\\
        \STATE \ \ \ \ \ $E \gets [\tau^*\Rightarrow d^*]$
        \STATE \textbf{return} \ \  $E \backslash \mathcal{P}$%,\ \  $Z$ 
  \end{algorithmic}
  \label{alg:Greedy}
\end{algorithm}
%$\Phi_R$ stands for realized; X is the random set; 
Where each phantom topic $\phi_{phantom}$ in the phantom topic links $\mathcal{P}$ is a topic with constant (improper) small probability on all words, e.g. $[1^{-10}]^{|V|}$.





\paragraph{\textbf{1-1/e Approximation Guarantee.}}
For completeness, we show \textsc{Simple-Greedy}'s $1-1/e$ approximation guarantee via the classic result of \citet{nemhauser1978best}. 
%
%
%  Let $E^{OPT}$ denote the optimal (maximum value) solution of size $\kappa|D|$, with value $\dot{f}(E^*)=OPT$. We claim via induction that for $0\le i \le \kappa|D|$:
%
% \begin{align}
%     f(O) - f(S_i) \le (1-1/k)^if(O)  \label{hypoth}
% \end{align}
%
% This is trivially true for $i=0$. First, consider \textsc{Simple-Greedy}'s solution $S_{i-1}$ at the last iteration $i-1$. Because there are $|O\backslash S_{i-1}| \le k$ more elements in $O$ than in $S_{i-1}$, and the `best' one we can add to $S_{i-1}$ now is what \textsc{Simple-Greedy} will add first, then we have (by subadditivity):
% \begin{align}
%     f(O) - f(S_{i-1}) \le \sum_{a \in O \backslash S_{i-1}} f_{S_{i-1}}(a) \notag \\
% \frac{1}{k}\big(f(O) - f(S_{i-1})\big) \le f_{S_{i-1}}(a_i) \label{useful}
% \end{align}
%
% Now, returning to our hypothesis, we can expand left-hand-side (i.e. `separate out' the last link that was added to \textsc{Simple-Greedy}'s solution at iteration $i$):
% \begin{align} 
% f(O) - f(S_i)  &= f(O) - f(S_{i-1}) - f_{S_{i-1}}(a_i) \notag\\ 
% &\le f(O) - f(S_{i-1}) - \frac{1}{k}\big(f(O) - f(S_{i-1})\big) \text{ \  substituting eq. \ref{useful}} \notag\\
% &=(1-1/k)(f(O) - f(S_{i-1})\notag\\
% & \le (1-1/k)^i f(O)\notag
% \end{align}
%
%
% \noindent Now set $i=k$, rearrange, and use $(1-1/k)^k \le 1/e$ to obtain $f(S) \ge (1-1/e)f(O)$
%
%
Let $E^{OPT}$ denote the optimal (maximum value) solution of size $\kappa|D|$, with value $\dot{f}(E^{OPT})=OPT$. Let $E^{i}$ denote \textsc{Simple-Greedy}'s solution at iteration $i$. We claim via induction that for its iterations $0\le i \le \kappa|D|$:
%
\begin{align}
    \dot{f}(E^{OPT}) - \dot{f}(E^i) \le \Big(1-\frac{1}{\kappa|D|}\Big)^i \dot{f}(E^{OPT})  \label{hypoth}
\end{align}
%
This is trivially true for $i=0$. First, consider \textsc{Simple-Greedy}'s solution $E^{i-1}$ at a previous iteration $i-1$. Because there are $|O\backslash E^{i-1}| \le \kappa|D|$ more elements in $E^{OPT}$ than in $E^{i-1}$, and the `best' one we can add to $E^{i-1}$ now is what \textsc{Simple-Greedy} will add first, then we have (by subadditivity):
\begin{align}
    \dot{f}(E^{OPT}) - \dot{f}(E^{i-1}) \le \sum_{a \in E^{OPT} \backslash E^{i-1}} \dot{f}_{E^{i-1}}(a) \notag \\
\frac{1}{\kappa|D|}\big(\dot{f}(E^{OPT}) - \dot{f}(E^{i-1})\big) \le \dot{f}_{E^{i-1}}(a_i) \label{useful}
\end{align}
%
Now, returning to our hypothesis, we can expand left-hand-side (i.e. `separate out' the last link that was added to \textsc{Simple-Greedy}'s solution at iteration $i$):
\begin{align} 
\dot{f}(E^{OPT}) - \dot{f}(E^{i})  &= \dot{f}(E^{OPT}) - \dot{f}(E^{i-1}) - \dot{f}_{E^{i-1}}(a_i) \notag\\ 
%
&\le \dot{f}(E^{OPT}) - \dot{f}(E^{i-1}) - \frac{1}{\kappa|D|}\big(\dot{f}(E^{OPT}) - \dot{f}(E^{i-1})\big) \text{ \  substituting eq. \ref{useful}} \notag\\
%
&=\big(1-\frac{1}{\kappa|D|}\big)\big(\dot{f}(E^{OPT}) - \dot{f}(E^{i-1})\big)\notag\\
%
& \le \big(1-\frac{1}{\kappa|D|}\big)^i \dot{f}(E^{OPT})\notag
\end{align}
%
%
\noindent Now set $i=\kappa|D|$, rearrange, and use $(1-\frac{1}{\kappa|D|})^{\kappa|D|} \le 1/e$ to obtain $\dot{f}(E) \ge (1-1/e)OPT$.











% \paragraph{\textbf{Complexity of \textsc{Simple-Greedy}.}}
\section{Complexity of \textsc{Simple-Greedy}}
\label{app:simplegreedy}

We now derive the complexity of the vanilla \textsc{Simple-Greedy} algorithm described in Section \ref{sec:submodular} and  compare it to the \textsc{Accelerated-Greedy-E-LDA} algorithm described here:


Simple-Greedy completes in $\kappa|D|$ iterations. Each iteration $i$ of Simple-Greedy computes the marginal value of $|\Phi||D| - i$ links. Without the speedups described in \textsc{FastGreedy-E-LDA}, computing one of these marginal values entails solving $f(E^i \cup [\tau\Rightarrow d]) - f(E^i)$, where $[\tau\Rightarrow d]$ is a new topic-doc link (where $E^i$ denotes the solution at iteration $i$). Computing a value of $f$ requires, for each document in $D$, finding the max log probability of each word in $d$ among $E_d$ topics (or $E_d+1$ topics for $f(E^i \cup [\tau\Rightarrow d])$), then summing the result. Denote the number of words in the longest document by $\ell$. Thus each marginal value requires $O(\ell|E_d||D|)$ which is $O(\ell\kappa|D|)$. An iteration of Simple-Greedy requires computing $O(|\Phi||D|)$ such marginal values, so each iteration is $O(\ell\kappa|\Phi||D|^2)$. 


==> dareDEVALII/archive/abstract_tryingsomething.tex <==




In this paper, we show how to obtain solutions to LDA topic models that exhibit four key properties. First, whereas all mainstream LDA solvers find only locally modal solutions that are arbitrarily badly fit to the data, we show how to obtain solutions that are guaranteed to \emph{near-optimally} describe the data (i.e. maximize an LDA log-posterior objective function). Second, whereas interpreting the results of a mainstream LDA solver currently requires researchers to manually contrive descriptions of what each topic is `about', we we show how to guarantee that each topic in the solution is rigorously interpretable via a near-optimally selected keyword and a known co-occurrence function. Third, whereas mainstream LDA solvers have no known convergence time, we show it is possible to obtain our solutions in just \emph{logarithmic} parallel computation time (adaptivity), so our method can be applied to massive data sets. Fourth, whereas mainstream LDA solvers violate the independence assumptions necessary to use their output in a causal 


resulting topics i

and to do so (4) without violating the independence assumptions required to use the topics for downstream causal inference methods.

interpreting the results requires researchers to manually contrive descriptions of what each topic is `about'








\begin{abstract}



Despite their widespread popularity, LDA topic models have three well-known problems. First, unlike other mainstream methods in the social science toolkit, mainstream LDA solvers have no \emph{provable guarantees}, meaning they find only locally modal topics that are arbitrarily badly fit to the data compared to the topics that would maximize their log posterior objective functions. Second, they also fail to meet contemporary notions of \emph{interpretability} because the algorithms used to solve LDA are interpretively opaque and understanding their results requires researchers to manually contrive descriptions of what each topic is `about'. Third, while the LDA model itself is compatible with \emph{causal inference} frameworks that would allow researchers to study their texts' topics as treatments or outcomes, standard LDA solvers violate the independence assumptions necessary to do so.

%In this paper, we show that it is possible to (1) obtain solutions to LDA models that are guaranteed to \emph{near-optimally} describe the data (i.e. maximize an LDA log-posterior objective function), and where (2) the resulting topics each have rigorous interpretability guarantees. We also show it is possible to obtain these solutions (3) in \emph{logarithmic} parallel computation time (adaptivity), and to do so (4) without violating the independence assumptions required for downstream causal inference methods.


In this paper, we show how to to (1) obtain solutions to LDA models that are guaranteed to \emph{near-optimally} describe the data (i.e. maximize an LDA log-posterior objective function). We then show we can obtain these near optimal solutions while also (2) guaranteeing that each resulting topic is rigorously interpretable via a near-optimally selected keyword and a known co-occurrence function. We also show it is possible to obtain these solutions (3) in \emph{logarithmic} parallel computation time (adaptivity), and to do so (4) without violating the independence assumptions required to use the topics for downstream causal inference methods.

% , such that each topic is associated with a near-optimally selected keyword, and the topic ascribes mass to each other word in proportion to how often it co-occurs with the keyword



% Specifically, we prove that it is possible to efficiently and near-optimally learn the Maximum A Posteriori LDA topic from which each word in a text dataset was drawn given a user-chosen sparsity constraint and access to a large set of topics that include the topics associated with the data. We then show that it is possible to obtain this set of topics using the same coherence functions that are already widely used for evaluating topic models post hoc, and this approach results in topics that have rigorous interpretability guarantees. We also show we can obtain these results without violating SUTVA assumptions, such that researchers can use the resulting near-optimal and interpretable topics as treatments or outcomes in downstream causal inference studies.

Finally, we show that beyond these optimality and interpretability guarantees, this approach consistently returns solutions of higher semantic quality than solutions from state-of-the-art LDA solvers, and these improvements hold across a diverse set of text datasets and a wide range of input and evaluation parameters. We include an application to an additional original dataset of all online text ads on the Google Ads platform from the $2020$ US Presidential election.

While our proofs leverage state-of-the-art machine learning theory, our algorithms are actually simple, practical, fast, and intuitively similar to the human process of iteratively connecting documents to the keywords that best describe them. 

\end{abstract}

==> dareDEVALII/rasmus/abstract.tex <==
\section*{Rasmus Abstract and Outline}

\section*{Abstract}
While achieving high accuracy remains the primary objective in training neural networks, growing concerns have emerged over the leakage of sensitive data through model inversion attacks (MIAs). Prior research has proposed various defense strategies, often attributing their effectiveness to reduced memorization. In this work, we challenge the assumption that MIAs primarily exploit memorization. Through analysis, we demonstrate that defenses believed to reduce memorization actually operate through a different mechanism: adversarial non-robustness. By explicitly optimizing for non-robustness, we develop a defense that significantly outperforms existing methods. Our findings reveal a strong link between adversarial non-robustness and resistance to model inversion, suggesting that both phenomena should be studied jointly in future defense research.

==> dareDEVALII/rasmus/outline.tex <==
\section*{Outline}

\subsection*{Introduction}
\begin{itemize}
    \item From BiDO and TL-DMI’s intuition of encoding minimal amounts of info from the training data, we can deduce that DropLayer should be effective.
    \item However, it is not effective. To further explore this, we perform the permutation experiment (100\% memorization) and find that the attack does not work at all.
    \item We find that BiDO does not work, HSIC is not connected.
    \item TL-DMI does work to some degree, but we find that it is also non-robust.
    \item This leads to the hypothesis that this is the mechanism that makes TL-DMI work and not dependency minimization, which can be exploited in our non-robust MI defense.
\end{itemize}

\subsection*{Related Works}
\begin{itemize}
    \item Quote and cite other defense papers' theories and reasoning for the working of their defenses. (BiDO/TL-DMI vs NegLS)
    \item Discuss some key results from the Madry papers that inspired us in the design of the non-robust defense (Transferability, representations, non-robust features are not bugs, adversarial training).
\end{itemize}

\subsection*{Methodology}
\begin{itemize}
    \item Explain the experimental setups (Datasets, Hyperparameters, Data augmentations, High-Res attacks, StyleGAN prior, DaredEVAL implementation).
\end{itemize}

\subsection*{Experiments}
\begin{itemize}
    \item DropLayer
    \item Permutation
    \item BiDO / HSIC 
    \item Non-robustness of TL-DMI 
    \item 100\% non-robust (Madry)
\end{itemize}

\subsection*{Main Results}
\begin{itemize}
    \item Our non-robust defense on FaceScrub (PPA and IF-GMI)
    \item Our non-robust defense on CelebA
\end{itemize}

\subsection*{Discussion}
\begin{itemize}
    \item While we do beat other state-of-the-art defenses, it is important to reiterate the drawbacks if one were to use this method as an actual defense.
    \begin{itemize}
        \item The point of the paper is that the fact we can use this to significantly beat other SOTA defenses supports the hypothesis of a connection between adversarial non-robust models and model inversion defense.
        \item Adversarial non-robust features transfer badly to other distributions—this is beneficial for defense, especially when prior models are involved. Without any prior, it is unlikely to be ``face-like''.
    \end{itemize}
\end{itemize}

\subsection*{Conclusion}
\begin{itemize}
    \item We show a strong connection between adversarial non-robustness and model inversion resilience. By exploiting this, we outperform other state-of-the-art defenses.
    \item Therefore, we propose that future research into other defenses should also perform adversarial attacks to verify that they didn’t achieve model inversion defense simply by being non-robust, thus introducing new security vulnerabilities in the network.
\end{itemize}

\subsection*{Appendix}
\begin{itemize}
    \item Extra results from non-robust defense
    \item Extra information about training non-robust models with our method
    \begin{itemize}
        \item Show instability of training; mention the importance of saving peak accuracies.
        \item Show how non-robust the model needs to be.
        \item Publish model weights to facilitate reproducibility.
    \end{itemize}
    \item More in-depth explanation of DropLayer implementation and experimentation
\end{itemize}

\cite{struppek_plug_2022}

\cite{zhang_secret_2020}

% \cite{carlini_extracting_nodate}

\cite{carlini2023extracting}


==> dareDEVALII/shailen/abstract.tex <==
\section*{Shailen Abstract and Outline}

\section*{Abstract}
 
 - White-box model inversion attacks (MIAs) against deep facial recognition models pose a privacy risk by inferring revealing attributes about the identities of those in the training data

 - Models vulnerable to MIAs are often considered to have 'memorized' the training data in some sense; to this end, many state-of-the-art defenses have tried, in various forms, to reduce the amount of information about the training data shared or encoded in the target model.

 - We argue that memorization actually has a neutral to negative effect on a model's MIA robustness. We support this claim on three fronts: (1) we introduce a novel feature selection technique that allows for the removal of over 95\% of the pixels in an image, and show that its effect on MIA robustness is limited; (2) we show that a fully trained model with permuted labels, which can be said to have wholly memorized the training data, is perfectly robust against SOTA MIAs; (3) we reveal numerous significant methodological flaws in a recent defense that seeks to minimize the dependence between input and output.

 - In place of reducing memorization, we argue that many defenses rely on \textit{increasing vulnerability to adversarial attacks}, creating a volatile loss landscape that is difficult for an MIA to traverse. We show that a recent SOTA defense is very vulnerable against adversarial attacks

- We then introduce a new defense that explicitly tries to increase adversarial vulnerability which outperforms all other SOTA defenses.

- This points to a natural trade-off between vulnerability to model inversion and adversarial attacks.

\input{dareDEVALII/Tables/mid-comparison}



==> dareDEVALII/shailen/intro_beginning.tex <==
\subsection{Introduction}

\begin{itemize}
    \item AI safety and data privacy have become more of a concern lately, mention rise of MLaaS, etc.
    \item describe similar things to abstract...
\end{itemize}

==> dareDEVALII/shailen/intro_to_mia.tex <==
\subsection{Introduction: Model Inversion Attacks}

% [TODO natural language description before math] \\\\

[commenting out since it's redundant compared to the intro]
% The objective of model inversion attacks is to generate images representing a class of the dataset that ideally is closely resembling images of the dataset. The success of the attack is determined by the confidence of the target model (AvgConf), the accuracy of an independently trained evaluation model (AttAcc@1 \& AttAcc@5) and the $L^2$ distance between the VGGFace2 embeddings of the generated images and the images of the class. Importantly, the image need not be a perfect reconstruction of any individual image in the training data, but aims to create a class representative images or class centroids.    

% Consider a private dataset $\mathcal{D}_{priv}=\{x_i,y_i\}_{i=1}^{N}$, where $x_i\in\mathbb{R}^{d_X}$, $y_i\in\{0,1\}^C$, and each $(x_i,y_i)$ are sampled i.i.d. from a joint distribution $\mathbb{P}_{XY}$. Let $T:\mathbb{R}^{d_X}\to\{0,1\}^C$ be a target model trained on $\mathcal{D}_{priv}$; in a model inversion attack, an adversary with access to the trained classifier $T$ seeks to infer revealing information about the dataset $\mathcal{D}_{priv}$, constituting a leakage of privacy; to do this, the adversary typically generates images that should visually resemble the identities of the members of $\mathcal{D}_{priv}$. In the white-box scenario, the adversary has full access to the model weights, allowing for the usage of gradients.

% Generative MIAs, first proposed by \cite{zhang_secret_2020}, utilize a generative adversarial network (GAN) trained on a public dataset as a natural image prior, allowing for improved image quality and the ability to attack deeper networks. As explained in \cite{struppek_be_2024}, GANs typically consist of a generator $G:Z \to X_{prior}$ and a discriminator $D$; generative MIAs then seek to solve the following optimization goal by optimizing a latent vector $\hat{z} \in Z$:
% $$\min_{\hat{z}} \mathcal{L}(T, G, D, \hat{z}, c)$$
% where $\mathcal{L}$ is a standard loss function (e.g. cross-entropy) to maximize the confidence of the generated image on class $c$. See App. \ref{mia-related-work-supp} for information on recent SOTA generative MIAs.

==> dareDEVALII/shailen/outline.tex <==
\section*{Outline}

\subsection*{Introduction}
\begin{itemize}
    \item describe similar things to abstract
    \item List contributions: 1) novel experiments that limiting shared information is ineffective (DropLayer and Permutations); 2) Reveal other explanations for BiDO and TL performance and flaws in their current explanations; 3) introduce a new SOTA defense that shows the importance of non-robust features.
\end{itemize}

\subsection*{Related work}
\begin{itemize}
    \item Previous model inversion defenses and their explanations for why model inversion defense works, focusing on disproving BiDO and TL intuitions. Frame MID as a worse version of BiDO to avoid discussing it further.
    \item Recent model inversion attacks and metrics they use
    \item FaceScrub and CelebA datasets
    \item Adversarial examples, robust vs. non-robust features, previous inclusions of adversarial-like ideas in the model inversion field, why we're different than them
\end{itemize}

\subsection*{Masking over 95\% of Pixels is an Ineffective Defense} 

% \subsubsection*{A 95\% pixels mask that retains accuracy}
\begin{itemize}
    \item we create a mask that removes over 95\% of pixels, see mask at figure X, see details of creation in Appendix A
\end{itemize}


% \subsubsection*{DropLayer is ineffective as a model inversion defense}
\begin{itemize}
    \item A model trained with this mask shows very limited improvements in inversion robustness beyond what can be explained from the drop in test accuracy
    \item \textit{Figure: Show mask, orig image, masked image, and a good reconstruction. Look for a good one to prove existence}
    \item The table and figure show that loss of information about individual pixels is not of great concern to an MIA because of the strong facial prior from the GAN.
    \item Recent theoretical approaches to guaranteeing privacy by bounding the variance of a reconstruction estimator suggest that the masked pixels should be near impossible to predict, perhaps our result shows that this is a poor theoretical direction to pursue, for more discussion see Appendix Q
\end{itemize}

% \input{dareDEVALII/Tables/DropLayer}

\subsection*{Permuting the Labels}

\begin{itemize}
    \item Madry paper showed that deep CNNs are capable of learning all training data even when the labels are permuted and have no visual meaning
    \item Such a model with permuted labels can be said to have wholly memorized the training data
    \item As shown in table \ref{table:perm}, PPA is completely ineffective against the permuted model. While this result is to be expected, it nonetheless highlights how memorization is not important for model inversion.
\end{itemize}
 
\input{dareDEVALII/Tables/Permutation-test}


\subsection*{Dependency is Unrelated to Model Inversion Robustness}

% \input{dareDEVALII/Tables/BiDO-HSIC}          


\begin{itemize}
    \item BiDO is a recent popular defense, BiDO actually raises HSIC instead of reducing it
    \item While the BiDO paper claims that the second regularizer term is necessary, we show it is not necessary with better hyperparameter tuning, however the models that actually do reduce HSIC have poor performance against model inversion, as shown in the table below
    \item (perhaps in the table, also include an undefended model with acc=88, say ``Most of BiDO attack success performance is explained by accuracy drop anyways" ?
\end{itemize}


\subsection*{The Invertibility of Adversarially Vulnerable Models}
% \subsection{Related work: Adversarial examples}
% \subsection{Results: TL-DMI is Adversarially Vulnerable} 

\begin{itemize}
    \item  Instead of various concepts of 'memorization' and 'dependency', we argue that we should instead be looking at vulnerability to adversarial attacks.
    \item We posit that the irregular loss landscape of models vulnerable to adversarial attacks should make the optimization process of model inversion difficult
    \item We can also think about this in terms of non-robust features, cite Madry '19
    \item We check adversarial vulnerability using the AutoAttack ensemble, which is well-established and comprehensive, follows the principles of adversarial evaluation laid out in (Carlini 2019)
    \item TL-DMI, a recent popular defense, is adversarially vulnerable even under quite small epsilon values, as shown in table \ref{table:small-aa}. We believe this is a significant cause of its success as a model inversion defense.
\end{itemize}

\input{dareDEVALII/Tables/TL-non-robustness}

\subsection*{A New SOTA Defense Focusing on Non-Robust Features}

\input{dareDEVALII/Tables/FS-ppa}

\input{dareDEVALII/Tables/FS-IF}

\input{dareDEVALII/Tables/CelebA-ppa}

\begin{itemize}
    \item To further test our hypothesis about non-robust features and adversarial vulnerability being important to model inversion defense, we seek to create a model that focuses a lot on non-robust features.
    \item Trying to do this using approaches in (Madry 2019) lead to poor accuracy
    \item We instead draw inspiration from adversarial training, and do the ``opposite'' (further explain this here, maybe show the algorithm?)
    \item Our approach is very vulnerable against AutoAttack even under very small epsilon, as shown in table [Insert table]
    \item We improve on state-of-the-art across multiple models, benchmarks, and attacks, as shown in the below tables.
\end{itemize}



\subsection*{Conclusion}
\begin{itemize}
    \item Our results point to the idea that `shared information' is not important for model inversion.
    \item Adversarial robustness and model inversion robustness are connected. Adversarial evaluation is an important part of thorough evaluation of future model inversion defenses.
    \item Our non-robust model is meant as a proof-of-concept and should not be used in practice, see appendix for more info
    \item While adversarial robustness is often achieved by `good' models, for various definitions of `good', model inversion robustness is instead often caused by `bad' models. This means that model inversion defense research might not end up achieving one of the goals of defense research described in \cite{carlini_evaluating_2019} about `measuring the progress of machine learning algorithms towards human-level abilities'. The study of adversarial robustness might achieve this goal, but model inversion robustness does not.

    \item Some other potentially-related concepts for future work: Relation between model inversion for facial classification vs. uncovering memorization in generative models; connection between representation inversion and model inversion, potential vulnerability of adversarially robust models to MIAs, metrics that measure the 'volatility' in the loss landscape in some way, whether these results apply to black-box attacks, or the low-res scenario, or split learning scenario
\end{itemize}

\subsection*{Appendix}

\begin{itemize}
    \item Section on how we made the mask to drop 95\% of pixels, talk about lasso-based origins, adding a mask layer, etc.
    \item Section on Fisher/HCR bounds and how our mask-layer experiment might be a counterexample to it
    \item Section describing hyperparameters used for all different MI defenses, MI attacks, Adversarial attacks
    \item We dropped the learning rate to 0.0001 instead of 0.001 in some cases because it made training better...
    \item Extended HSIC results
    \item Section with figures with visual results of reconstruction for our defense compared to the other defenses
    \item A note on instability and length of training of our non-robust method
    \item A note on why running the attack on only a subset of classes is OK

    \item Information about GPU usage, estimated carbon footprint
\end{itemize}


